Probabilistic failure mechanisms via Monte Carlo simulations of complex microstructures

A probabilistic approach to phase-field brittle and ductile fracture with random material and geometric properties is proposed within this work. In the macroscopic failure mechanics, materials properties and exactness of spatial quantities (of different phases in the geometrical domain) are assumed to be homogeneous and deterministic. This is unlike the lower-scale with strong fluctuation in the material and geometrical properties. Such a response is approximated through some uncertainty in the model problem. The presented contribution is devoted to providing a mathematical framework for modeling uncertainty through stochastic analysis of a microstructure undergoing brittle/ductile failure. Hereby, the proposed model employs various representative volume elements with random distribution of stiff-inclusions and voids within the composite structure. We develop an allocating strategy to allocate the heterogeneities and generate the corresponding meshes in two- and three-dimensional cases. Then the Monte Carlo finite element technique is employed for solving the stochastic PDE-based model and approximate the expectation and the variance of the solution field of brittle/ductile failure by evaluating a large number of samples. For the prediction of failure mechanisms, we rely on the phase-field approach which is a widely adopted framework for modeling and computing the fracture phenomena in solids. Incremental perturbed minimization principles for a class of gradient-type dissipative materials are used to derive the perturbed governing equations. This analysis enables us to study the highly heterogeneous microstructure and monitor the uncertainty in failure mechanics. Several numerical examples are given to examine the efficiency of the proposed method.

==> 1d.tex <==
%=======================================================================
\sectpa[Section3]{One-dimensional examples}
%=======================================================================

In following we used:

\begin{equation*}
	a'(x,t)=\frac{\partial a(x,t)}{\partial x} \AND \dot{a}(x,t)=\frac{\partial  a(x,t)}{\partial  t}
\end{equation*}

Hereinafter, the spatial gradient is denoted as $\Box'(x,t):=\partial\Box(x,t)/\partial x$.


%=======================================================================
 \sectpb[Example1]{Example 1: Linear elasticity}\label{Ex1}
%=======================================================================
This example provides a brief illustrative parameter estimation based on Bayesian inference for one-dimensional linear elasticity. Specifically, we estimate Young's modulus as the single uncertain parameter in the given problem. The observation, i.e., the reference response, is taken as the analytical solution of the governing second-order ordinary differential equation. %The Bayesian approach provides a principal framework for combining prior knowledge with dynamic data in order to make predictions on quantities of interest.

%=======================================================================
\sectpc[Section21]{State variables and kinematics}
\label{sec:basic_def1}
%=======================================================================

Let us consider the one-dimensional boundary value problem (BVP) shown in Figure~\ref{Fig_Ch_intro_2}a. An isothermal elastic rod is completely fixed on the left side and subjected to an imposed traction per unit area ${\bar t}$ on the right side. The external body force $\rho A {\bar b}(x)$ has the sinusoidal form $\rho A {\bar b}(x)={\bar q}(x)=q_0\sin(2\pi x/l)$, as shown in Figure~\ref{Fig_Ch_intro_2}b, where ${\bar b}$ is a body force per unit mass. Moreover, the deformation process is assumed to be quasi-static, such that inertial effects can be neglected.


% \mathrm{H}_0^1(\mathcal{B})
The material is assumed to obey linear elasticity in the small strain setting. Consequently, letting  $\mathcal{B}:=[0,L]$, the displacement field $u : \mathcal{B} \rightarrow \mathbb{R}$ constitutes the only primary variable, from which the strain field is obtained as
%
\begin{equation}
\varepsilon(x)=\frac{\mathrm{d}u(x)}{\mathrm{d}x}  .
\label{small_strain}
\end{equation}
%
The stress field then follows from Hooke's law as
%
\begin{equation}
\sigma(x)=E\varepsilon(x),
\label{stress_elast}
\end{equation}
%
where $E$ is Young's modulus, assumed to be constant throughout the bar for the sake of simplicity.

With these definitions at hand, the quasi-static mechanical balance problem takes the following strong form: 
%
\begin{equation}\label{1Del}
\text{Find}\;\; u(x)\quad \text{s.t.}\;: \quad EA\frac{\mathrm{d}^2u(x)}{\mathrm{d}x^2}+q_0\sin\bigg(\frac{2\pi x}{L}\bigg)=0,
\end{equation}
%
along with the Dirichlet boundary condition $u=0$ at $x=0$ and the Neumann boundary condition $\mathrm{d}u/\mathrm{d}x=\bar{t}/E$ at $x=L$. Here, $A$ is the cross-sectional area of the bar, assumed to be constant for simplicity. The second-order ordinary differential equation  \req{1Del} has the following exact solution for the displacement field:
%
\begin{equation}\label{1Dsol}
	u(x)=\frac{q_0L^2}{4EA\pi^2}\sin\bigg(\frac{2\pi}{L}x\bigg)+\bigg(\frac{\bar t}{E}-\frac{q_0L}{2\pi EA}\bigg)x
	\quad\forall\;0\le x\le L.
\end{equation}

The analytical solution is taken here as the reference response. On the other hand, for the numerical solution, the finite element method is employed, for which the variational formulation of the BVP is presented below.

\begin{algorithm}[!t]
	\vspace{0.2cm}
	\textbf{Initialization ($j=0$)}:  Produce the candidates according to the prior density $\theta^0$\\
	
	\textbf{while}~$j<N$\\
	
	\qquad1. Solve the model equations and estimate the its response  $f(\theta^{j-1})$ considering $\theta^j$.\\
	
	\qquad2. Update the Kalman gain	\quad$\mathcal{K}=\C_{\theta M} \left(\C_{MM}+\mathcal{R}\right)^{-1}$.\\
	
	\qquad3.  Shift the ensemble \quad $\theta^\star=\theta^{j-1}+\K\left( y^{j-1}+s^{j-1}\right)$\\
	
	\qquad4. Accepted/rejected the forecast.\\ 
	
	\qquad5. Set $j=j+1$.
	\caption{Bayesian inversion with ensemble-Kalman filter.} 
	\label{algorithm3}	
\end{algorithm}

%=======================================================================
\sectpc{Energy quantities and variational principles}
\label{sec:energy_functions1}
%=======================================================================
The strain energy density for one-dimensional linear elasticity reads
%
\begin{equation}
W_{elas}(\varepsilon):=\frac{1}{2}E\varepsilon^2=\frac{1}{2}E\bigg(\frac{\mathrm{d}u}{\mathrm{d}x}\bigg)^2.
\end{equation}
%
The total energy functional $\mathcal{E}(u)$ is then given by
%
\begin{equation}\label{1D1}
\begin{aligned}
\mathcal{E}(u)=\int^{L}_{0}AW_{elas}(\varepsilon)\,
\mathrm{d}{{x}}
-\int^{L}_{0} \rho A{ {\bar b}}  u\,\mathrm{d}x
- A \bar{t} u \, \big|_{\partial_N\mathcal{B}}  ,
\end{aligned}
\end{equation}
%
where the external forces evaluated at the Neumann boundary $\partial_N\mathcal{B}\equiv\{L\}$ have been used (Figure~\ref{Fig_Ch_intro_2}a). Minimization of the energy functional~\eqref{1D1} with respect to the displacement field leads to the following weak formulation.

\begin{form}[\textsc{F1}: Bayesian inversion for linear elasticity]
	\label{form_1}
	Consider a given open bounded one-dimensional bar on an interval $\calB:=[0,L]$ with boundary $\partial \calB$ defined at $x=0$ and $x=L$, and constant $E \geq 0$. Find $ u \in \mathcal{W}^u_{\bar{u}}$ satisfying the following Euler-Lagrange equation in weak form:	 
	\begin{align*}
	\calE_u(u;\delta u)=\int^L_{0}\bigg[EA\bigg(\frac{\mathrm{d}u}{\mathrm{d}x}\bigg)\bigg(\frac{\mathrm{d}(\delta u)}{\mathrm{d}x}\bigg)-\rho A \bar{b} \delta u\bigg]\,\mathrm{d}x - A \bar{t} \delta u \, \big|_{\partial_N\mathcal{B}} = 0 \quad \forall \, \delta u \in \mathrm{H}_0^1(\mathcal{B})  . 
    \end{align*} %         \tag{\text{LE}}
Here the main aim of the Bayesian inversion is determining Young's modulus $E$.
%\begin{equation*}
%	E\leftarrow\textsc{BI}\big(\textsc{F1}(u)\big).
%\end{equation*}
\end{form}

\begin{figure}[!b]
	\centering
	{\includegraphics[clip,trim=1cm 21.5cm 1cm 4cm, width=15cm]{Figures/oneD/F1.pdf}}  %left, bottom, right and top
	\caption{ Geometry and loading setup for the one-dimensional bar. (a) Boundary value problem and (b) sinusoidal body force with constant amplitude $q_0=14$ N/m.}
	\label{Fig_Ch_intro_2}
\end{figure}
%=======================================================================
\sectpc{Bayesian inference}
\label{sec:bayesian1}
%=======================================================================

In the present example, we set the bar, of unitary length L = 1 with $x\in\calB:=[0,1]$ that is initially unstretched, $q_0=14$ N/m, and a unit cross-sectional area throughout the bar ($A=1$ m$^2$). The minimum finite element size in the domain $\calB$ is $h=0.005$ mm. The left-end is fixed ($x=0$) while on its right-end ($x=1$, a monotonic displacement increment  $\Delta\bar{u}=5\times10^{-4}$ mm is applied for 1\,001 time steps, see Figure \ref{Fig_Ch_intro_2}.

Then, the statistical problem consists of identifying the Young's modulus $E$ where that is chosen in the bar. Bayesian inference is then applied to determine the  target value, while no specific information (other than its positivity) is available a priori.
\\
From now on, in order to estimate the model response the function
\begin{align}
\texttt{[response] = forwardmodel($\theta^\star$)}
\end{align}
is employed. Then, $\texttt{response}$ is used to calculate the likelihood of the given proposal. The main script named $\texttt{elasticity{\_1}D}$. We assume the elasticity is between $E$=0.1\,GPa and $E$=20\,GPa, the initial guess is $\theta^0=3$, and we use $\sigma^2=0.1$. As a synthetic measurement, we employ $E=4.259$ to estimate the displacement during the time-steps.  
\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/MCMC_MH}} 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/MCMC_AM}}
	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/MCMC_DR}}\\ 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/MCMC_DRAM}}
	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/MCMC_KF}}
	\caption{Example 1. The MCMC chain of $E$ obtained by different Bayesian techniques. Form left to right: MH, AM, and DR (the first row), and DRAM as well as EnKF (the second row).
	}
	\label{MCMC1}
\end{figure}

\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/pdf_MH}} 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/pdf_AM}}
	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/pdf_DR}}\\ 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/pdf_DRAM}}
	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/oneD/pdf_KF}}
	\caption{Example 1. The posterior distribution of $E$ obtained by different Bayesian techniques. Form left to right: MH, AM, and DR (the first row), and DRAM as well as EnKF (the second row).
	}
	\label{pdf1}
\end{figure}

As a one-dimensional Bayesian inversion ($k=1$), we plan to compare the performance of all methods, including the convergence of the MCMC chain, elapsed CUP time, and the convergence rate. Figure \ref{MCMC1} shows the evolution of the MCMC chain using different Bayesian techniques. All chains converged effectively and EnKF shows a significantly lower fluctuation. As a result, as Figure \ref{pdf1} illustrates a narrow posterior distribution has obtained using the MCMC techniques. Again, EnKF-MCMC shows a better performance (a narrower density) compared to others.

\begin{table}[!]
	\caption{Example 1: The median of the posterior density and its elapsed CPU time and the acceptance rate using different MCMC methods}
	\vspace{1mm}
	\centering.
	\begin{tabular}{|l |c c c c c|}
			\hline
	method \hspace{8cm}&MH        & AM    &   DR   &   DRAM   &~~~EnKF       \\\hline\hline
				   ~$E$ \hspace{2cm}  &~~~4.243~~~   & ~~~4.255~~~  & ~~~4.257~~~ &~~~4.259~~~ & ~~~4.26~~~ \\[4mm]
		   CPU time [s]\hspace{2cm}  & 11.9   & 12.68  & 23.36 &22.01 &  66\\[4mm]
		 acceptance rate (\%) &   16.1  &  30.1  &  50.4 & 60.2 &91.8 \\ 
		\hline
	\end{tabular}	\label{comp1}
\end{table}

 


Posterior density provides informative knowledges about the parameter and we extract the median of the accepted candidates as the inferred solution. Table \ref{comp1} shows the computational features of our Bayesian inversion. Although all methods estimated the Young's modulus with a reasonable accuracy, using DRAM and EnKF gives rise to a precise inference. As expected, the acceptance rate of MH is minimum and it increases by a global adaption (adaptive Metropolis). The delayed rejection increases significantly the ratio; however raises the computational time. Combining AM and DR again increases the acceptance ratio 10\% more. Since we adopt the proposal every 100 iterations, AM does not increases the computational time. Regarding EnKF-MCMC the CPU time is much higher; however, using Kalman gain leads an excellent ratio and a very low uncertainty in MCMC, see Figure \ref{MCMC1}. We conclude, both DRAM and EnKF are accurate MCMC techniques.    


 
 %=======================================================================
 \sectpb[Example2]{Example 2: Heat equation with convection contribution}
 \label{Ex2}
 %============================================================
 The heat equation coupled to convection is a convection-diffusion equation used to model heat transfer, e.g., in soil, when a noticeable amount of water is continuously infiltrating.  Convective transport is a physical process that takes place along the streamlines in the
 flow field. So, in the second example, we apply Bayesian inversion to a one-dimensional convection-diffusion equation. Herein, the goal is to estimate thermal diffusivity, and thermal velocity in a convection-diffusion equation.
 
 %=======================================================================
 \sectpc[Section21]{State variables and kinematics}
 \label{sec:basic_def3}
 %=======================================================================
 
In the context of the one-dimensional bar treated in the previous example, we now consider an elastoplastic deformation process occurring in a time interval $\mathbb{T}:=[0,T]$. In particular, at material points $x\in\mathcal{B}$ and time $t\in\mathbb{T}$, the BVP solution provides the temperature field $\mathcal{T}:\mathcal{B}\times\mathbb{T} \rightarrow \mathbb{R}$.  To elaborate the corresponding variational formulation, we employ the function spaces for the temperature field
 %
 \begin{equation}\label{space1_e2}
 	\mathcal{W}^{\mathcal{T}}_{\bar{\mathcal{T}}}:=\{ \mathrm{H}^1(\mathcal{B}) \ : \  \mathcal{T}=\bar{\mathcal{T}} \ \ \text{on} \ \  \partial^{\mathcal{T}}_D\mathcal{B} \}.
 \end{equation}
 %
In the present one-dimensional problem, the thermal Dirichlet is set at the beginning and the ending points, the problem includes the following boundary conditions:
 %
\begin{align}\label{BC_heat}
	\mathcal{T}(0,t)=\mathcal{T}_1\qquad\mathcal{T}(L,t)=\mathcal{T}_2 \quad\;\; \forall\; t>0 \;\;\textrm{on}\  \ {\partial^{\mathcal{T}}_ D\mathcal{B}}.
\end{align}
%
along with Neumann boundary conditions 
%
\begin{equation}
	Q\, n = \bar{q} \ \ \textrm{on}\ \ {\partial^{\mathcal{T}}_N\mathcal{B}},
	\label{flu-bcs_e2}
\end{equation}
 %
 where $Q$ is the thermal volume flux and $\bar{q}$ is the thermal transport on the Neumann boundary, where $n=1$ for $x=L$ and $n=-1$ for $x=0$, and $\bar{\mathcal{T}}$ is the imposed temperature on the Dirichlet boundary. Moreover, the heat flux in~\req{flu-bcs_e2} can be described by the negative direction of the thermal heat gradient $\mathcal{T}'$ through Fourier's law of heat conduction as
 \begin{equation}
 	Q =-{\cal{K}}\; \mathcal{T}',
 \end{equation}
 %
here, ${\cal{K}}$ is  the thermal conductivity.
 
 
  %=======================================================================
 \sectpc{Time discretization of the temporal variables}
 \label{sec:time_increment}
 %=======================================================================
 
 In the following, we shortly comments on the time-discretization of the temporal variables for the rate-depenet problems (i.e., Examples 2-3 and 5-7). To do so, let the interval {$\mathbb{T} := ( t_0,T)$} is discretized using the discrete time (loading) points
 %
\begin{equation}
 0 = t_0 < t_1 < \ldots < t_n < t_{n+1} < \ldots < t_N = T,
\end{equation}
 %
 {with the end time value $T>0$.} {The parameter $t\in \mathbb{T}$ denotes for rate-dependent problems due the time, for rate-independent problems an incremental loading parameter.} In the following, to formulate the incremental variational principles, we denote the current time $t:=t_{n+1}>0$ with known fields at $t_n$. In order to advance the solution within a specific time step, we focus on the finite time increment $[t_n,t_{n+1}]$, with
 %
 \begin{equation}
 	\Delta t=t_{n+1}-t_{n}>0,
 	\label{eq:time_interval}
 \end{equation}
 %
 denotes the time step length. 
 
 %=======================================================================
 \sectpc{Strong quantity and variational principles}
 \label{sec:energy_functions3}
 %=======================================================================
%
One-dimensional  diffusion equation with convection can be written as 
%
 \begin{align}\label{PDE_ex2}
 \rho\,c\,\dot{\mathcal{T}}+\kappa\,\mathcal{T}'+Q'=0\quad\quad \text{in}\quad \calB \times \mathbb{T}
 \end{align}
 %
 where $c$ is the heat capacity, $\rho$ is the heat density, ${\cal{K}}$ denotes its conductivity (thermal diffusivity), and $\kappa$ indicates its thermal velocity. The temporal variable is positive ($t\geq 0$) and the spatial variable varies between 0 and $L$ ($0\leq x\leq L$). 
 
 
 Typically, to identify the relative importance between convection and diffusion response in a heat equation, the dimensionless quantity so-called {\'P}eclet number is estimated  by {\'P}e$:=(\kappa\,h)/(2\,{\cal{K}})$ where $h$ is the element size. This value expresses the ratio of convective to diffusive transport in a heat flow problem. 
 
Denoting the test function $\delta \mathcal{T} \in \mathcal{W}^{\mathcal{T}}_{0}$, the heat problem given \req{PDE_ex2} has the following variational form:
 %
 \begin{align}\label{weak-heat}
 \int_{0}^{L}  \rho\, c\, \dot{\mathcal{T}}\delta \mathcal{T} \,dx +  \int_{0}^{L} \kappa \mathcal{T}' \delta \mathcal{T}\,dx+ \int_{0}^{L} \left({\cal{K}}  \mathcal{T}'\right) \cdot \delta \mathcal{T}'\,dx=\left[ {\cal{K}} \mathcal{T}' \delta \mathcal{T}\right]_{0}^{L}.
 \end{align}
%
 The standard variational equation (initiated from Galerkin formulation) for the heat equation including convection and diffusion effects where convection response are dominated compared with diffusion typically leads to unstable results, and thus numerical stabilization has to be used \cite{brooks1982streamline,codina1998comparison}. More specifically, without stabilization techniques some spurious oscillations (or wiggles) which prevent the numerical solution to converge to physical response.
It can be observe that the stronger convective effects leads to the larger oscillations for evolution thermal response versus time.  It is shown for the value {\'P}e$>1$, where convective response is dominated, the solution obtained through standard FEM is failed by spurious oscillations. More specifically, without stabilization techniques some spurious oscillations (or wiggles) which prevent the numerical solution to converge to physical response. Thus, this  non-physical node-to-node oscillations makes the solution of FEM to become unstable \cite{padilla2014numerical,johannesson1998modelling}. 
%
\begin{align}\label{weak-heat1}
	\widetilde{\delta \mathcal{T}}=\delta \mathcal{T}+\beta\frac{h}{2}\delta \mathcal{T}' \WITH 
	\widetilde{\delta \mathcal{T}}'=\delta \mathcal{T}'.
\end{align}
%
here $\beta$ and its optimal value denoted by $\beta_{opt}$ reads:
%
\begin{align}\label{weak-heat2}
	\beta_{opt}:=coth|Pe|-\frac{1}{|Pe|}.
\end{align}
%
Observe that for linear interpolation basis function used for the finite element discrtization, we have:
%
\begin{align}\label{weak-heat21}
	\widetilde{\delta \mathcal{T}}'=\delta \mathcal{T}',
\end{align}
%
so modified weak formulation reads:
%
 \begin{align}\label{weak-heat3}
	\int_{0}^{L}  \rho\, c\, \dot{\mathcal{T}}\widetilde{\delta \mathcal{T}} \,dx +  \int_{0}^{L} \kappa \mathcal{T}' \widetilde{\delta \mathcal{T}}\,dx
	+ \int_{0}^{L} \left({\cal{K}}  \mathcal{T}'\right) \cdot\widetilde{\delta \mathcal{T}}'\,dx
	=\left[ {\cal{K}} \mathcal{T}' \widetilde{\delta \mathcal{T}}\right]_{0}^{L}.
\end{align}
%
This variational equation typically refers to the Streamline-Upwind (SU) formulation.
%
\begin{table}[!b]
	\caption{Different version of the $\omega$-algorithmic based on different weight function ${\cal{G}}(t)$ \cite{johannesson1998modelling,zienkiewicz2005finite}.}
		\vspace{1mm}
	\centering
	\begin{tabular}{|l c c l|}
		\hline
		Scheme \hspace{2cm} &\quad Weight function ${\cal{G}}(\Delta t)$ \quad&~ $\omega$ \qquad&  Stability condition \\
		\hline\hline
		Explicit & $\delta(t-t_i);\,t_i=0$ & 0 & conditional \\[2mm]
		Crank-Nicolson & 1 & 0.5 & unconditional \\[2mm]
		Galerkin type 2 & $t/\Delta t$ & 0.666 & unconditional \\[2mm]
		Liniger  & $\delta(t-t_i);\,t_i=0.878\Delta t$&0.878 & unconditional \\[2mm]
		Implicit &  $\delta(t-t_i);\,t_i=\Delta t$  & 1 & unconditional \\[1mm]
		\hline
	\end{tabular}\label{omega}
\end{table}





 


% 
An algorithm for the update of the temperature field $\mathcal{T}$ in the increment $[t_n,t_{n+1}]$ results in a time-discrete field variables in incremental setting of the convection-diffusion equation. To do so, \req{weak-heat31} becomes:
%
\begin{align}\label{weak-heat31}
	\int_{0}^{L}  \rho\, c\, \dot{\mathcal{T}}\widetilde{\delta \mathcal{T}} \,dx 
	+  \int_{0}^{L} \left(\kappa \mathcal{T}'\right)^{\omega} \widetilde{\delta \mathcal{T}}\,dx
	+ \int_{0}^{L} \left({\cal{K}}  \mathcal{T}'\right)^{\omega} \cdot\widetilde{\delta \mathcal{T}}'\,dx
	=\left[ {\cal{K}} \mathcal{T}' \widetilde{\delta \mathcal{T}}\right]_{0}^{L}.
\end{align}
%
in terms of the $\omega$-algorithmic expressions by
%
\begin{equation}
	\dot{\mathcal{T}}=\frac{1}{\Delta t}(\mathcal{T}-\mathcal{T}_n) \AND (\bullet)^{\omega}=(1-\omega)(\bullet)_n+\omega(\bullet),
\end{equation}
%
with 
%
\begin{equation}
	\omega:=\frac{\displaystyle\int_{t_n}^{t_{n+1}}{\cal{G}}(t)t/\Delta t\;dt}{\displaystyle\int_{t_n}^{t_{n+1}}{\cal{G}}(t)\;dt},
\end{equation}
%
such that ${\cal{G}}(t)$ is a temporal weighting function. The scalar value $\omega$ for different variation of  ${\cal{G}}(t)$ is given in Table \ref{omega}.

 Regarding the analytical solution, we will consider $\mathcal{T}_1=1\;^{\circ}\text{C}$ and $\mathcal{T}_2=0\;^{\circ}\text{C}$ in \req{BC_heat}, thus the solution has the following form:
 \begin{align}\label{analytic_sol_heat}
\mathcal{T}(t,x)=\exp\bigg(\frac{\kappa}{2\mathcal{K}} x-\frac{K^2\,t}{4\mathcal{K} \rho c}\bigg)\sum_{i=1}^{\infty} \sqrt{2}\,\sin(i \pi x)\,\exp\bigg(\frac{-\mathcal{K}(i\pi)^2\,t }{\rho c}\bigg)\,k_i +\frac{1-\exp\bigg(\dfrac{\kappa}{\mathcal{K}} \left(x-1\right)\bigg)}{1-\exp\bigg(-\dfrac{\kappa}{\mathcal{K}}\bigg)}
 \end{align}
 where 
 \begin{align}
 k_i=-\frac{(-1)^i\,4\sqrt{2} \mathcal{K}^2\,i\pi \sqrt{\mathcal{K}} \exp(-\frac{\kappa}{2\mathcal{K}})}{\kappa^2+4\mathcal{K}^2\,(i\pi)^2\mathcal{K}}.
 \end{align}
 The reader is referred to \cite{guerrero2009analytical} for the details. 
 
 
 
 
 
 

 

 
 
 \begin{form}[\textsc{F2}: Bayesian inversion for convection-diffusion]
 	\label{form_21}
 	Consider an open bounded one-dimensional bar on an interval $\calB:=[0,L]$ with boundary $\partial \calB$ defined at $x=0$ and $x=L$.
 	Let constants $(\kappa,\mathcal{K},\rho,c) \geq 0$  be given with the initial conditions $\mathcal{T}_0= \mathcal{T}({x},0)$. For the loading increments $n=1,2,\ldots, N$, find $ \mathcal{T}:=\mathcal{T}^n\in\mathrm{H}^1_0(\mathcal{B})$ satisfying the following Euler-Lagrange equation in weak form:		 
%
\begin{equation*}
	\begin{aligned}
		\calE_\mathcal{T}(\mathcal{T};\delta \mathcal{T})=
		\int_{0}^{L}  \rho\, c\, {(\mathcal{T}-\mathcal{T}_n)}\widetilde{\delta \mathcal{T}} \,dx 
		&+  \int_{0}^{L} (1-\omega)\Delta t\kappa \mathcal{T}'_n \widetilde{\delta \mathcal{T}}\,dx
		+ \int_{0}^{L} (1-\omega)\Delta t\mathcal{K}  \mathcal{T}'_n \cdot\widetilde{\delta \mathcal{T}}'\,dx\\
		&+  \int_{0}^{L} (\omega)\Delta t\kappa \mathcal{T}' \widetilde{\delta \mathcal{T}}\,dx
		+ \int_{0}^{L} (\omega)\Delta t\mathcal{K}  \mathcal{T}' \cdot\widetilde{\delta \mathcal{T}}'\,dx\\
		&-\left[ \Delta t\mathcal{K} \mathcal{T}' \widetilde{\delta \mathcal{T}}\right]_{0}^{L}=0.
		\hspace{3.7cm}\forall \, \delta \mathcal{T} \in \mathcal{W}^{\mathcal{T}}_{0} 
	\end{aligned}
\end{equation*}
%
 	The unknown material parameters then follow from the probabilistic Bayesian inversion
 	\begin{equation*}
 		\BfrakP\leftarrow\textsc{BI}\big(\textsc{F2}(\Bfraku)\big) \WITH
 		\Bfraku:=\mathcal{T} 
 		\AND
 		\BfrakP:=(\kappa,\mathcal{K}) .
 	\end{equation*}
 \end{form}
 
 \begin{figure}[!t]
 	\centering
 	{\includegraphics[clip,trim=1cm 12cm 1cm 15cm, width=15cm]{Figures/geoF.pdf}}  %left, bottom, right and top
 	\caption{ Geometry and loading setup for the one-dimensional bar. (a) Example 3,4,7 (b) Example 2, and (c) Example 6.}
 	\label{Fig_Ch_geoF}
 \end{figure}

 %=======================================================================
 \sectpc{Bayesian inference}
 %=======================================================================
 
 
 For the simulation, let the bar of unitary length L = 1 with $x\in\calB:=[0,1]$ is isolated form right-edge , i.e., $x=1$ with a prescribed temperature from the left-end, i.e., $x=0$, see Figure \ref{Fig_Ch_geoF}b.  Temperature boundary conditions are set according to \req{BC_heat} such that $\mathcal{T}_1=1\;^{\circ}\text{C}$ and $\mathcal{T}_2=0\;^{\circ}\text{C}$. Additionally, we set initial temperature as ${\cal{T}}=0$ at $t=0$. The reference simulation is performed for $t=0.2$ s. 
 
 The Bayesian inversion aims to determine two thermal parameters, namely ($\kappa$, $\mathcal{K}$). We set $c=1.2\,\text{J/K}$ and $\rho=1.6 \,\mathrm{W/m^{2}}$. We use the online MATLAB codes presented in \cite{schiren2018finite}. We assume $\kappa$ is between 5 $\mathrm{m/s}$ and 20 $\mathrm{m/s}$ and $\mathcal{K}$ varying from 0.5 $\mathrm{W/mK}$ to 2 $\mathrm{W/mK}$ uniformly. The script $\texttt{heat{\_}1D}$ and has a comparison between all methods considering a two-dimensional Bayesian inversion (simultaneous interference of $\kappa$ and $\mathcal{K}$). Finally, we set $\theta^0=(1.2,15)$ and $\sigma^2=0.05$. In order to provide a reference observation, we use $\mathcal{K}=0.9$ and $\kappa=15$, which can be found at $\texttt{reference.mat}$. 

 \begin{figure}[!t]
 	\centering
 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/MH_chi}} 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/AM_chi}}
 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/DR_chi}}\\ 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/DRAM_chi}}
 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/EnKF_chi}}
 	\caption{Example 2. The MCMC chain of $\mathcal{K}$ obtained by different Bayesian techniques. Form left to right: MH, AM, and DR (the first row), and DRAM as well as EnKF (the second row). }
 	\label{MCMC21}
 \end{figure}
 
 \begin{figure}[!t]
 	\centering
 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/MH_kappa}} 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/AM_kappa}}
 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/DR_kappa}}\\ 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/DRAM_kappa}}
 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/heat/EnKF_kappa}}
 	\caption{Example 2. The MCMC chain of $\kappa$ obtained by different Bayesian techniques. Form left to right: MH, AM, and DR (the first row), and DRAM as well as EnKF (the second row).
 	}
 	\label{MCMC22}
 \end{figure}
 
  \begin{figure}[!t]
  	\centering
  	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/heat/pdf_eta}} 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/heat/pdf_kappa}}
  	\caption{Example 2. The posterior distribution of $\mathcal{K}$ (left) and $\kappa$ (right) obtained by different Bayesian techniques. The true values are shown with a black dashed line.
  	}
  	\label{pdf2}
  \end{figure}

 \begin{figure}[!t]
	\centering
	\includegraphics[width=0.7\textwidth]{Figures/heat/temp.jpg}
	\caption{Solution of the heat equation in Example 2 using the inferred values at $t=0.2$.}
	\label{hear3}
\end{figure}



 We plot the evolution of the MCMC chain of $\mathcal{K}$ and $\kappa$ as shown respectively in Figure \ref{MCMC21} and Figure \ref{MCMC22}. MH shows a significant uncertainty in both parameters. However, EnKF and DRAM estimated $\mathcal{K}$ and $\kappa$ with a low fluctuation. Figure \ref{pdf2} depicts a comparison between the posterior density using all MCMC techniques. As shown, the MH method failed to estimate the parameters effectively since a wide distribution is obtained, and the estimated values are relatively far from the true values. The proposal adaptation enhanced Metropolis-Hastings; however, the results are similar to a bimodal distribution. The local adaptation (DR) gives rise to a better inference and the peak point of both distributions located exactly at the true values. EnKF and DRAM showed an excellent performance. 
 
 \begin{table}[!]
 	\caption{Example 2: The median of the posterior density of $\cal{K}$ and $\kappa$ as well as the elapsed CPU time and the acceptance rate using different MCMC methods}
 	\vspace{1mm}
 	\centering
 	\begin{tabular}{|l c c c c c|}
 		\hline
	method \hspace{8cm}&MH        & AM    &   DR   &   DRAM   &~~~EnKF~~~      \\\hline\hline
$\mathcal{K}$ \hspace{2cm}  &~~~0.878~~~   & ~~~0.879~~~  & ~~~0.912~~~ &~~~0.902~~~ & ~~~0.896~~~ \\[4mm]
$\kappa$ \hspace{2cm}  &~~~14.91~~~   & ~~~14.8~~~  & ~~~15.14~~~ &~~~15.01~~~ & ~~~14.98~~~ \\[4mm]
CPU time [s]\hspace{2cm}  & 12.61   & 14  & 28.05 &22.01 &  27\\[4mm]
acceptance rate (\%) &   4.5  &  5.8  &  10.9 & 9 &72.5   \\[2mm]
 		\hline
 	\end{tabular}\label{comp2}
 \end{table}





 
 The computational features of the methods are listed in Table \ref{comp2}. The median of the posterior densities of all methods are close to the true values. Here, MH and AM have a low (less than 10\%) acceptance rate and EnKF has an excellent ratio.
   Finally, the evolution of the temperature using the estimated parameters from DRAM and EnKF is shown in Figure \ref{hear3}. The results are compared with the analytical solution (using true values), where a very good agreement is achieved.
 
 
 %============================================================ 
 %=======================================================================

  
%
%=======================================================================
\sectpb[Example3]{Example 3: Elastoplasticity}\label{Ex3}
%=======================================================================

As a third example, we apply Bayesian inversion to a one-dimensional elastoplasticity problem. Herein, the goal is to estimate Young's modulus $E$, in addition to the material parameters characterizing the elastoplastic response, namely, the plastic yield strength $\sigma_Y$ and the hardening modulus $H$. Moreover, due to the dissipative nature of the problem, time evolution is now explicitly considered \cite{de2011computational,wriggers2008nonlinear}. 
 
 %=======================================================================
 \sectpc[Section21]{State variables and kinematics}
 \label{sec:basic_def2}
 %=======================================================================
 
In the context of the one-dimensional bar treated in the previous example, we now consider an elastoplastic deformation process occurring in a time interval $\mathbb{T}:=[0,T]$. The strain defined in~\eqref{small_strain} is additively decomposed into an elastic part $\varepsilon^e$ and a plastic part $\varepsilon^p$:
%
\begin{equation}
	\varepsilon(x,t) = \varepsilon^e(x,t) + \varepsilon^p(x,t).
	\label{s2-strain-e-p}
\end{equation}
%
The plastic strain $\varepsilon^p:\mathcal{B}\times\mathbb{T}\rightarrow\mathbb{R}$ is considered as a local internal variable. Moreover, to account for phenomenological hardening effects, a hardening variable $\alpha:\mathcal{B}\times\mathbb{T}\rightarrow\mathbb{R}_+$ is introduced as a second local internal variable. For simplicity, $\alpha$ is assumed to coincide with the equivalent plastic strain, such that 
%
\begin{equation}
	\dot\alpha(x,t) = \vert \dot{\varepsilon}^p(x,t) \vert.
	\label{s2-evol-alpha}
\end{equation}
%
The hardening variable starts to evolve from the initial condition $\alpha(x,0) = {\color{red}\mathit{0}}$. The elastoplastic response of the bar is thus characterized by the displacement field $u$, the plastic strain $\varepsilon^p$, and the hardening variable $\alpha$. 

%Hence, the constitutive approach focuses on the set
%%
%\begin{equation}
%	\mbox{Constitutive State Variables}\, 
%	\BfrakP := \{ \varepsilon, \varepsilon^p, \alpha \}.
%	\label{state}
%\end{equation}

 %=======================================================================
\sectpc{Energy quantities and variational principles}
\label{sec:energy_functions2}
%=======================================================================

Let us define the following pseudo-energy density per unit volume:
%
\begin{equation}
	{W}(\varepsilon,\varepsilon^p,\alpha) := 
	{W}_{elas}(\varepsilon,\varepsilon^p) + {W}_{plas}(\alpha).
	\label{pseudo-energy}
\end{equation}
%
The {elastic contribution} is assumed to have the simple quadratic form
\begin{equation}
	{W}_{elas}(u,\varepsilon^p):= \frac{1}{2}E(\varepsilon-\varepsilon^p)^2.
	\label{elas-part}
\end{equation}
Accordingly, the {\it plastic contribution} in \req{pseudo-energy} is assumed to have the form
\begin{equation}
	{W}_{plas}(\alpha) := \sigma_y \alpha + \frac{H}{2} \alpha^2,
	\label{plas-part}
\end{equation}
%
with the initial yield stress $\sigma_Y\ge$ and the isotropic hardening modulus $H\ge 0$. Note that $W_{elas}$ can be viewed as a stored energy density, while $W_{plas}$ can be viewed as a dissipated energy density, defined here as a state function.

From the strain energy density, the constitutive stress-strain relation and the generalized stress follow as
%
\begin{equation}
\sigma=\frac{\partial W_{elas}}{\partial \varepsilon}=E(\varepsilon-\varepsilon^p) \AND s^p=-\frac{\partial W_{elas}}{\partial \varepsilon^p}\equiv\sigma.
\label{stress_pals}
\end{equation}

The elastoplasticity model additionally requires evolution equations for the plastic strain. To this end, the yield function is first defined in terms of the generalized stress $s^p$ and the resisting force $R^p$ as
%
\begin{equation}
\beta:=\vert s^p \vert - R^p \WITH
	R^p:=R^p(\alpha)= \frac{\partial {W}_{plas}}{\partial \alpha}  .
\end{equation}
%
With the yield function at hand, an associative flow rule is adopted for the plastic strain, such that
%
\begin{equation}
\dot{\varepsilon}^p=\lambda^p\partial_{s^p}\beta=\lambda^p\mathrm{sign}(s^p),
\label{flow2}
\end{equation}
%
where $\lambda^p\ge0$ is the plastic multiplier. The flow rule is complemented with the set of Kuhn-Tucker conditions 
%
\begin{equation}
	\beta \le 0 , \quad\quad \lambda^p \ge 0, 
	\quad\quad \mbox{and} \quad\quad
	\beta\; \lambda^p = 0 .
\label{kkt2}
\end{equation}

To derive the weak form of the evolution problem, the total energy functional for the elastoplasticity model is defined as
%
\begin{equation}\label{1D2}
\begin{aligned}
\mathcal{E}(u,\varepsilon^p,\alpha)=\int^{L}_{0} A \big[ {W}_{elas}(u,\varepsilon^p)+{W}_{plas}(\alpha) \big ]\,
\mathrm{d}{{x}}
-\int^{L}_{0} \rho A{ {\bar b}}  u\,\mathrm{d}x
- A \bar{t} u \, \big|_{\partial_N\mathcal{B}}  .
\end{aligned}
\end{equation}
%
Minimization of the energy functional~\eqref{1D1} with respect to the displacement field leads to the following weak formulation.

\begin{form}[\textsc{F3}: Bayesian inversion for elastoplasticity]
	\label{form_2}
	Consider an open bounded one-dimensional bar on an interval $\calB:=[0,L]$ with boundary $\partial \calB$ defined at $x=0$ and $x=L$.
	Let constants $(E$ $,H,\sigma_Y) \geq 0$  be given with the initial conditions $u_0= u({x},0)$ and $\varepsilon^p=\alpha({x},0)$. For the loading increments $n=1,2,\ldots, N$, find $ u:=u^n\in\mathrm{H}^1_0(\mathcal{B})$ satisfying the following Euler-Lagrange equation in weak form:		 
	\begin{align*}
	\calE_u(u,\Bve^p,\alpha;\delta u)=\int^L_{0}\big[A\sigma\big(\varepsilon(u),\varepsilon^p\big)\varepsilon(\delta u)-\rho A \bar{b} \delta u\big]\,dv  - A \bar{t} \delta u \, \big|_{\partial_N\mathcal{B}} = 0 \quad \forall \, \delta u \in \mathrm{H}_0^1(\mathcal{B})  ,
    \end{align*}
    %        \tag{\text{EP}}
    where $\varepsilon^p(x,t)$  evolves according to the evolution equations~\eqref{flow2} and~\eqref{kkt2}, while $\alpha(x,t)$ evolves according to the hardening law~\eqref{s2-evol-alpha}. 
    The unknown material parameters then follow from the probabilistic Bayesian inversion
    \begin{equation*}
    	\BfrakP\leftarrow\textsc{BI}\big(\textsc{F3}(\Bfraku)\big) \WITH
    	\Bfraku:=(u,\varepsilon^p,\alpha) 
    	\AND
    	\BfrakP:=(E,H,\sigma_Y) .
    \end{equation*}
\end{form}

One can show that the evolution equations~\eqref{s2-evol-alpha}, \eqref{flow2} and~\eqref{kkt2}, which completely determine the evolution of the plasticity variables $(\varepsilon^p,\alpha)$, can also be obtained in weak from through minimization of the energy functional~\eqref{1D2} with respect to $(\varepsilon^p,\alpha)$. Due to the local nature of the plasticity variables in the present example, only the weak form of the mechanical balance equation is included in Formulation~\ref{form_2}.

%=======================================================================
\sectpc{Bayesian inference}
\label{sec:bayesian2}
%=======================================================================

%Let the bar, of unitary length L = 1 with $x\in\calB:=[0,1]$ that is initially unstretched, and undamaged. Its left-end is fixed, i.e., $x=0$, while on its right-end, i.e., $x=1$, a monotonic displacement increment  $u=5\times10^{-4}$ mm is applied for 155 time steps, see Figure \ref{label}. The minimum finite element size in the domain $\calB$ is $h=0.005$ mm.  
 

In this numerical example, let the bar, of unitary length L = 1 with $x\in\calB:=[0,1]$ that is initially unstretched. Its left-end is fixed, i.e., $x=0$, while on its right-end, i.e., $x=1$, a monotonic displacement increment  $\Delta \bar{u}=1\times10^{-5}$ mm is applied for 151 time steps, see Figure \ref{Fig_Ch_geoF}a. We set $(\alpha,\varepsilon^p)=(0,0)$ at $t=0$. Regarding the finite element mesh size, 100 elements are used.  The main script is \texttt{EP\_1D.m} and the code \texttt{forwardmodel.m} computes the solution with respect to the candidates.

This problem is a good example to compare EnKF-MCMC and DRAM. The unknown ranges are mentioned in Table \ref{range2}. The true values are used to produce the reference observation (\texttt{reference.mat}). We use $\theta^0=(E^0,\,H^0,\,\sigma_Y^0) =(60\,000,\,200,\,300)$.
As Figure \ref{EP1} shows, the estimated chains by the DRAM algorithm have a low uncertainty for $E$ and $\sigma_Y$; however, the variation of $H$ is notable. On the other hand, the fluctuation of all unknowns in EnKF is negligible. Of course, it is an important advantage of using the Kalman filter compared to DRAM. The posterior densities verify this statement, where a wide distribution is achieved for $H$. For the yield stress, both methods performed similarly and have a relatively same distribution. Also, the acceptance rate of EnKF is 98.4\% and DRAM is 6.9\%. The medians are summarized in Table \ref{range2}, indicating the accuracy of both techniques (the is an excellent agreement between the simulations and the true values). In total, due to the higher acceptance ratio and significantly lower uncertainty (specifically of hardening), we conclude that EnKF is more suitable for the elastoplasticity example.
 Finally, we use the estimated values of EnKF and DRAM to plot the load-displacement curve during different time-steps, see Figure \ref{EP3}.
 
  \begin{table}[!]
  	\caption{Example 3. The computational features and the results of the Bayesian inversion.}
  	\vspace{1mm}
  	\centering
  	\begin{tabular}{|llcc|}
  		\hline
  		Parameter   &   $   E\,[\text{MPa}] \qquad      $    &   $\qquad H\,[\text{MPa}]\qquad $ &   $\qquad \sigma_Y\,[\text{MPa}]\qquad $         \\\hline\hline
  		 $\mathrm{min}$    &30\,000   & 200  &  200 \\[4mm]
  		  $\mathrm{max}$   &100\,000  &  400  &  400   \\[4mm]
  		 $\mathrm{DRAM}$\qquad\qquad   &   71\,201  &  251  &  350   \\[4mm]
  		 $\mathrm{EnKF}$\qquad\qquad   &   71\,300  &  250  &  350   \\[4mm]
  		 $\mathrm{true~value}$\qquad\qquad   &   71\,300  &  250  &  350   \\[2mm]
  		\hline
  	\end{tabular}\label{range2}
  \end{table}
 
 
 

 
 
 
 
 
 \begin{figure}[!t]
 	\centering
 	 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/EP/MCMC_E}} 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/EP/MCMC_H}}
 	 	\subfloat{\includegraphics[width=0.33\textwidth]{Figures/EP/MCMC_sigma}}\\\hspace{-0.3cm}
 	 		\subfloat{\includegraphics[width=0.33\textwidth]{Figures/EP/post_E}} 	\subfloat{\includegraphics[width=0.326\textwidth]{Figures/EP/post_H}}
 	 		\subfloat{\includegraphics[width=0.33\textwidth]{Figures/EP/post_sigma}}
 	 		\vspace{0.2cm}
 	\caption{Example 4. The evolution of the MCMC chains obtained by DRAM and EnKF for $E$, $H$, and $\sigma_Y$ (the first row) and the corresponding pdf (the second row). The true values are shown with green dashed lines. 
 	}
 	\label{EP1}
 \end{figure}
 
 
   \begin{figure}[!t]
   	\centering
   	\includegraphics[width=0.7\textwidth]{Figures/EP/EP}
   	\caption{Load-displacement curve for the elastoplasticity problem in Example 3, obtained using the inferred values. 
   	}
   	\label{EP3}
   \end{figure}
 
In order to implement the Bayesian inversion, we require the available range for the parameters (the prior density), for which we adopt the uniform distribution summarized in Table \ref{range2}. As previously discussed, both DRAM and EnKF-MCMC methods perform  efficiently, i.e., lead to fast convergence. For this example, we employed the DRAM algorithm. Figure~\ref{EP1} depicts posterior density using 8\,000 samples. All parameters converged rapidly to the true values. This is validated in detail in Figure~\ref{EP1}, where all mechanical parameters show fast convergence. The uncertainty of the parameters is not high.
The inferred values were used to estimate the load-displacement curve shown in Figure \ref{EP3}. 
 
 %
%=======================================================================
 

  

  

 
%======================================================================= 
\sectpb[Example4]{Example 4: Phase-field fracture for brittle materials}\label{Ex4}
%======================================================================= 

The fourth example addresses the variational phase-field modeling of brittle fracture. Starting with the work of~\cite{francfort1998revisiting,bourdin2000numerical} and the subsequent developments~\cite{amor2009,freddi2010regularized,hakim2009,kuhn2010,miehe+welschinger+hofacker10a,pham2011,borden2012}, this framework has gained significant popularity in the past decade due to its ability to naturally handle the complex behavior of fracturing solids. We refer the reader to~\cite{ambati2015review} for an overview of initial contributions.

Bayesian inversion framework was applied to the phase-field modeling of brittle fracture in~\cite{khodadadian2020bayesian}.  In the present illustrative example, we consider the one-dimensional setting, where the objective is to estimate Young's modulus $E$ and the fracture toughness $G_c$ for a fixed length scale parameter (although the length scale can also be estimated). 
 


  
 %=======================================================================
 \sectpc[Section21]{State variables and kinematics}
 \label{sec:basic_def4}
 %=======================================================================
 
The response of a fracturing solid obeying a brittle phase-field model is governed by a two-field system of PDEs. In particular, at material points $x\in\mathcal{B}$ and time $t\in\mathbb{T}$, the solution of the coupled system provides the displacement field $u:\mathcal{B} \times \mathbb{T} \rightarrow \mathbb{R}$ and the phase-field fracture variable $d:\mathcal{B} \times \mathbb{T} \rightarrow [0,1]$. 
%As such, the global primary fields are given by
% %
% \begin{equation}
% 	u: 
% 	\left\{
% 	\begin{array}{ll}
% 		\mathcal{B} \times \mathbb{T} \rightarrow \mathbb{R} \\
% 		(x, t)  \mapsto u(x,t)
% 	\end{array}
% 	\right.
% 	,\quad \
% 	d: 
% 	\left\{
% 	\begin{array}{ll}
% 		\mathcal{B} \times \mathbb{T} \rightarrow [0,1] \\
% 		(x, t)  \mapsto d(x,t)
% 	\end{array}.
% 	\right.
% 	%\WITH
% 	%\dot{d} \ge 0
% 	\label{primary_4}
% \end{equation}
% %
Here, $d(x,t)=0$ and $d(x,t)=1$ characterize an undamaged and a completely fractured material point, respectively. 
With the purpose of stating variational principles, we introduce the function spaces
%\theta=\bar{\theta} \; \mathrm{on} \; \partial^{\theta}_D\mathcal{B}
 \begin{equation}\label{space1}
 \begin{aligned}
 		\mathcal{W}^{u}_{\bar{u}}:= \{ \mathrm{H}^1(\mathcal{B}) \ : \ u=\bar{u}  \ \ \text{on} \ \ {\partial_D\mathcal{B}} \}, \quad
 		\mathcal{W}^{d}_{d_n}:= \{ d \in \mathrm{H}^1(\mathcal{B}) \ : \ d \geq d_n \}.
 \end{aligned}
 \end{equation}
%
% \begin{equation}\label{space1}
% 	\begin{aligned}
% 		\mathcal{W}^{u}_{\bar{u}}&:= \{ \mathrm{H}^1(\mathcal{B}) \ : \ u=\bar{u} \ \text{at} \ x=L  \}, \quad\\ 
% 		\mathcal{W}^{d}&:= \mathrm{H}^1(\mathcal{B}) , \AND
% 		\mathcal{W}^{d}_{d_n} := \{ d \in \mathrm{H}^1(\mathcal{B}) \ : \ d \geq d_n \}.
% 	\end{aligned}
% \end{equation}
 %
Here, ${\partial_D\mathcal{B}}\equiv\{0,L\}$ denotes the Dirichlet boundary, with $\bar{u}(0,t)=0$. On the other hand, $\mathcal{W}^{d}_{d_n}$ is a non-empty, closed, and convex subset of  $\mathrm{H}^1(\mathcal{B})$. This function space introduces the evolutionary character of the phase-field, incorporating an irreversibility condition in incremental form, where $d_n$ is the damage value at a previous time instant.
 
 %=======================================================================
 \sectpc{Energy quantities and variational principles}
 \label{sec:energy_functions4}
 %=======================================================================
 
The energy density per unit volume in the present model is additively decomposed into stored elastic strain energy and crack-surface dissipated energy. In particular, one has
%
\begin{equation}
	{W}(\varepsilon,d) := 
	{W}_{elas}(\varepsilon,d) + {W}_{frac}(d,d').
	\label{pseudo-energy_4}
\end{equation}
%
The {elastic contribution} is assumed to have the simple quadratic form
%
\begin{equation}
	{W}_{elas}(u,d):=\frac{1}{2}g(d)E\varepsilon^2,
	\label{elas-part4}
\end{equation}
%
where $g(d)$ is a degradation function for which the usual quadratic form
%
\begin{equation}
g(d):=(1-d)^2,
\label{quad_deg}
\end{equation}
%
is adopted. On the other hand, the fracture contribution represents the regularized crack-surface energy density, expressed in terms of the current damage state as well as its spatial gradient, and modulated by a length scale parameter. In particular, we adopt the so-called AT-2 version of the formulation~\cite{marigo2016}, where
%
\begin{equation}
	{W}_{frac}(d,d') := G_c\bigg(\frac{d^2}{2l_f} + \frac{l_f}{2}d'^2\bigg).
	\label{frac-part}
\end{equation}
%
 In~\eqref{frac-part}, $G_c>0$ is the fracture toughness (more specifically, Griffith's critical energy release rate) and $l_f>0$ is the fracture length scale parameter that governs the regularization. 

With the above definitions, a global energy functional is defined as
%
\begin{equation}\label{1D4}
\begin{aligned}
\mathcal{E}(u,d)=\int^{L}_{0} A \big[ {W}_{elas}(u,d)+{W}_{frac}(d,d') \big ]\,
\mathrm{d}{{x}}  .
\end{aligned}
\end{equation}
%
Minimization of the energy functional~\eqref{1D4} with respect to the displacement field and the crack phase-field leads to the following weak formulation.

\begin{form}[\textsc{F4}: Bayesian inversion for phase-field brittle fracture]
	\label{form_4}
	Consider an open bounded one-dimensional bar on an interval $\calB:=[0,L]$ with boundary $\partial \calB$ defined at $x=0$ and $x=L$.
	Let constants $(E$ $,G_c,l_f) \geq 0$  be given with the initial conditions $u_0= u(x,0)$ and  $d_0=d({x},0)$. For the loading increments $n=1,2,\ldots, N$, find $ u:=u^n\in \mathcal{W}^u_{\bar{u}}$ and $d:=d^n\in \mathcal{W}^d_{d_{n-1}}$ satisfying the following Euler-Lagrange equations in weak form:	 
	\begin{equation*}
	\left\{
	\begin{aligned}
		%========================	
		&\calE_u(u,d;\delta u)=\int^L_{0}(1-d)^2 E\varepsilon(u)\varepsilon(\delta u)\,\mathrm{d}x =0 \quad \forall \,\delta u\in\mathcal{W}^u_0 ,%\
		%\hspace{3.18cm} \emph{(E)}	
		\\
		%\tag{E}\\
		%========================
		&\calE_d(u,d;\delta d)=
		\int^L_{0} \Big[-(1-d)E\varepsilon(u)^2\delta d + \frac{G_c}{l_f}d\,\delta d + l_f d'(\delta d)'\Big]\,\mathrm{d}x \geq 0 \quad \forall \,\delta d \in \mathcal{W}^d_{0}  .
		%\hspace{0.1cm} \emph{(D)}	\\
		%========================
	\end{aligned}
    \right.
    \label{weak_4}
    \end{equation*}
The unknown material parameters then follow from the probabilistic Bayesian inversion
\begin{equation*}
	\BfrakP\leftarrow\textsc{BI}\big(\textsc{F4}(\Bfraku)\big) \WITH
	\Bfraku:=(u,d) 
	\AND
	\BfrakP:=(E,G_c) .
\end{equation*}
\end{form}

The inequality in~\eqref{weak_4}$_2$ is a consequence of the irreversibility condition embedded in the constraint $d_{n}\in \mathcal{W}^d_{d_{n-1}}$. To resolve this issue and solve~\eqref{form_4}$_2$ as an equality, the \emph{history field} approach, proposed in~\cite{MieWelHof10b} and widely employed in the phase-field literature, is adopted in this work.

%Accordingly,  the Kuhn-Tucker conditions (KKT) for the gradient damage model reads
%\begin{equation*}
%	\chi^d \le 0 \quad\quad , \quad\quad \lambda^d=\dot d_L\ge 0 
%	\quad\quad \mbox{and} \quad\quad
%	\chi^d\; \lambda^d = 0 .
%	\label{kktD}
%	\tag{KKT$_\text{D}$}	
%\end{equation*}
%%
%such that the so-called damage yield function defined as
%\begin{equation}
%	\chi^d:=- \delta_{d} W\le 0 \WITH 
%	W=W(\nabla u, \nabla \alpha, \alpha, d, \nabla d),
%\end{equation}
%
%%
%Herein, the test functions for displacement field, and crack phase-field are $(w,\psi)$. Also, the following descending functions are used:
%\begin{equation}
%	\begin{aligned}
%		E(d)=h(d)E_0, \WITH  
%		h(d)=(1-d)^2+\kappa.
%	\end{aligned}
%\end{equation}

%=======================================================================
\sectpc{Bayesian inference}
%=======================================================================

In this numerical example, let the bar, of unitary length L = 1 with $x\in\calB:=[0,1]$ that is initially unstretched, and undamaged. Its left-end is fixed, i.e., $x=0$, while on its right-end, i.e., $x=1$, a monotonic displacement increment  $\Delta \bar{u}=1\times10^{-5}$ mm is applied for 151 time steps, see Figure \ref{Fig_Ch_geoF}a. Regarding the finite element mesh size, 300 elements are used. 

  \begin{table}[!]
	\caption{The uniform prior distribution of the inferred parameters in Example 4 (brittle fracture) including the true values.}
	\vspace{1mm}
	\centering
	\begin{tabular}{|llc|}
		\hline
		Parameter  &$ E\,[\text{MPa}]\quad$        &  $\quad G_c\,[\text{MPa}]\quad$          \\\hline\hline
		$\mathrm{min}$    &30\,000   & 0.02    \\[4mm]
		$\mathrm{max}$ &  100\,000  &  0.03      \\[4mm]
		$\mathrm{true~value}$\qquad\qquad  &   70\,500  &  0.027     \\[4mm]
		$\mathrm{EnKF}$\qquad\qquad  &   70\,493  &  0.027     \\[2mm]
		\hline
	\end{tabular}\label{range4}
\end{table}

We use a two-dimensional Bayesian inversion to identify ($E$, $G_c$). The reference solution is a $1\times151$ vector estimated by $E=70\,500\,\text{MPa}$ and $G_c=0.027$\,kN/mm{$^2$} (the true values).
 As the initial guess, we se $\theta^0=(60\,000,0.025)$. The script name $\texttt{brittle\_1D.m}$. The parameters range are mentioned in Table \ref{range4}. 
Using EnKF-MCMC with 1\,000 iterations leads to the estimation of MCMC and also the posterior density. Figure \ref{bri1} depicts the MCMC evolution for both parameters. A narrow posterior density for both unknowns points out the low uncertainty and fast convergence employing EnKF-MCMC. The acceptance ratio of the chain is 12.2\%. The estimated medians are $E=70493$ and $E=0.027$, which the method efficiency. Finally, we use these values to estimate the load-displacement curve, and the results are shown in Figure \ref{bri3}.

 
  \begin{figure}[!t]
 	%\centering
 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/brittle/MCMC_E}} 
 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/brittle/MCMC_Gc}}\\
 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/brittle/pdf_E}} 
 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/brittle/pdf_Gc}}
 	\vspace{0.4cm}  
 	\vspace{-0.4cm}
 	\caption{Example 4. The posterior densities of different parameters estimated by EnKF method. The true values are shown with green dashed lines. 
 	}
 	\label{bri1}
 \end{figure}
  
 \TODO{(Amir) Add Table for Example 4}

%=======================================================================
\sectpb[Example5]{Example 5: Phase-field fracture for gradient-extended ductile materials }\label{Ex5}
%=======================================================================

In this example, the phase-field model for brittle fracture explored above is extended to the ductile case. To this end, the evolution of the phase-field variable is coupled to elastoplasticity, allowing for the initiation and propagation of ductile cracks. Initial works on this topic include~\citep{alessi2015,du2015,ambati2015,miehe+hofacker+schaenzel+aldakheel15,borden2016,ulloa2016,kuhn2016} (see~\cite{alessi2018comparison,noii2021bayesian} for an overview). Moreover, to achieve a regularized plastic response, the extension to gradient-extended plasticity~\cite{miehe+hofacker+schaenzel+aldakheel15,aldakheel16,miehe2016aphase,rodriguez2018} is considered, which has shown to ensure mesh-objective and physically meaningful responses in the post-critical stage. 

The present Bayesian inversion framework was applied to the phase-field modeling of ductile fracture in our recent work~\cite{noii2021bayesian}, where three dimensional simulations were performed and compared to experimental observations. Herein, we present an illustrative one-dimensional example, where the objective is to estimate the parameters involved in both the elatoplasticity example (Section~\ref{Ex2}) and the brittle fracture example (Section~\ref{Ex4}).

  \begin{figure}[!t]
	\centering
	\includegraphics[width=0.7\textwidth]{Figures/brittle/disp}
	\caption{Load-displacement curve for the brittle phase-field problem in Example 4, estimated by the inferred values. 
	}
	\label{bri3}
\end{figure}

 %=======================================================================
\sectpc[Section21]{State variables and kinematics}
\label{sec:basic_def5}
%=======================================================================

%The response of a fracturing solid obeying the present ductile phase-field model with gradient plasticity is governed by a three-field system of PDEs and the local evolution equation for the plastic strain. In particular, at material points $x\in\mathcal{B}$ and time $t\in\mathbb{T}$, the solution of the coupled system provides the displacement field $u(x,t)$, the phase-field fracture variable $d(x,t)$, and the plastic variables $\varepsilon^p(x,t)$ and $\alpha(x,t)$.  As such, the primary fields are given by
% %
% \begin{equation}
% \begin{aligned}
% 	u: 
% 	\left\{
% 	\begin{array}{ll}
% 		\mathcal{B} \times \mathbb{T} \rightarrow \mathbb{R} \\
% 		(x, t)  \mapsto u(x,t)
% 	\end{array}
% 	\right.
% 	,\quad \
% 	d: 
% 	\left\{
% 	\begin{array}{ll}
% 		\mathcal{B} \times \mathbb{T} \rightarrow [0,1] \\
% 		(x, t)  \mapsto d(x,t)
% 	\end{array}
% 	\right. ,
% 	\label{primary_5_0}
% 	\end{aligned}
% \end{equation}
% %
% along with the plasticity variables
% % 
%  %
% \begin{equation}
% \begin{aligned}
% 	\varepsilon^p 
% 	\left\{
% 	\begin{array}{ll}
% 		\mathcal{B} \times \mathbb{T} \rightarrow \mathbb{R} \\
% 		(x, t)  \mapsto \varepsilon^p(x,t)
% 	\end{array}
% 	\right.
% 	,\quad \
% 	\alpha: 
% 	\left\{
% 	\begin{array}{ll}
% 		\mathcal{B} \times \mathbb{T} \rightarrow \mathbb{R}_+ \\
% 		(x, t)  \mapsto \alpha(x,t)
% 	\end{array}.
% 	\right.
% 	\label{primary_5_1}
% 	\end{aligned}
% \end{equation}
%%
%Recall that the crack phase-field variable and the plasticity variables have  been introduced in sections~\ref{Ex4} and~\ref{Ex2}. 

The response of a fracturing solid obeying the present ductile phase-field model with gradient plasticity is governed by a three-field system of PDEs and a local plastic evolution equation. In particular, at material points $x\in\mathcal{B}$ and time $t\in\mathbb{T}$, the solution of the coupled system provides the displacement field $u:\mathcal{B}\times\mathbb{T}\rightarrow\mathbb{R}$, the phase-field fracture variable $d:\mathcal{B}\times\mathbb{T}\rightarrow[0,1]$ introduced in Section~\ref{Ex4}, and the plasticity variables $\varepsilon^p:\mathcal{B}\times\mathbb{T}\rightarrow\mathbb{R}$ and $\alpha:\mathcal{B}\times\mathbb{T}\rightarrow\mathbb{R}_+$ introduced in Section~\ref{Ex2}. Being a phase-field model, as in Section~\ref{Ex4}, the constitutive state includes the gradient of the crack phase-field $d'(x,t)$. Moreover, in contrast with Section~\ref{Ex2}, we now render the equivalent plastic strain $\alpha$ a non-local internal variable to regularize the plastic response in post-critical stages. As such, the constitutive state further includes the spatial gradient $\alpha'(x,t)$. 

With the purpose of stating variational principles, we consider the function spaces~\eqref{space1} for the displacement field and the crack phase-field, and further introduce the function spaces for the plasticity variables
%
 \begin{equation}\label{space2}
 	\begin{aligned}
 		\mathcal{W}^{p}&:= \mathrm{L}^2(\mathcal{B}), \quad
 		\mathcal{W}^{\alpha}_{\alpha_n,\,q} := \{ \alpha \in \mathrm{H}^1(\mathcal{B}) \ : \ \alpha = \alpha_n + \vert q \vert, \quad q\in \mathcal{W}^{p} \}.
 	\end{aligned}
 \end{equation}
 %
The hardening law~\eqref{s2-evol-alpha} is then enforced in incremental form as $\alpha\in\mathcal{W}^{\alpha}_{\alpha_n,\,\varepsilon^p-\varepsilon^p_n}$.

%=======================================================================
\sectpc{Energy quantities and variational principles}
\label{sec:energy_functions5}
%=======================================================================
 
The energy density per unit volume in the present model is additively decomposed into stored elastic strain energy and the sum of plastic and crack-surface dissipation. In particular, one has
%
\begin{equation}
	{W}(\varepsilon,\varepsilon^p,\alpha,d,\alpha',d') := 
	{W}_{elas}(\varepsilon,\varepsilon^p,d) + {W}_{plas}(\alpha,d,\alpha') + {W}_{frac}(d,d').
	\label{pseudo-energy_5}
\end{equation}
%
In agreement with~\eqref{elas-part} and~\eqref{elas-part4}, the {elastic contribution} reads
%
\begin{equation}
	{W}_{elas}(u,\varepsilon^p,d):=\frac{1}{2}g(d)E(\varepsilon-\varepsilon^p)^2,
	\label{elas-part5}
\end{equation}
%
where $g(d)$ is the quadratic degradation function defined in~\eqref{quad_deg}. The stress-strain relation then reads%
\begin{equation}
\sigma(\varepsilon,\varepsilon^p,d)=\frac{\partial W_{elas}}{\partial \varepsilon}=(1-d)^2E(\varepsilon-\varepsilon^p).
\label{stress_5}
\end{equation}
%
The plasticity contribution is defined as a gradient-extended damaged version of~\eqref{plas-part}:
%
\begin{equation}
	{W}_{plas}(\alpha,d,\alpha') := g(d)\bigg(\sigma_Y \alpha + \frac{1}{2}H \alpha^2 + \frac{1}{2}\sigma_Y\,l_p\,\alpha'^2\bigg),
	\label{plas-part5}
\end{equation}
%
where, for simplicity, and as commonly done in the literature, the same quadratic degradation function~\eqref{quad_deg} is employed to degrade the plastic energy density. Finally, the fracture contribution reads
%
\begin{equation}
	{W}_{frac}(d,d') := w_0 d + \frac{1}{2} w_0 \, l_d^2\, d'^2.
	\label{frac-part5}
\end{equation}
%
Note that, as opposed to~\eqref{frac-part}, the fracture energy density is here defined as a linear function of $d$, representing a so-called AT-1 type formulation, where an elastic stage is included in the deformation process~\cite{miehe+hofacker+schaenzel+aldakheel15,alessi2018comparison}. In~\eqref{frac-part}, $w_0>0$ is a critical fracture energy density, which can be directly related to the fracture toughness in the case of brittle fracture, while $l_d>0$ is the fracture length scale parameter. It is worth mentioning that~\eqref{plas-part5} and~\eqref{frac-part5} imply that the dissipated energy in the present model is a state function.

With the above definitions, a global energy functional is defined as
%
\begin{equation}
\label{1D5}
\begin{aligned}
\mathcal{E}(u,\varepsilon^p,\alpha,d)=\int^{L}_{0} A \big[ {W}_{elas}(\varepsilon,\varepsilon^p,d) + {W}_{plas}(\alpha,d,\alpha') + {W}_{frac}(d,d') \big ]\,
\mathrm{d}{{x}}  .
\end{aligned}
\end{equation}
%
Minimization of the energy functional~\eqref{1D5} with respect to the displacement field, the crack phase-field, and the plasticity variables leads to the following weak formulation.

%\begin{form}[Euler-Lagrange equations for phase-field brittle fracture]
%	\label{form_5}
%	Let constants $(E$ $,G_c,l_f) \geq 0$  be given with the initial conditions $u_0= u(x,0)$ and  $d_0=d({x},0)$. For the loading increments $n=1,2,\ldots, N$, find $ u:=u^n\in \mathcal{W}^u_{\bar{u}}$ and $d:=d^n\in \mathcal{W}^d_{d_{n-1}}$: 
%	\begin{equation}
%	\left\{
%	\begin{aligned}
%		%========================	
%		&\calE_u(u,\varepsilon^p,\alpha,d;\delta u)=\int^L_{0}(1-d)^2 E\big(\varepsilon(u)-\varepsilon^p\big)\varepsilon(\delta u)\,\mathrm{d}x =0 \quad \forall \,\delta u\in\mathcal{W}^u_0,%\
%		%\hspace{3.18cm} \emph{(E)}	
%		\\
%		%\tag{E}\\
%		%========================
%		&\calE_d(u,\varepsilon^p,\alpha,d;\delta d)=
%		\int^L_{0} \bigg[-(1-d)\bigg(E\big(\varepsilon(u)-\varepsilon^p\big)^2 + H\alpha^2+ 2\sigma_Y\alpha+ \sigma_Yl_p\alpha'^2 + w_0\bigg)\delta d + l_f d'(\delta d)'\bigg]\,\mathrm{d}x \geq 0 \quad \forall \,\delta d \in \mathcal{W}^d_{0} .
%		%\hspace{0.1cm} \emph{(D)}	\\
%		%========================
%	\end{aligned}
%    \right.
%    \label{weak_5}
%    \end{equation}
%\end{form}
%

\begin{form}[\textsc{F5}: Bayesian inversion for phase-field ductile fracture with gradient plasticity]
	\label{form_5}
	Consider an open bounded one-dimensional bar on an interval $\calB:=[0,L]$ with boundary $\partial \calB$ defined at $x=0$ and $x=L$.
	Let constants $(E$ $,H,\sigma_Y,w_0,l_d,l_p) \geq 0$  be given with the initial conditions $u_0= u({x},0)$, $\varepsilon^p_0=\varepsilon^p({x},0)$, $\alpha_0=\alpha({x},0)$, and  $d_0=d({x},0)$. For the loading increments $n=1,2,\ldots, N$, find $ u:=u^n\in \mathcal{W}^u_{\bar{u}}$, $\varepsilon^p={\varepsilon^p}^n\in \mathcal{W}^p$, $\alpha:=\alpha^n\in \mathcal{W}^\alpha_{\alpha_{n-1},\,\varepsilon^p-\varepsilon^p_{n-1}}$, and $d:=d^n\in \mathcal{W}^d_{d_{n-1}}$ satisfying the following Euler-Lagrange equations in weak form:		
		\begin{equation*}
		\left\{
		\begin{aligned}
		%========================
		&\calE_u(u,\varepsilon^p,\alpha,d;\delta u)=\int^L_{0}(1-d)^2 E\big(\varepsilon(u)-\varepsilon^p\big)\varepsilon(\delta u)\,\mathrm{d}x =0 \quad \forall \,\delta u\in\mathcal{W}^u_0  , 
		%\hspace{1.55cm} \emph{(E)}	
		\\
		%========================
		&\calE_\alpha(u,\varepsilon^p,\alpha,d;\delta\varepsilon^p,\delta\alpha)=
		\int^L_{0} -(1-d)^2 \Big[E\big(\varepsilon(u)-\varepsilon^p\big)\delta \varepsilon^p
		+ \Big( H\alpha 
		+ \sigma_Y \Big)\delta\alpha \\ & \hspace*{5cm}
		+ \sigma_Y \,l_p^2\,\alpha'(\delta \alpha)' \Big]\,dx 		
		\geq 0 \quad \forall \,\delta\varepsilon^p \in \mathcal{W}^p, \quad \forall \,\delta\alpha \in \mathcal{W}^\alpha_{0,\,\delta\varepsilon^p}  ,
		%\hspace{1.55cm} \emph{(P)}	
		\\
		%========================
		&\calE_d(u,\varepsilon^p,\alpha,d;\delta d)=
		\int^L_{0} \Big[-(1-d)\Big(E\big(\varepsilon(u)-\varepsilon^p\big)^2 + H\alpha^2+ 2\sigma_Y\alpha+ \sigma_Y\,l_p\,\alpha'^2\Big)\delta d + w_0\delta d  \\ & \hspace*{9cm}
		+ w_0 \,l_d^2\, d'(\delta d)' \Big]\,\mathrm{d}x \geq 0 \quad \forall \,\delta d \in \mathcal{W}^d_{0}  .
		%\hspace{1.4cm} \emph{(D)}	
		\\
		%========================
	\end{aligned}
\right.
\label{weak_5}
\end{equation*}
The unknown material parameters then follow from the probabilistic Bayesian inversion 
\begin{equation*}
	\BfrakP\leftarrow\textsc{BI}\big(\textsc{F5}(\Bfraku)\big) \WITH
	\Bfraku:=(u,\varepsilon^p,\alpha,d) 
	\AND
	 \BfrakP:=(E,H,\sigma_Y,w_0,l_p) .
\end{equation*}
\end{form} 			
%
As in Section~\ref{Ex4}, the {history field} approach~\cite{MieWelHof10b} is employed to solve the  variational inequality~\eqref{weak_4}$_3$. On the other hand, in~\eqref{weak_4}$_2$, one makes use of the relation $\delta\alpha=\vert\delta\varepsilon^p\vert$ and the incremental hardening law $\alpha_{n}=\alpha_n+\vert \varepsilon^p_{n}-\varepsilon^p_{n-1}\vert$. This problem can be solved in a convenient way by eliminating $\varepsilon^p$ through the incremental flow rule $\varepsilon^p_{n}=\varepsilon^p_{n-1}+(\alpha_n-\alpha_{n-1})\,\mathrm{sign}(\sigma^{trial}_n)$, where $\sigma^{trial}_n:=\sigma(\varepsilon_{n},\varepsilon^p_{n-1},d_{n})$, with $\sigma$ given in~\eqref{stress_5}; see, e.g.,~\cite{ulloa2021,noii2021bayesian}. For  loading paths without plastic flow reversals, e.g., monotonic loading with possible elastic unloading, the 1D problem is further simplified by setting $\varepsilon^p\equiv\alpha$.


%=======================================================================
\sectpc{Bayesian inference}
%=======================================================================
In this numerical example, let the bar, of unitary length L = 1 with $x\in\calB:=[0,1]$ that is initially unstretched, and undamaged. Its left-end is fixed, i.e., $x=0$, while on its right-end, i.e., $x=1$, a monotonic displacement increment  $\Delta \bar{u}=1\times10^{-5}$ mm is applied for 151 time steps, see Figure \ref{Fig_Ch_geoF}a. For the spatial discretization, we use 100 elements and the main script named \texttt{ductile\_1D.m}.

In this example we use a four-dimensional Bayesian inversion to identify $(E,\,\sigma_Y,\,w_0,\,H)$ simultaneously. To this end, EnKF is chosen and we set an initial guess of $E^0=60\,000$, $\sigma_Y^0=300$, $H^0=300$, $w_0^0=20$.   The parameters bound are listed in Table \ref{range5} including the true values. Figure \ref{duc1} shows the MCMC chains where they converge very fast. The posterior densities are depicted in Figure \ref{duc2}, where for all unknowns, a narrow distribution is obtained. The medians of the MCMC chains are mentioned in Table \ref{range5} (a very good accuracy). These values are used to plot the load-displacement curve as shown in Figure \ref{duc3}.
 


  \begin{table}[!]
	\caption{The uniform prior distribution of the inferred parameters in Example 5 (ductile fracture) including the true values.}
	\vspace{1mm}
	\centering
	\begin{tabular}{|llccc|}
		\hline
		Parameter  &$ E\,[\text{MPa}]\quad$        &  $\quad\sigma_Y\,[\text{MPa}]\quad$  &   $\qquad w_0\,[\text{MPa}]\quad$   & $\quad H\,[\text{MPa}] \quad$       \\\hline\hline
	$\mathrm{min}$    &30\,000   & 300  & 10 &200 \\[4mm]
	$\mathrm{max}$ &  100\,000  &  400  &  50 & 400 \\[4mm]
	$\mathrm{true~value}$\qquad\qquad  &   70\,500  &  330  &  30 & 250\\[4mm]
	$\mathrm{EnKF}$\qquad\qquad  &   70\,495  &  329.9  &  30 & 250 \\[2mm]
		\hline
	\end{tabular}\label{range5}
\end{table}


\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/ductile/MCMC_E}} 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/ductile/MCMC_sigma}}\\
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/ductile/MCMC_w}}
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/ductile/MCMC_H}}
	\caption{Example 5. The evolution of the MCMC chains using EnKF for four different material parameters in ductile fracture.}
	\label{duc1}
\end{figure}

\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/ductile/pdf_E}} 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/ductile/pdf_sigma}}\\
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/ductile/post_w}}
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/ductile/pdf_H}}
	\caption{Example 5. The posterior density of the material parameter in ductile fracture using EnKF. The true values are shown with green dashed lines. 
	}
	\label{duc2}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.7\textwidth]{Figures/ductile/load}
	\caption{The load-displacement curve for the ductile fracture problem in Example 5, estimated by the inferred values. 
	}
	\label{duc3}
\end{figure}

 In this example, following the new proposed the step-wise Bayesian inversion for ductile phase-field fracture\cite{noii2021bayesian}, we consider four stages of  Bayesian inversion to identify the parameters $E$ (elastic stage), $\sigma_Y$ (perfectly plastic stage), $H$ (hardening stage), and $w_0$ (damaging stage). The uniform prior densities, including the true values, are listed in Table~\ref{range5}. Such a step-wise Bayesian framework is computationally effective since a single parameter is estimated in each stage (and used as input in subsequent stages). The posterior densities (using the last 4\,000 iterations) are illustrated in Figure~\ref{duc1}. The $\hat{R}$-convergence of the parameters is depicted in Figure~\ref{duc2} indicating the rapid convergence of all unknowns. Finally, the load-displacement curve obtained using the estimated parameters is shown in Figure~\ref{duc3}, indicating a typical ductile fracture process.



%=======================================================================
\sectpb[Example6]{Example 6: Phase-field fracture for thermoelastic materials}
%=======================================================================
The crack propagation due to the thermal effect is occurred in different engineering problems such laser fracture, additive manufacturing, drying shrinking cracking of concrete, etc. Here, the main challenge is the estimation of displacement, phase-field, and temperature. In \cite{miehe2015phase}, a fully coupled approach for solving the thermo-mechanical system was presented. This technique overcame the computational problems related to realization of sharp crack discontinuities, specifically in the complex crack topologies. 

The effect of temperature on the plastic deformation, e.g., in metals (nucleation and coalescence of voids toward rapture) or glassy polymers (plastic and craze deformations) is happened because of the temperature increase due to the plastic dissipation \cite{miehe2015phase}. The authors of \cite{wang2020phase}, introduced a parallel algorithm to simulate the dynamic and quasi-static brittle fracture of theromoelastic materials including the source codes. Finally, in order to enhance the efficiency of the monolithic solver, in \cite{mandal2021fracture}, a monolithic \texttt{BFGS} algorithm was implemented to solve the multi-field discretized equations.    
%=======================================================================
\sectpc[Section21]{State variables and kinematics}
\label{sec:basic_def6}
%=======================================================================
In this example, the given BVP is a coupled multi-field system for fracturing solids with thermal effects. Such a model can be formulated based on a coupled three-field system.  In particular, at material points $x\in\mathcal{B}$ and time $t\in\mathbb{T}$, the BVP solution provides the displacement field $u:\mathcal{B}\times \mathbb{T} \rightarrow \mathbb{R}$, the temperature field $\mathcal{T}:\mathcal{B}\times\mathbb{T} \rightarrow \mathbb{R}$, and the crack phase-field fracture variable $d:\mathcal{B}\times \mathbb{T} \rightarrow [0,1]$. 
%As such, the global primary fields are given by
% %
% \begin{equation}
% 	u: 
% 	\left\{
% 	\begin{array}{ll}
% 		\Gamma \times \calT \rightarrow \mathbb{R} \\
% 		(x, t)  \mapsto u(x,t)
% 	\end{array}
% 	\right.
% 	,\quad \
% 	\theta:
% 	\left\{
% 	\begin{array}{ll}
% 		\Gamma \times \calT \rightarrow \mathbb{R} \\
% 		(x, t)  \mapsto \theta(x,t)
% 	\end{array}
% 	\right.
% 	,\quad \
% 	d: 
% 	\left\{
% 	\begin{array}{ll}
% 		\Gamma \times \calT \rightarrow [0,1] \\
% 		(x, t)  \mapsto d(x,t)
% 	\end{array}.
% 	\right.
% 	%\WITH
% 	%\dot{d} \ge 0
% 	\label{phi-p-d-fields}
% \end{equation}
% %
Adopting the small strain hypothesis, the strain tensor is additively decomposed into an elastic part $\varepsilon^e$ and a thermal part $\varepsilon^\mathcal{T}$ as
%
\begin{equation}
	\varepsilon(x,t) = \varepsilon^e(x,t) + \varepsilon^\mathcal{T}(x,t).
	\label{s2-strain-e-t}
\end{equation}

For materials that expand isotropically when the temperature is increased, the thermal part can be computed as
%
\begin{equation}
	\varepsilon^\mathcal{T} =\alpha(\mathcal{T}-\mathcal{T}_0),
	\label{strain-t}
\end{equation}
where $\mathcal{T}_0$ is the initial temperature and $\alpha$ is the thermal expansion coefficient. 

In the present one-dimensional problem, the thermal Dirichlet and Neumann boundary conditions are described by
%
\begin{equation}
	\mathcal{T} = \bar{\mathcal{T}} \ \ \textrm{on}\  \ {\partial^{\mathcal{T}}_ D\mathcal{B}} \AND
	Q\, n = \bar{q} \ \ \textrm{on}\ \ {\partial^{\mathcal{T}}_N\mathcal{B}},
	\label{flu-bcs}
\end{equation}
%
where $Q$ is the thermal volume flux and $\bar{q}$ is the thermal transport on the Neumann boundary, where $n=1$ for $x=L$ and $n=-1$ for $x=0$, and $\bar{\mathcal{T}}$ is the imposed temperature on the Dirichlet boundary. Moreover, the heat flux in~\req{flu-bcs} can be described by the negative direction of the thermal heat gradient $\mathcal{T}'$ through Fourier's law of heat conduction as
\begin{equation}
	Q =-{\cal{K}}_d \;\mathcal{T}'=- g(d)\cal{K} \mathcal{T}'.
\end{equation}
%
Here, ${\cal{K}}_d=g(d)\cal{K} $ is  the degraded thermal conductivity with the same quadratic degradation function given in ~\eqref{quad_deg}.

To elaborate the corresponding variational formulation, we employ the function spaces~\eqref{space1} for the displacement and the crack phase-field, and further introduce the function space for the temperature field
%
\begin{equation}\label{space1_ex6}
	\mathcal{W}^{\mathcal{T}}_{\bar{\mathcal{T}}}:=\{ \mathrm{H}^1(\mathcal{B}) \ : \  \mathcal{T}=\bar{\mathcal{T}} \ \ \text{on} \ \  \partial^{\mathcal{T}}_D\mathcal{B} \}.
\end{equation}

%=======================================================================
\sectpc{Energy quantities and variational principles}
\label{sec:energy_functions6}
%=======================================================================
Let $\calB\subset\mathbb{R}$ be open and let $\mathbb{T} := ( t_0,T)$ with $T>0$ being the end time value.
The strong formulation of the quasi-static balance of linear momentum along with prescribed external body force $\bar{f}$ satisfy:
%
\begin{equation}
	\begin{aligned}\label{PDE_ex61}
		\Big(E(x)g(d)(\varepsilon(x,t)-\varepsilon^\mathcal{T}(x,t))\Big)'+\bar{f}=0\quad\quad\forall \,  u \in \mathcal{W}^u_{\bar{u}}  \quad\quad \text{in} \quad \calB \times \mathbb{T},
	\end{aligned}
\end{equation}
%
Also, the energy balance statement based on the evolution of  temperature yields for the following strong form:  
%
\begin{equation}
	\begin{aligned}\label{PDE_ex62}
		\rho\,c\,\dot{\mathcal{T}}+Q'=\bar{r}_\mathcal{T} \quad\quad\forall \,\mathcal{T} \in \mathcal{W}^\mathcal{T}_{\bar{\mathcal{T}}} \quad\quad \text{in} \quad\calB \times \mathbb{T}.
	\end{aligned}
\end{equation}
%
initialized with
\begin{equation}
	\mathcal{T}=\mathcal{T}_0 \quad\quad \text{in} \quad \calB \times {0},
\end{equation}
%
Additionally, the global evolution equation for the crack phase-field in the rate-dependent form yields the following  local statement:
%
\begin{equation}
	\begin{aligned}\label{PDE_ex63}
		(1-d)\mathcal{D}-(d-l_f^2d'')=\eta_f\dot{d}\quad\quad\forall \,  d \in \mathcal{W}^d_{\bar{d}}\quad\quad \text{in}\quad \calB \times \mathbb{T}.
	\end{aligned}
\end{equation}
%
together with a homogeneous Neumann condition for crack surface by
\begin{equation}
	\partial_n{d}=0\quad\quad \text{in} \quad \partial\calB \times \mathbb{T},
\end{equation}
%
We introduce  a positive crack driving force $\calD$ in $t\in [0,t_n]$  as a driving force for the crack surface. To define $\calD$, in agreement with~\eqref{elas-part} and~\eqref{elas-part4}, the {elastic contribution} affected by temperature response reads:
%
In agreement with~\eqref{elas-part} and~\eqref{elas-part4}, the quadratic {elastic contribution} reads as follows:
%
\begin{equation}
	{W}_{elas}(u,\varepsilon^\mathcal{T},d):=\frac{1}{2}g(d)E(\varepsilon-\varepsilon^\mathcal{T})^2,
	\label{elas-part5Heat}
\end{equation}
%
so, a positive crack driving force $\calD$ becomes:
\begin{equation}
	\mathcal{D}:=\mathcal{D}(\varepsilon,\varepsilon^\mathcal{T})=\frac{\partial W_{elas}}{\partial d}=-(1-d)E(\varepsilon-\varepsilon^\theta)^2, 
\end{equation}	
%
where $g(d)$ is a degradation function. Varitional equations due to the strong local statements of the \req{PDE_ex61}, \req{PDE_ex62}, and \req{PDE_ex63} induces the following Formulation:
%
\begin{form}[\textsc{F6}: Bayesian inversion for phase-field fracture with thermoelasticity]
	\label{form_ETD}
	Consider an open bounded one-dimensional bar on an interval $\calB:=[0,L]$ with boundary $\partial \calB$ defined at $x=0$ and $x=L$.
	Let constants $({\bar{r}_\mathcal{T}},\bar{q}, E,G_c,l_f,K,\rho,\cal{C}) \geq \text{0}$  be given with the initial conditions $u_0= u({x},0)$, $\mathcal{T}_0=\mathcal{T}({x},0)$, and  $d_0=d({x},0)$. For the loading increments $n=1,2,\ldots, N$, find $ u:=u^n\in \mathcal{W}^u_{\bar{u}}$, $\mathcal{T}:=\mathcal{T}^n\in \mathcal{W}^{\mathcal{T}}_{\bar{\mathcal{T}}}$, and $d:=d^n\in \mathcal{W}^{d}_{d_n}$ satisfying the following Euler-Lagrange equations in weak form:	
	\begin{equation*}
		\left\{
		\begin{aligned}
			%========================
			&\calE_u(u,\mathcal{T},d;\delta u)=\int^L_{0}(1-d)^2 E\big(\varepsilon(u)-\varepsilon^{\mathcal{T}}(\mathcal{T})\big)\varepsilon(\delta u)\,\mathrm{d}x =0 \quad \forall \,\delta u\in\mathcal{W}^u_0  , 
			%\hspace{1.55cm} \emph{(E)}	
			\\
			%========================
			&\calE_\mathcal{T}(u,\mathcal{T},d;\delta\mathcal{T}) = \displaystyle\int^L_0 \Big[\Big({\rho\;\cal{C}}(\mathcal{T}-\mathcal{T}_n)  -\Delta t\;\bar{r}_\mathcal{T}
			\Big)s + (\Delta t\;{\cal{K}}_d \;\mathcal{T}') \cdot (\delta \mathcal{T})' \Big] \,\mathrm{d}x +  \bar{q}\delta\mathcal{T}\,\big|_{\partial_N^{\mathcal{T}}\mathcal{B}}  = 0, \\ & \hspace*{13cm} \forall \,\delta \mathcal{T} \in \mathcal{W}^\mathcal{T}_{0},\\ 
			%======================== 
			&\calE_d(u,\varepsilon^p,\alpha,d;\delta d)=
			\int^L_{0} \Big[-(1-d)E\big(\varepsilon(u)-\varepsilon^\mathcal{T}(\mathcal{T})\big)^2\delta d + \frac{G_c}{l_f}d\,\delta d + l_f d'(\delta d)'\Big]\,\mathrm{d}x \geq 0 \\ & \hspace*{13cm} \forall \,\delta d \in \mathcal{W}^d_{0}  .
			%\hspace{1.4cm} \emph{(D)}	
			\\
			%========================
		\end{aligned}
		\right.
	\end{equation*}
	The unknown material parameters then follow from the probabilistic Bayesian inversion 
	\begin{equation*}
		\BfrakP\leftarrow\textsc{BI}\big(\textsc{F6}(\Bfraku)\big) \WITH 
		\Bfraku:=(u,\mathcal{T},d) 
		\AND
		\BfrakP:=(E,G_c,K,\cal{C}) .
	\end{equation*}
\end{form}

 
 %=======================================================================
\sectpc{Bayesian inference}
%=======================================================================
In this example, we have a couples system of equations, including the phase-field, elasticity, and heat equation. The range of the parameters and the true values are listed in Table \ref{range6}. The script named $\texttt{1D\_thermoelastic.m}$ and EnKF is used to identify the unknown parameters. We use the load-displacement curve (estimated by the true values) as the reference observation at time $T=1\times 10^{5}$ seconds.  

  \begin{table}[!]
	\caption{The uniform prior distribution of the inferred parameters in Example 6 (thermoelastic) including the true values.}
	\vspace{1mm}
	\centering
	\begin{tabular}{|llccc|}
		\hline
		Parameter  &$ \hspace{-0.5cm}G_c\,[\text{MPa mm}]\quad$        &  $\quad E\,[\text{MPa}]\quad$  &   $K\,[\text{W/(m $\cdot$ K)}]\quad$   & $\quad \alpha\,[\text{K$^{-1}$}] \quad$       \\\hline\hline
		$\mathrm{min}$    & 0.01  & 200  &  $1\times 10^{-2}$& $7\times 10^{-4}$\\[4mm]
	  $\mathrm{max}$ &  0.10  &  400  &  $1\times 10^{-1}$ & $5\times 10^{-3}$ \\[4mm]
	 $\mathrm{true~value}$\qquad\qquad  &   0.04  &  340  &  $2\times 10^{-2}$ & $8\times 10^{-4}$\\[4mm]
	 $\mathrm{EnKF}$\qquad\qquad  &   0.0399  &  340.001  &  $2.21\times 10^{-2}$ & $7.91\times 10^{-4}$ \\[2mm]
		\hline
	\end{tabular}\label{range6}
\end{table}




\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/MCMC_Gc}} 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/MCMC_E}}\\
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/MCMC_K}}
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/MCMC_alpha}}
	\caption{Example 6. The evolution of the MCMC chains using EnKF for four different material parameters in thermoelastic example.
	}
	\label{EH1}
\end{figure}

\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/pdf_Gc}} 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/pdf_E}}\\
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/pdf_K}}
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/pdf_alpha}}
	\caption{Example 6. The posterior density of the material parameter in thermoelastic example using EnKF. The true values are shown with green dashed lines. 
	}
	\label{EH2}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.7\textwidth]{Figures/EH/comp}
	\caption{The load-displacement curve for the thermoelastic fracture problem in Example 6 estimated by the inferred and true values. 
	}
	\label{EH3}
\end{figure}

\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/disp}} 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/phase}}\\
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/EH/thermal.png}}
	\caption{Example 6. The evolution of displacement (top left), phase-field (top right), and the temperature (bottom) during different time steps. The last step which used for the Bayesian inversion is shown with a dashed black line.
	}
	\label{EH4}
\end{figure}

Let the bar, of unitary length L = 1 with $x\in\calB:=[0,1]$ that is initially unstretched, and undamaged. Its left-end is fixed, i.e., $x=0$, while on its right-end, i.e., $x=1$, a monotonic displacement increment  $\Delta \bar{u}=1\times10^{-5}$ mm is applied for 155 time steps, see Figure \ref{Fig_Ch_geoF}c. Additionally, we use 99 elements for the spatial discretization. The initial values are $G_c^0=0.05$, $E^0=300$, $\mathcal{K}^0=5\times 10^{-2}$, and $\alpha^0=1\times 10^{-3}$. For temperature boundary condition, one dimensional bar is restricted according to \req{BC_heat} such that $\mathcal{T}_1=1\;^{\circ}\text{C}$ and $\mathcal{T}_2=0\;^{\circ}\text{C}$.

The evolutions of the MCMC chains for all parameters are shown in Figure \ref{EH1}. The unknowns show a negligible uncertainty and converge rapidly to the true values with an acceptance rate of 71.6\%. The posterior densities are illustrated in Figure \ref{EH2}. The distribution of $G_c$ and $E$ is symmetric, and the true values are exactly in the center (the median). The medians are denoted in Table \ref{range6}. We compare the load-displacement diagram using inferred and true values, as shown in Figure \ref{EH3}. An excellent agreement between the curves points out the efficiency of the method. 

As we already mentioned, the reference observation is chosen at the last time step.  We show the displacement $u$, the phase-field $d$, and the temperature $\mathcal{T}$ for 100 time steps in Figure \ref{EH4}.   




 


%=======================================================================
\sectpb[Example7]{Example 7: Phase-field approach to fatigue in brittle materials}\label{Ex7}
%=======================================================================

The last example considers the phase-field approach to fatigue, a topic that has been gaining attention in the recent literature. Most works on this subject focus on brittle materials~\cite{alessi2018phenomenological,carrara2020,mesgarnejad2019,lo2019,schreiber2020}, although models for rubber~\cite{loew2020}, ductile materials~\cite{seiler2020efficient}, and ductile materials with plastic coupling~\cite{ulloa2021,selevs2021} have also been proposed. Here, we focus on the 1D formulation for the brittle case, initially addressed in~\cite{alessi2018phenomenological}.

The brittle fracture problem presented in Section~\ref{Ex4} is taken as a point of  departure. However, the displacements are now imposed cyclically. To account for the effect of cyclic loading, a fatigue degradation function is introduced, characterized in the simplest case by two material parameters which are hereby estimated along with Young's modulus and the fracture toughness.

 %=======================================================================
\sectpc[Section21]{State variables and kinematics}
\label{sec:basic_def7}
%=======================================================================

As in Section~\ref{Ex4}, the primary fields in the present model consist of the displacement field $u:\mathcal{B} \times \mathbb{T} \rightarrow \mathbb{R}$ and the non-local phase-field fracture variable $d:\mathcal{B} \times \mathbb{T} \rightarrow [0,1]$, with the corresponding function spaces given in~\eqref{space1}. Consequently, the fatigue mechanism does not entail the introduction of a new internal variable, but rather, of a history-dependent parameter, as will become clear below.

%=======================================================================
\sectpc{Energy quantities and variational principles}
\label{sec:energy_functions7}
%=======================================================================

The standard phase-field model for brittle fracture, i.e., based on the regularized crack surface energy density~\eqref{frac-part}, predicts crack propagation at critical stress amplitudes. As such, the model is not suitable to describe fatigue fracture under cyclic loading, which may occur at repetitive load amplitudes well below the ultimate strength of the material. To account for fracture under such conditions, \cite{alessi2018phenomenological} proposed to progressively degrade the crack resisting force by means of a suitable accumulation variable, for which a measure of accumulated energy was later established~\cite{carrara2020} and adopted in subsequent works.

In the context of the above-mentioned framework, the definition of energy quantities that comply with the second law of thermodynamics, i.e., non-decreasing energy dissipation, requires a delicate treatment. Specifically, the definition of a state function representing the regularized dissipated energy due to fracture, as done in~\eqref{frac-part} and~\eqref{frac-part5}, is no longer possible. Instead, we must rely on a path-dependent quantity, with a fatigue degradation mechanism acting on the rate of crack-surface energy dissipation. In particular, we may define a total energy density of the form
%
\begin{equation}
	{W}(\varepsilon,d;\gamma) := 
	{W}_{elas}(\varepsilon,d) + \int_0^tf(\gamma)\frac{\mathrm{d}}{\mathrm{d}t}{W}_{frac}(d,d')\,\mathrm{d}t.
	\label{pseudo-energy_7}
\end{equation}
%
Because the crack driving force is not modified, the stored elastic strain energy~\eqref{elas-part4} is again employed in the present model. On the other hand, the time derivative of the regularized fracture energy density~\eqref{frac-part} is scaled by a non-negative degradation function $f(\gamma)$, to be defined below, which renders the dissipated energy a path-dependent quantity. Note that in~\eqref{pseudo-energy_7}, the second law of thermodynamics is satisfied by the non-negativity of the dissipation rate, i.e., $f(\gamma)\frac{\mathrm{d}}{\mathrm{d}t}{W}_{frac}(d,d')\geq 0$.

In~\eqref{pseudo-energy_7}, we have introduced a \emph{fatigue accumulation} variable $\gamma:\mathcal{B}\times\mathcal{T}\rightarrow\mathbb{R}_+$ and a \emph{fatigue degradation function} $\gamma\mapsto f(\gamma)\in[0,1]$, endowed with the properties $f(\gamma\leq\gamma_c)=1$, $f(\gamma>\gamma_c)\in[0,1]$ and $f'(d) \geq 0$. In particular, we adopt the following form~\cite{carrara2020}:
%
\begin{equation}
f(\gamma)\coloneqq \begin{dcases} 1 & \text{if}  \quad \gamma(x,t) \leq \gamma_c, \\ 
\bigg[1-k\log\bigg(\frac{\gamma(x,t)}{\gamma_c}\bigg)\bigg]^2 & \text{if} \quad \gamma_c\leq\gamma(x,t) \leq \gamma_c10^{1/k}, \\ 
0 & \text{otherwise},
\end{dcases}
\label{fat_func}
\end{equation}
%
where  $k$ is a material parameter that controls the rate of (logarithmic) decay of the fatigue degradation function, and $\gamma_c\geq0$ is a material threshold parameter, under which no fatigue effects are triggered. The fatigue variable $\gamma$ is defined as an accumulation of strain energy density during loading stages. To this end, we define
%
\begin{equation}
\gamma(x,t) := \int_{0}^t\dot{\vartheta}(x,s)\bar{H}\big(\dot{\vartheta}(x,s)\big)\, \mathrm{d}s, \quad \text{with} \quad \vartheta(x,t)\coloneqq W_{elas}(\varepsilon,d),
\label{fat_field}
\end{equation}
%
where $\bar{H}$ is the Heaviside function.

In view of the path-dependent energy density~\eqref{pseudo-energy_7}, a total energy functional can only be approximated in incremental form. In agreement with previous incremental treatments for state-dependent dissipation potentials~\cite{miehe2011,ulloa2021}, we consider the form
%
\begin{equation}\label{1D7}
\begin{aligned}
\mathcal{E}(u_{n+1},d_{n+1};\gamma_n)=\int^{L}_{0} A \big[ {W}_{elas}(u_{n+1},d_{n+1})+f(\gamma_n){W}_{frac}(d_{n+1},d_{n+1}')\big]\,
\mathrm{d}{{x}}  ,
\end{aligned}
\end{equation} %  \\ + \sum_{s=0}^{n-1} f(\gamma_{s}){W}_{frac}(d_{s+1},{d'}_{s+1})  
%
where the current time step is denoted with a subscript $n+1$. Note that the pseudo-time integral in~\eqref{pseudo-energy_7} has been evaluated in incremental form by fixing the fatigue variable $\gamma$ at the previous time step. Minimization of the energy functional~\eqref{1D7} with respect to the displacement field and the crack phase-field leads to the following weak formulation.


\begin{form}[\textsc{F7}: Bayesian inversion for phase-field approach to fatigue]
	\label{form_7}
	Consider an open bounded one-dimensional bar on an interval $\calB:=[0,L]$ with boundary $\partial \calB$ defined at $x=0$ and $x=L$.
	Let constants $(E$ $,G_c,l_f,\gamma_c,k) \geq 0$  be given with the initial conditions $u_0= u(x,0)$ and  $d_0=d({x},0)$. For the loading increments $n=1,2,\ldots, N$, find $ u:=u^n\in \mathcal{W}^u_{\bar{u}}$ and $d:=d^n\in \mathcal{W}^d_{d_{n-1}}$ satisfying the following Euler-Lagrange equations in weak form:		
	\begin{equation}
	\left\{
	\begin{aligned}
		%========================	
		&\calE_u(u,d;\delta u)=\int^L_{0}(1-d)^2 E\varepsilon(u)\varepsilon(\delta u)\,\mathrm{d}x =0 \quad \forall \,\delta u\in\mathcal{W}^u_0 ,%\
		%\hspace{3.18cm} \emph{(E)}	
		\\
		%\tag{E}\\
		%========================
		&\calE_d(u,d;\delta d)=
		\int^L_{0} \Big[-(1-d)E\varepsilon(u)^2\delta d + f(\gamma_{n-1})\frac{G_c}{l_f}d\,\delta d + f(\gamma_{n-1})l_f d'(\delta d)'\Big]\,\mathrm{d}x \geq 0 \\ & \hspace*{13cm}
		\forall \,\delta d \in \mathcal{W}^d_{0}   .
		%\hspace{0.1cm} \emph{(D)}	\\
		%========================
	\end{aligned}
    \right.
    \label{weak_7}
    \end{equation}
The unknown material parameters then follow from the probabilistic Bayesian inversion 
\begin{equation*}
	\BfrakP\leftarrow\textsc{BI}\big(\textsc{F7}(\Bfraku)\big) \WITH
	\Bfraku:=(u,d) 
	\AND
	\BfrakP:=(E,G_c,\gamma_c,k) .
\end{equation*}
\end{form}

Once more, the history field approach~\cite{MieWelHof10b} is employed here to handle the inequality constraint in~\eqref{weak_7}$_2$.

\begin{figure}[!b]
	\centering
	\subfloat{\includegraphics[width=0.6\textwidth]{Figures/fatigue/load11}} 
	\vspace{0.4cm}  
	\vspace{-0.4cm}
	\caption{Example 7. Cyclic displacement loading applied to the right-edge of the homogeneous uniaxial test shown in Figure \ref{Fig_Ch_geoF}c. \TODO{(Amir) change Y-axis like Figure 22 Xaxis: $\bar{u}$[mm]}} 
	\label{fat1-0}
\end{figure}
%=======================================================================
\sectpc{Bayesian inference}
%=======================================================================
In this numerical example, let the bar, of unitary length L = 1 with $x\in\calB:=[0,1]$ that is initially unstretched, and undamaged. We set $\gamma=0$ at $t=0$. Its left-end is fixed, i.e., $x=0$, while on its right-end, i.e., $x=1$, a monotonic displacement increment  $\Delta \bar{u}=1\times10^{-5}$ mm is applied for 151 time steps, see Figure \ref{Fig_Ch_geoF}a. Regarding the spatial discretization, we use 300 elements. Cyclic displacement loading applied to the right-edge of the homogeneous uniaxial test shown in Figure \ref{fat1-0} the displacements are now imposed cyclically. 

In order to perform our Bayesian inversion, we estimate simultaneously $(E,\,k,\,G_c,\,\gamma_c)$ (four-dimensional Bayesian inversion). The assumed ranges and true values are list in Table \ref{range7}. 
The main script is $\texttt{1D\_fatigue.m}$ and we employ DRAM algorithm to infer the materials unknowns. 

Figure \ref{fat2} shows the effect of different parameters on the load-displacement diagram. For materials with low Young's modulus (e.g., ductile materials), several load cycles are needed for the fracture. However, for too stiff materials (e.g., brittle materials), fewer load cycles lead to a full fracture.
It is more pronounced with the higher difference between the peak points, as higher $E$ enhances the peak points' time. Regarding higher $G_c$, as more energy is needed for the fracture, more load cycles are necessary. Hence, e.g., $G_c=0.04\,\text{MPa}$ requires more time (i.e., higher cycle number), and the difference between the peak point is more. Inversely, less $G_c$ facilitates the full fracture time. As shown, the same pattern is observed for $\gamma_c$. Finally, $k$ is a phenomenological parameter that enhances the fracture time.



  \begin{table}[!]
	\caption{The computational features and the results of the Bayesian inversion for Example 7.}
	\vspace{1mm}
	\centering
	\begin{tabular}{|llccc|}
		\hline
	Parameter  &$\hspace{-0.1cm} E\,[\text{MPa}]\quad$        &  $\quad k\,[\text{MPa}]\quad$  &   $\qquad G_c\,[\text{MPa mm}]\quad$   & $\quad \gamma_c\,[\text{MPa}] \quad$         \\\hline\hline
	$\mathrm{min}$    &30\,000   & 0.2  & 0.02 &0.001 \\[4mm]
	$\mathrm{max}$ &  100\,000  &  0.6  &  0.04 & 0.01 \\[4mm]
	$\mathrm{true~value}$\qquad\qquad  &   71\,300  &  0.4  &  0.027 & 0.0075\\[4mm]
	$\mathrm{DRAM}$\qquad\qquad  &   70\,320  &  3.96  &  0.035 & 0.00572 \\[2mm]
		\hline
	\end{tabular}\label{range7}
\end{table}




\begin{figure}[!t]
	%\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/E}} 
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/k}}\\
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/Gc}} 
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/gamma}}
	\vspace{0.4cm}  
	\vspace{-0.4cm}
	\caption{Example 7. The effect of different parameters on the load-displacement curve.
	}
	\label{fat2}
\end{figure}



\begin{figure}[!t]
	%\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/load2}} 
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/load4}}
	\caption{Example 7. Left curve is a load-displacement curves of the homogeneous response for a uniaxial tests under displacement loading,
	     and right curve is homogeneous load response versus cycle number with damage under displacement loading and the
		 selected critical points for the Bayesian inversion (shown in red) \TODO{(Amir) change right figure x-axis tile to cycle number}.}
	\label{fat1}
\end{figure}
%
 Figure \ref{fat1} shows the homogeneous response for a uniaxial tests under displacement loading displayed in Figure \ref{Fig_Ch_geoF}c. In this example due to the fatigue loading, the displacements are now imposed cyclically on the right point in one-dimensional bar in Figure \ref{Fig_Ch_geoF}c. The load-displacement curve under fatigue load is described in \ref{fat1} left, while homogeneous load response versus cyclic number with damage under displacement loading shown in \ref{fat1} right.
 
In order to enhance the Bayesian inference efficiency, we only select some critical points. In fact, as Figure \ref{fat2} depicts the effect of different material unknowns on the load-displacement is more tangible on the peak points and after the full fracture time. Therefore, instead of the entire points, only these points are used for the Bayesian framework. These points are illustrated in Figure \ref{fat1}.  

 \begin{figure}[!t]
	%\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/MCMC_E}} 
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/MCMC_k}}\\
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/MCMC_Gc}} 
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/MCMC_gamma}}
	\vspace{0.4cm}  
	\vspace{-0.4cm}
	\caption{Example 7. The evolution of the MCMC chains for different parameters.
	}
	\label{fat3}
\end{figure}








\begin{figure}[!t]
	%\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/post_E}} 
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/post_k}}\\
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/post_Gc}} 
	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/fatigue/post_gamma}}
	\vspace{0.4cm}  
	\vspace{-0.4cm}
	\caption{Example 7. The posterior density for different parameters. The true values are shown with a dashed green line.
	}
	\label{fat4}
\end{figure}		 		 

\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.7\textwidth]{Figures/fatigue/comp}} 
	\caption{Example 7. The load versus cyclic number curves of the homogeneous uniaxial tests under displacement loading using, true, inferred, and initial values.
	}
	\label{fat5}
\end{figure}	

We use the DRAM algorithm to identify the parameters. Figure \ref{fat4} shows the MCMC chains of the parameters where the acceptance rate is 3.3\% and all parameters converged. The initial values are $E^0=60\,000$, $k=0.4$, $G_c=0.3$, and $\gamma_c=0.0075$. The respective posterior densities are shown in Figure \ref{fat4}, and the medians are summarized in Table \ref{range7}. It seems that $E$ and $k$ are inferred correctly. However, the estimation of $G_c$ and $E$ is not sufficiently accurate. This probably due to the same effect of the energy parameters on the load-displacement curve that decreased the convergence rate. In fact, a similar effect causes to overestimation of $G_c$ and underestimation of $\gamma_c$ that probably balanced each other.
We use the inferred values (Table \ref{range7}) to calculate the diagram and compare the obtained values with initial values ($\theta^0$) and the reference values.  As Figure \ref{fat5} show, excluding the last peak point, other points are estimated correctly that show the relative accuracy of the model. 





			 			 		 
		 	 		 

==> MCFEM.tex <==
 


%%=======================================================================
\sectpa[Section3]{The stochastic phase-field fracture}
We consider a probability space $(\Omega, \mathbb{A},
\mathbb{P})$, where $\Omega$ indicates the set of elementary events (
the sample space), $\mathbb{A}$ is the $\sigma$-algebra of all possible
events, and $\mathbb{P}\colon \mathbb{A} \to [0,1]$ is a probability
measure. A real-valued random variable $\xi:\Omega\rightarrow\mathbb{R}$ is a set of possible events ($\Omega$), mapping the probability space to the real values. Here, we assumed that the random variable is Gaussian (has normal ditsribution), i.e. they have the following probability density function 
\begin{align}
	\mathbb{P}(\omega)=\frac{1}{\sqrt{2\pi\sigma^2}} \exp\frac{(\omega-\mu)^2}{2\sigma^2}.
\end{align}
For the Gaussian random variables, the probability density function considers two components, namely the mean value ($\mu$) and the variance ($\sigma$). Exceptionally, once we have $\mu=0$ and $\sigma=1$, we call the random variable, standard normal. Here, for a more realistic case, we use uniformly distributed random variables.



Now, we define an inner product $	\langle \xi,\zeta\rangle_{\mathcal{A}}=\mathbb{E}\left[ \xi\,\zeta\right]$ and the following Lebesgue space of the random variables with the finite variance
\begin{align}
	\mathcal{A}:=L_2(\Omega,\mathbb{R})=\{\xi:\Omega\rightarrow\mathbb{R}:~~\|\xi\|_{\mathcal{A}}^2:=	\langle \xi,\xi\rangle_{\mathcal{A}}=\mathbb{E}[\xi^2]<\infty\}.
\end{align}
Using the above-mentioned definition, we define the the covariance operator given by $\mathcal{COV}(\xi,\zeta):=\mathbb{E}\left[\left( \xi-\mathbb{E}[\xi]\right)\left( \zeta-\mathbb{E}[\zeta]\right)  \right]= \langle \xi-\mathbb{E}[\xi],\zeta-\mathbb{E}[\zeta] \rangle_{\mathcal{A}}$. Obviously, the variance function can be defined $\mathbb{V}(\zeta)=\mathcal{COV}(\zeta,\zeta)$. We can set the uncorrelated random variables when we have $\mathcal{COV}(\xi,\zeta)$=0.
A random variable $\xi(\boldsymbol{x},\omega):\Omega\times X\rightarrow \mathbb{R}$ is related to the spatial variable $\boldsymbol{x}\in X$ and the random variable $\xi\in\Omega$. Considering the fixed random variable $\omega\in\Omega$, $\xi(\omega,\cdot)$ indicates the deterministic cases, which is one observation in the phase-field problem (ductile/brittle).   
 
We denote a quantity of interest (QoI) as a function of $(\boldsymbol{u}, \varphi, \alpha) \in X\times X\times X$ (\todo{Amir: write the solution spaces}) shown by $\Delta (\boldsymbol{u}, \varphi, \alpha)$. Considering the randomness, we have the effect of the random variable on the solution, and then we have $\Delta (\boldsymbol{u} (\omega), \varphi (\omega), \alpha(\omega))$. Therefore, we normally compute the expectation of QoI denoting $\boldsymbol{\Delta}=\mathbb{E}\left[\Delta (\boldsymbol{u} (\omega), \varphi (\omega), \alpha(\omega))\right]$.
 
 
 
  In a Monte Carlo finite-element (FE) method several evaluations
 are combined   to obtain an approximation of the solution of
 the model equation or equations.
 Considering the Bochner space $L^2(\Omega;X)$ for the mappings $\mathcal{Y}\colon \Omega \to X$, we can define
 \begin{align}\label{bochner norm}
 	\| \mathcal{Y} \|_{L^2(\Omega;X)} :=\Big( \int_\Omega \| \mathcal{Y}(\cdot,\omega) \|_X^2 \,\P(\omega)
 	\Big)^{1/2}
 	= \E\Big[\| \mathcal{Y}(\cdot,\omega) \|_X^2 \Big]^{1/2}.
 \end{align}
Here, the variance function is given by $\mathbb{V} ( \mathcal{Y}) = \|\E[ \mathcal{Y}]- \mathcal{Y}\|_{L^2(\Omega;D)}^2$
 We consider the quantity of interest $\mathcal{X}$,  the standard MC estimator $\EMC$ for
 $\mathbb{E}[\mathcal{X}]$ is the sample mean
 \begin{equation}\label{MC-estimator}
 	\EMC[\mathcal{X}]
 	:= \frac{1}{M} \sum_{i=1}^{M} \mathcal{X}^{(i)},
 \end{equation}
 where $ \mathcal{X}^{(i)}$ is the $i$-th sample (independent random variable) of $ \mathcal{X}$. $\mathcal{X}$ is the function of ...............
 
 A perturbed (material) parameter can be defined using the perturbation value $\eta$ as
 \begin{align}
 	\chi=\bar{\chi}+\eta \tilde{\theta},
 \end{align}
where $\tilde{\theta}$ is a uniformly distributed random variable in [-1,\,1].

==> MCMC.tex <==
%=======================================================================
\sectpa[Section3]{Parameter estimation based on Bayesian inference }
\label{Bayesian}
%=======================================================================

 The estimation of the effective parameters in different deformation stages enables us to provide an accurate model which can predict the fracture behavior during all time steps precisely.
In this section we review the how efficient MCMC techniques can be used to provide accurate information of the material parameters. 
  As a probabilistic model, Bayesian inversion is used to update the available information (prior knowledge) and provide more accurate data (i.e., posterior density), which obtain an accurate estimation of the model parameters. As a result, a very good agreement between the measurement and the model response (as an aim of the inference) allows us to predict the deformation correctly.
  
  First of all, we define the following statistical model  
  \begin{align}
  \label{BE}
  \mathcal{S}=\mathcal{L}(\xx,\theta)+\varepsilon,
  \end{align}
  where $\mathcal{S}$ denotes an $n$-dimensional measurement/reference vector, $\mathcal{L}$ refers to the model response affected by the $k$-dimensional model parameters $\theta$ which belongs to the random field $\Theta$ and the position $\xx$, and $\varepsilon$ is the observation error (e.g., a Gaussian independent and identically distributed error $\varepsilon\sim\mathcal{N}(0,\sigma^2\,I)$, including the parameter $\sigma^2$.
  
 


In the Bayesian estimation, a parametric forward model (e.g., a PDE-based model) is used to update the available data (considered as random variables) based on the available information (denoting the prior knowledge).  Having a measurement $\ms=\mathtt{obs}$, the conditional density has the following form

\begin{align}
	\pi(\mathtt{obs})= \int_{\R^n}\pi(\mathtt{obs}|\theta)\pi_0(\theta)\,d\theta
\end{align}
Considering the parameter estimation setting, by a specific observation $m$, we strive to estimate the posterior distribution  $\pi(\theta|m)$, where a prior information is available.
Denoting the statistical model \eqref{BE}, the likelihood function can be estimated
\begin{align}\label{83}
\pi(\ms|\theta)=L(\theta,\sigma^2|\ms)=\frac{1}{(2\pi\sigma^2)^{n/2}}\exp\left(-\mathcal{EE}_\ms/2\sigma^2\right)
\end{align} 
where
\begin{align}\label{84}
\mathcal{EE}_\ms=\sum_{j=1}^{n}[\ms_j-\mathcal{L}_j(\xx,\theta)]^2
\end{align}
is the sum of square errors.

The random walk Metropolis (RWM) algorithm, introduced by Metropolis in 1953 \cite{metropolis1953equation}. The algorithm initials with a given initial guess $\chi^0$ according to the prior density. Then, based on the proposal distribution (the current state of the chain is perturbed randomly) a new candidate  that depends on the chain (the previous candidates) $\theta^{\star}$ is proposed. The acceptance rate is computed by
\begin{align}
\lambda(\theta^{j-1},\theta^{\star})=\min\left(1,\frac{\pi(\theta^{\star})}{\pi(\theta^{j-1})}\right),
\end{align} 
where the likelihood function is given in \ref{84}. Either the new candidate is accepted, or the MCMC chain follows in the current way. Here a symmetric proposal density is used. A generalized form of the algorithm using a non-symmetric introduced by Hastings \cite{hastings1970monte}, where the probability of the forward jump is not equal to the backward one. This algorithm has been widely used to estimate the desired distribution of the parameters, specifically when the problem dimensionality is low. In contrast, in the high-dimensional cased, the rejection rate increases dramatically. Furthermore, since the proposal density has no tunning, the convergence is significantly slow. It will be more pronounced when an unsuitable initial guess is used. Although the algorithm is easy to implement and versatile, its computational drawbacks (mostly in multi-dimensional domains) motivate the researchers to develop improvements to the Metropolis-Hastings (MH) algorithm. 

In the codes, we first determine a range for each parameter (based on the prior information). We assign an initial guess (prior knowledge) $\theta^0$ for the proposals. During the iterations ($j=2\,\cdots\,N$) the next proposal $\theta^\star$ is estimated as
\begin{align}
\label{prop}
\theta^\star=\theta^{j-1}+\mathcal{COV}*\text{randn(k,1)},
\end{align} 
where $\mathcal{COV}$ denotes the Cholesky decomposition of the given proposal function and $\text{randn(k,1)}$ is a $k$-dimensional normally distributed random variable. The function 
\begin{align}
\texttt{$\theta^\star$ = check\_bound($\theta^\star$,range)},
\end{align}
controls whether the new candidate is in the determined range or not. If each element of the proposal exceed the maximum value, this element is replaced with the upper bound. If the value is less than the minimum of the range, it will be replaced by the minimum. In the MH algorithm, the fixed (not adopted) covariance matrix is used during the MCMC chain. If the acceptance rate $\lambda$ is greater than a produced random variable between 0 and 1 (\texttt{rand}), the proposal is accepted, and the chain is followed with the new proposal. Otherwise, we continue with the previous candidate $\theta^{j-1}$. A summary of the relative algorithm is given in Algorithm 1.

 
 \begin{algorithm}[ht!]
 	\text{Initialization}: set prior data $\theta^0$ and number of samples $N$.\\[2mm]  
 		\textbf{while} $j<N$\\[2mm]
 			
 		\quad 1. Propose a new candidate based on the proposal distribution $\theta^{*}\sim\mathcal{K}(\theta^*|\,\theta^{j-1})$.    \\[2mm]
 		
 		% (i.e., the proposal distribution)\\
 		\quad  2. Compute the acceptance/rejection probability 
 		$$\upsilon (\theta^*|\,\theta^{j-1})=\min\left(1, \cfrac{\pi(\theta^*|\,m)}{\pi(\theta^{j-1}|\,m)}\,\cfrac{\mathcal{K}(\theta^{j-1}|\,\theta^*)}{\mathcal{K}(\theta^*|\,\theta^{j-1}))}\right).$$\\
 		
 		\quad 3. Generate a random number $\mathcal{R}\sim \text{Uniform}\,(0,1)$.\\[2mm]
 		
 		\quad 4.$~\textbf{if}~$ $\mathcal{V}<\upsilon~$ \textbf{then}\\ 
 		
 		\qquad\quad accept the proposed candidate $\theta^*$ and set $\theta^i:=\theta^*$\\
 		
 		\qquad \textbf{else}\\
 		
 		\qquad\quad reject the proposed candidate $\theta^*$ and set $\theta^{j}:=\theta^{j-1}$\\
 		
 		\qquad \textbf{end if}\\[2mm]
 		
 		\quad 5. Set $j=j+1.$
 	
 	\caption{The Metropolis-Hastings algorithm.} 
 	\label{algorithm}	
 \end{algorithm}
 
 
\sectpb[AM]{Adaptive Metropolis (AM)}\label{AM}
The adaptive Metropolis algorithm \cite{haario1999adaptive} is based on tuning the proposal density. This is done based on the obtained information from the previous samples (path of the MCMC chain) by computation of the covariance function.
According to the available information, we can adapt the the proposal distribution as
\begin{align}
V_j=K_p\text{Cov}\left(\theta^0,\theta^1\ldots,\theta^{j-1}\right)+\epsilon I_j.
\end{align}
Here the parameter $\epsilon$ is chosen close to zero to guarantee that the covariance is positive definiteness, and $K_p=\frac{2.38^2}{j}$ \cite{smith2013uncertainty}. The covariance function is given by
\begin{align}
\mathcal{COV}_j=\text{Cov}(\theta^0,\theta^1,\ldots,\theta^{j})=\frac{1}{j}\left(\sum_{i=0}^{j}
\theta^i\left(\theta^i\right)^T-(n+1)~\hat{\theta}^j\left(\hat{\theta}^j\right)^T\right),
\label{cov1}
\end{align}   
where $\hat{\theta}^j=\frac{1}{j+1}\sum_{i=0}^{j}\theta^j$ \cite{smith2013uncertainty}. To enhance the method efficiency, the proposal can be adapted 
after a specific number of iterations, e.g., 100. We propose the new proposal employing the Cholesky
decomposition of the covariance function \eqref{cov1}:
$$\theta^{*}=\theta^{j-1}+\mathcal{COV}_j\mathcal{I}_j,$$ 
where
$\mathcal{I}_j$ is the identity matrix. In contrast to \eqref{prop} we adopt the proposal iteratively (e.g., each 100 iterations). By using the updated proposal, the chain will have sufficient information from the accepted candidates which enhances the method efficiency. We use the code introduced in \cite{haario2006dram}, named \texttt{covupd}. Finally, the acceptance/rejection probability is estimated by
\begin{align}
\lambda_1 (\theta^*|\,\theta^{j-1})=\min\left(1, \cfrac{\pi(\theta^*|\,m)~\phi(\theta^{j-1}|~\theta^*)}{\pi(\theta^{j-1}|\,m)~\phi(\theta^*|\,\theta^{j-1}))}\right).
\end{align}


%=======================================================================
\sectpb[DR]{Delayed rejection (DR)}\label{DR}
%=======================================================================
 As we already mentioned, the MH algorithm suffers from computational disadvantages, mostly when we have a high-dimensional parameter space. 
 The delayed rejection \cite{green2001delayed} is based on giving another chance to the rejected candidate by using a second stage move. For this, we change the proposal density to increase the acceptance probability of the rejected candidate.
 The essential parameter is $\gamma_2$, which will be chosen less than one so that the next stage has a narrower proposal function (normally, $\gamma_2=1/5$ is chosen). The alternative proposal $\theta^{**}$ is chosen using the proposal function
 \begin{align}
 	\phi(\theta^{**}|\theta^{j-1},\theta^*)=\mathcal{N}(\theta^{j-1},\gamma_2^2 V_j),
 \end{align}
 where $V_j$ is the covariance matrix estimated by the adaptive algorithm \cite{green2001delayed}.
 We use the following acceptance ratio
\begin{align}\label{821}\nonumber
\lambda_2(\theta^{**}|\theta^{j-1},\theta^*)&:=\min\left(1,\frac{\pi(\theta^{**}|m) \phi(\theta^*|\theta^{**} ) \phi_2(\theta^{j-1}|\theta^{**},\theta^*) [1-\lambda(\theta^*|\theta^{**})]}{\pi(\theta^{j-1}|m) \phi(\theta^*|\theta^{j-1} ) \phi_2(\theta^{**}|\theta^{j-1},\theta^*) [1-\lambda(\theta^*|\theta^{j-1})]}\right)\\
&=\min\left(1,\frac{\pi(\theta^{**}|m) \phi(\theta^*|\theta^{**} )  [1-\lambda(\theta^*|\theta^{**})]}{\pi(\theta^{j-1}|m) \phi(\theta^*|\theta^{j-1} )  [1-\lambda(\theta^*|\theta^{j-1})]}\right).
\end{align}
The DR process can be implemented once, or a random/fixed number of iterations.


%=======================================================================
\sectpb[DRAM]{Delayed Rejection Adaptive Metropolis (DRAM)}\label{DRAM}
%=======================================================================
In the DRAM algorithm in order to reduce the rejected candidates and enhance the convergence we follow two steps. Globally, we adapt the proposal density based on the already obtained information from the chain (AM). Locally, we pursue the DR strategy that in each iteration, the rejected candidate will have at least one additional chance to the rejected proposal.
In the case that the initial values are too far from the desired density (target distribution), the adaptive strategy may not be started appropriately. It is due to the large variance of a near singular covariance matrix. As a solution, the DR strategy reduces the variance in different delayed stages, so some accepted proposals are available. They enable the AM to start appropriately. As seen, the DRAM technique can effectively overcome the drawbacks of the MH algorithm\cite{haario2006dram}. 
 A summary of the process is given in Algorithm 1. 
\begin{algorithm}[ht!]
	\vspace{0.2cm}
	\label{algorithm1}
	\textbf{Initialization ($j=0$)}: Produce the initial parameter $\theta^0\sim\pi(\theta^0|\,m)$.\\  
	
	
	
	
	\textbf{while~}{$j<N$}{
		\vspace{0.3cm}
		

		
		\quad 1. Propose a new candidate $\theta^{*}=\theta^{j-1}+\mathcal{R}_j\mathcal{Z}_j$  where $\mathcal{R}_j$ is the Cholesky decomposition \\
		
		\vspace{-0.3cm} ~~~~~~~of $\mathcal{V}_j$ and $\mathcal{Z}_j\sim$ Uniform (0, $I_j$) where $I_j$ denotes the identity matrix. \\
		% (i.e., the proposal distribution)\\
		
		
		
		
		
		\quad  2. Calculate the acceptance/rejection probability $\lambda_1 (\theta^*|\,\theta^{j-1})$.\\
		
		\quad 3. Draw a random number $\mathcal{R}\sim \text{Uniform}\,(0,1)$.\\
		
		\quad 4.$~\textbf{if}~$ $\mathcal{R}<\lambda_1~$ \textbf{then} ~~~accept the candidate $\theta^*$ and set $\theta^j=\theta^*$\\
		
		\qquad \textbf{else}~~~(i)  Calculate the alternative candidate
		\quad$\theta^{**}=\theta^{j-1}+\gamma_2^2\mathcal{R}_j\mathcal{Z}_j$.\\
		
		\hspace{1.85cm} (ii)   Calculate the acceptance/rejection probability $~~~\lambda_2 (\theta^{**}|\,\theta^{j-1},\theta^*) $.\\
		
		\vspace{-0.1cm}\hspace{1.85cm} (iii)  \textbf{if} ~$\mathcal{R}<\lambda_2$~~\textbf{then}\quad~~accept the candidate $\theta^{**}$ and set $\theta^{j}=\theta^{**}$\\
		
	\hspace{2.65cm}  \textbf{else}~~  reject the candidate $\theta^{**}$ and set $\theta^{j}=\theta^{j-1}$
		\qquad\quad\\
		
		\quad 5. Update the covariance matrix as $\mathcal{V}_j=\text{Cov}(\theta^0,\theta^1,\ldots,\theta^{j})$ and  $\mathcal{R}_j$.\\
		
				\quad 6. Set $j=j+1$.
	}
	\caption{The DRAM algorithm.}
\end{algorithm}
\\
The algorithm follows two important aspects
\begin{itemize}
	\item Increasing the acceptance rate by a local adaptation (DR).
	\item Increasing MCMC chain accuracy by a global adaptation (AM). 
\end{itemize}

\sectpb[kalman]{MCMC with ensemble-Kalman filter (EnKF-MCMC)}\label{kalman}
%Kalman-inspired proposal
As previously mentioned, a good detection of the proposal density will enhance the Markov chain movement to the target density. 
EnKF represents the error covariance matrix by a large stochastic ensemble of model realizations \cite{evensen2009ensemble}. In this method, to have an accurate estimation of posterior density, Kalman gain (similar to weighting matrix in particle filter) is calculated employing mean and covariance of prior distribution and cross-covariance between parameters and observations. 
%Performance of ensemble Kalman filter and Markov chain Monte Carlo under uncertainty in forecast model
Here, we introduce another proposal distribution detection technique using  a {\color{black}ensemble-Kalman filter}. The idea is based on using the Kalman filter \cite{kalman1960new} and we obtain
\begin{align}
	\theta^\star=\theta^{j-1}+\Delta \theta,
	\label{prop1}
\end{align}
where $\Delta \theta$ indicates the jump of Kalman-inspired proposal. For updating the proposed candidates, we can rewrite \eqref{prop1} as
\begin{align}
\Delta \theta=\mathcal{K}\left( y^{j-1}+s^{j-1}\right).
	\label{prop2}
\end{align} 
Here $\mathcal{K}$ points out the so-called Kalman gain,
\begin{align}
\mathcal{K}=\C_{\theta M}\left(\C_{MM}+\mathcal{R}\right)^{-1},
\end{align}
where $\C_{\theta M}$ denotes the covariance matrix between the identified unknowns and the PDE-based model, $\C_{MM}$ is the covariance matrix of the model solution (i.e., PDE response), and $\mathcal{R}$ indicates the measurement noise covariance matrix \cite{zhang2020improving}. Furthermore, $y^{j-1}$ indicates the residual of candidates with respect to the model.  Denoting $\texttt{obs}$ as an observation, $y^{j-1}=\texttt{obs}-f(\theta^{j-1})$ and  $s^{j-1}\sim\N(0,\mathcal{R})$, refers to the density of measurement. In order to enhance the method efficiency, i.e. reducing the effect of the initial guess different MCMC chains instead of a single chain can be employed. 

After the estimation of $\theta^\star$, we check its bounds, calculate its acceptance rate $\lambda$ that determines the new proposal is rejected, or chain should be continued with $\theta^{j-1}$.  
We summarized the procedure in Algorithm 2. The main advantage of EnKF-MCMC is using the covariance between the model response and between parameters and the PDE-response. This approach noticeably increases the possibility of the acceptance of the candidate.

 Table 1 provides an informative summary of the computational characteristics of the discussed MCMC techniques. MH algorithm shows a more efficient performance compared to RWM since an asymmetric proposal density is used. Also, the method is very simple for implementation. AM overcomes the drawback of MH by adapting the proposal based on the obtained information. DR method improves the AM specifically when the initial guess is not suitable and a local adaption is used. DRAM takes advantage of the benefits of both AM and DR (global and local chain adjustment). EnKF-MCMC has an effective proposal improvement and is significantly useful for high-dimensional unknowns. The theoretical results show that DRAM and EnKF will perform effectively compared to other methods. We will validate the aforementioned discussion with practical examples. 

\begin{table}[!t]
	\begin{tabular}{l |cccc}\hline
		method        & proposal & DR strategy& convergence& initial guess    \\[3mm]\hline\hline\\
		RWM \cite{metropolis1953equation}         & symmetric & -- & low-dimensional & sensitive    \\[3mm]\hline\\
		MH \cite{hastings1970monte} & asymmetric & -- & low-dimensional  &   sensitive   \\[3mm]\hline\\
		AM \cite{haario1999adaptive}           & global adaption & -- & high-dimensional & less-sensitive    \\[3mm]\hline\\
		DR-MH \cite{green2001delayed}         & local adaption & once/multiple &  high-dimensional & less-sensitive     \\[3mm]\hline\\
		DRAM \cite{haario2006dram}        & adaptive & once/multiple & high-dimensional & less-sensitive    \\[3mm]\hline\\
		EnKF-MCMC  \cite{evensen2009ensemble} ~~   & Kalman filter & -- & high-dimensional & less-sensitive     \\[3mm]\hline
	\end{tabular}\label{comp}
	\caption{A comparison of the computational features of different MCMC methods.}
\end{table}






%=======================================================================

 
%\sectpc{Convergence performance of the MCMC methods}
%Here, we introduced different effective MCMC techniques to estimate the parameters. In order to make a fair comparison between the methods, the convergence diagnostic tool can be employed to determine how many replications are needed to converges to the posterior distribution. For an accurate convergence different MCMC chains $m$ with different initial values (according to the prior density). 
%
%
%The $\hat{R}$-convergence tool \cite{brooks1998general,gelman1992inference} is an accurate diagnostic measure to observe the convergence of the Markov chain by comparing the between and within chain estimates for the unknowns and other univariate quantities of interest. Denoting the variance between the MCMC chain means by $V/N$ ($N$ is the length of the chain) and  the average of the within chain variances by $A$, the target variance is
%\begin{align}
%\mathcal{S}^2=(1-\frac{1}{N})A+\frac{V}{N}.
%\end{align}
% We compute the $\hat{R}$-statistics by
%\begin{align}
%\hat{R}=\frac{m+1}{m}\frac{\mathcal{S}^2}{A}-\frac{N-1}{m}.
%\end{align}
%
%
%%If the MCMC method converges appropriately, the chains are not affected by the starting point, and $\hat{R}$ reduces to 1. In other words, we can conclude that all chains are close to the target distribution \cite{brooks1998general}. In order to verify the method efficiency, a threshold can be defined, e.g., values less than 1.5 or 1.2 indicating a good convergence performance.
%% 
 

==> conclusion.tex <==
%=======================================================================
\sectpa[Section7]{Conclusion}
%=======================================================================

The implementation of the Bayesian inversion in different benchmark mechanical problems has been studied in this work. We compared the performance of different common MCMC techniques. Random-walk MCMC and MH can be used easily; however, they could not infer the unknowns in multi-dimensional cases. Using proposal adaptation and delayed rejection (global and local adaptation) improved the Bayesian inversion, which combing both gives rise to an effective MCMC technique. Employing the Kalman filter in Bayesian inference leads to the accurate estimation of the desired parameters. As observed, different material parameters can be estimated accurately and simultaneously using the probabilistic MCMC techniques. We presented a MATLAB package including all relative code alongside the manuscript.

In mechanical problems, the simultaneous and accurate inference of the parameters is crucial; otherwise, the estimation is not reliable. We conclude that DRAM and EnKF-MCMC are more suitable MCMC techniques for parameter estimation compared to other presented methods (although they are simpler). Using an ensemble Kalman filter leads to less fluctuation of MCMC in comparison with DRAM and more acceptance rate. Therefore, the posterior densities are relatively narrower indicating more reliable results.  
 

%=======================================================================
\subsection*{Acknowledgment}
%=======================================================================
N. Noii  and F. Aldakheel were founded by the Priority Program \texttt{DFG-SPP 2020} within its second funding phase. T. Wick and P. Wriggers were funded by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under Germany's Excellence Strategy within the Cluster of Excellence PhoenixD, \texttt{EXC 2122} (project number: 390833453). 
%=======================================================================



==> sec2.tex <==
%=======================================================================
\sectpa[Section2]{Phase-field modeling of ductile fracture in anisotropic elastic-plastic materials}
%=======================================================================

In this section, we summarize the material models considered for the phase-field approach to ductile fracture. Three models found in the literature are revisited and extended to anisotropic fracture, considering the case of transversely isotropic  materials. To this end, a unified formulation is first provided in sections~\ref{sec:basic_def}--\ref{sec:eq_general}. The three examined models are then recovered in sections~\ref{sec:model1}--\ref{sec:model3}. These models will be analyzed in subsequent sections using Bayesian inversion techniques, aiming for parameter identification in anisotropic elastic-plastic fracturing materials. 


% The formulation here is based on the minimization of a pseudo-potential energy for the coupled problem undergoing small strains. 

%=======================================================================
\sectpb[Section21]{State variables and kinematics}
\label{sec:basic_def}
%=======================================================================

Let us consider a solid domain $\calB\subset{\calR}^{\delta}$, where, generally, $\delta=3$, with boundary $\partial\calB$. We assume Dirichlet boundary conditions on $\partial_D\calB $ and Neumann boundary conditions on $\partial_N \calB := \Gamma_N \cup \mathcal{C}$, where $\Gamma_N$  denotes the outer domain boundary and $\calC\subset \calR^\delta$ is the crack boundary, as illustrated in Figure \ref{Figure1}a. % \ju[inline]{I changed $\calC\in\calR^{\delta-1}$ to $\calC\in\calR^\delta$. If I'm not mistaken, the boundary is a manifold of dimension $\delta-1$, but a subset of $\calB\subset\calR^{\delta}$. I also changed $\in$ to $\subset$. We can check this.}

The response of the fracturing solid at material points $\Bx\in\calB$ and time $t\in \calT = [0,T]$ is described by the displacement field $\Bu(\Bx,t)$ and the crack phase-field $d(\Bx,t)$ as
%
\begin{equation}
\Bu: 
\left\{
\begin{array}{ll}
\calB \times \calT \rightarrow \calR^\delta \\
(\Bx, t)  \mapsto \Bu(\Bx,t)
\end{array}
\right.
\AND
d: 
\left\{
\begin{array}{ll}
\calB \times \calT \rightarrow [0,1] \\
(\Bx, t)  \mapsto d(\Bx,t)
\end{array}
\right.
\WITH
\dot{d} \ge 0 .
\label{s2-fields}
\end{equation}
%
Intact and fully fractured states of the material are characterized by $d(\Bx,t)=0$ and $d(\Bx,t)=1$, respectively. The fracture surface $\mathcal{C}$ is approximated in $\calB_L\subset\calB$, the so-called \textit{local domain}. The intact region with no fracture is denoted
as the \textit{complementary domain} $\calB_C:=\calB \backslash \calB_L\subset\calB$, such that ${\calB}_C\cup{\calB}_L=\calB$ 
and ${\calB_C}\cap{\calB_L}=\varnothing$. We note that $\calB_L$,
i.e., the domain in which the smeared crack phase-field is approximated, and its boundary $\partial \calB_L$, depend on the choice of the phase-field regularization parameter $l_f>0$. With the purpose of stating variational principles, we let $\Bu\in\mathbf{V}$ and $d\in \mathrm{W}_{d}$, where $\mathbf{V}$ and $\mathrm{W}_{d}$ denote suitable function spaces given by
%
\begin{equation}
\begin{aligned}
\mathbf{V}(\overline{\Bu})&:=\{\Bu\in\mathbf{H}^1(\calB;\calR^\delta) \ \colon \ \Bu=\overline{\Bu} \ \text{on} \ \partial_D\calB\}, \\
\mathrm{W}_{d}(d_n)&:=\{d\in\mathrm{H}^1(\calB;[0,1]) \ \colon \ d \geq d_n \},
\end{aligned}
\label{eq:spaces_u_d}
\end{equation}
%
where $d_n$ is the damage value in a previous time instant. Note that $\mathrm{W}_{d}$ is a non-empty, closed and convex subset of $\mathrm{H}^1(\calB)$, whose definition introduces the evolutionary character of the phase-field and incorporates an irreversibility condition in incremental form. % \ju[inline]{I used the notation in Eq.~\ref{eq:spaces_u_d} for the function spaces because it is convenient for subsequent statements. For instance, we can later define the admissible variations as $\delta\Bu\in\mathbf{V}(\mathbf{0})$ and ${\delta d\in \mathrm{H}^1(\calB;\calR_+)}$. It also helps in defining function spaces for the plastic variables later. Of course, you can change to the notation you prefer.}


Focusing on the isochoric setting of von Mises plasticity theory, we define the plastic strain tensor $\Bve^p(\Bx,t)$ and the hardening variable $\alpha(\Bx,t)$ as
%
\begin{equation}
\Bve^p: 
\left\{
\begin{array}{ll}
\calB \times \calT \rightarrow \calR^{\delta\times\delta}_{dev} \\
(\Bx, t)  \mapsto \Bve^p(\Bx,t)
\end{array}
\right.
\AND
\alpha: 
\left\{
\begin{array}{ll}
\calB \times \calT \rightarrow \calR_+ \\
(\Bx, t)  \mapsto \alpha(\Bx,t)
\end{array}
\right.
\WITH
\dot{\alpha} \ge 0 ,
\label{s2-fields}
\end{equation}
%
where $\calR^{\delta\times\delta}_{dev}:=\{\Be\in\calR^{\delta\times\delta} \ \colon \ \Be^T=\Be,\ \tr{[\Be]}=0\}$ is the set of symmetric second-order tensors with vanishing trace. The plastic strain tensor is considered as a local internal variable, while the hardening variable is a possibly non-local internal variable. In particular, $\alpha$ may be introduced to incorporate phenomenological hardening responses and/or non-local effects, for which the evolution equation 
%
\begin{equation}
\dot\alpha = \sqrt{\frac{2}{3}}\vert\dot{\Bve}^p\vert
%\WITH
%\dot\alpha \ge 0
\label{s2-evol-alpha}
\end{equation}
%
is considered. As such, $\alpha$ can be viewed as the equivalent plastic strain, which starts to evolve from the initial condition $\alpha(\Bx,0) = \mathit{0}$. In this work the elastic-plastic material behavior is considered in both the {\it complimentary domain} and the {\it local domain}, whereas the fracture response lives locally at the lower scale $\calB_L$. Concerning function spaces, we assume sufficiently regularized plastic responses, i.e., endowed with hardening and/or non-local effects, for which we assume $\Bve^{p}\in\mathbf{Q}:=\mathrm{L}^2(\calB;\calR^{\delta\times\delta}_{dev})$. Moreover, in view of Eq.~\eqref{s2-evol-alpha}, it follows that $\alpha$ is irreversible, such that, in an incremental context, $\alpha\in \mathrm{W}_\alpha$, with 
%%
%\begin{equation}
%\mathrm{W}_\alpha(\alpha_n):=\{\alpha\in\mathrm{H}^1(\calB;\calR_+) \ \colon \ \alpha \geq \alpha_n\} \.
%\end{equation}
%
\begin{equation}
\mathrm{W}_\alpha(\Bve^p-\Bve^p_n,\alpha_n):=\{\alpha\in\mathrm{H}^1(\calB;\calR_+) \ \colon \ \alpha = \alpha_n + \sqrt{2/3}\vert \Bve^p - \Bve^p_n \vert\}.
\label{Walpha}
\end{equation}

\ju[inline]{Should we omit the concept of local domain here?}

%Suitable function spaces for the plastic variables are relevant for the gradient plasticity model presented in Sec.~\ref{sec:model3}, and will thus be defined therein.

\begin{figure}[!t]
	\centering
	{\includegraphics[clip,trim=0cm 6.5cm 0cm 1cm, width=15cm]{Figures/geo1.pdf}}  %left, bottom, right and top 
	\caption{ Setup of the notation. (a) Global Cartesian coordinate system with unit vectors
		$(\bm{e}_{\bm{x}},\bm{e}_{\bm{y}})$ and local orthogonal principal
		material coordinates corresponding to the first and second families of fibers $(\bm{a},\bm{g})$, (b) solid with a crack inside of a plastic zone and boundary conditions, and (c) tangential and unit vectors denoted by $(\bm{n}_L, \bm{n}_\mathcal{C})$ at the crack tip point $\bm{x}$.}
	\label{Figure1}
\end{figure}

The gradient of the displacement field defines the symmetric strain tensor of the geometrically linear theory as
\begin{equation}
\Bve = \nabla_s \Bu = \sym[ \nabla \Bu ] := \frac{1}{2} [\nabla\Bu + \nabla\Bu^T]
.
\label{s2-disp-grad}
\end{equation}
%
In view of the small strain hypothesis and the isochoric nature of the plastic strains, the strain tensor is additively decomposed into an elastic part $\Bve^e$ and a plastic part $\Bve^p$ as
%
\begin{equation}
\Bve = \Bve^e + \Bve^p 
\WITH
\tr{[\Bve^p]} = 0
\AND
\tr{[\Bve]} = \tr{[\Bve^e]}
.
\label{s2-strain-e-p}
\end{equation}

%\ju[inline]{I usually use $\calR^{\delta\times\delta}_{dev}$ for the set symmetric deviatoric tensors. We can change it as you prefer. Maybe $\dev(\calR^{\delta\times\delta})$?}

For simplicity, the anisotropic material is assumed to be strengthened by a single family of fibers, whose direction is described by a unit vector field $\Ba$ (Figure~\ref{Figure1}). Consequently, the direction-dependent response is characterized by the second-order structural tensor
%
\begin{equation}
\BM:=\Ba\otimes\Ba .
\end{equation}
%
%We note the introduction of additional preferred directions can be easily incorporated

The solid $\calB$ is loaded by prescribed deformations and external tractions on the boundary, defined by time-dependent Dirichlet conditions and Neumann conditions
%
\begin{equation}
\Bu = \overline{\Bu} \ \textrm{on}\ \partial_D\calB
\AND
\Bsigma \cdot \Bn 
= \overline{\Btau} \ \textrm{on}\ \partial_N\calB ,
\label{s2-bcs}
\end{equation}
%
where $\Bn$ is the outward unit normal vector on the surface $\partial \calB$. The stress tensor $\Bsigma$ is the thermodynamic dual to $\Bve$ and $\bar{\Btau}$ is the prescribed traction vector. Finally, the stress equilibrium is defined as the quasi-static form of the balance of linear momentum
% 
\begin{equation}
\div\,\Bsigma + \overline\Bf = \Bzero,
\label{s2-equil:defo}
\end{equation}
where dynamic effects are neglected and $\overline\Bf$ is a given body force. 

%Following the Coleman-Noll procedure, the stress tensor is obtained from the potential ${W}_{elas}$ in \req{elas-part_m1} by
%\begin{equation}
%\Bsigma := \partial_{\Bve^e} {W}_{elas}
%= g(d) \widetilde\Bsigma_{+} + \widetilde\Bsigma_{-}
%\WITH
%\widetilde\Bsigma_{\pm} = \kappa \langle\mbox{tr}[\Bve^e]\rangle_{\pm} \Bone 
%+ 2 \mu \dev(\Bve^e_\pm)
%\label{vari-bf-23}
%\end{equation}
%%
%where $\widetilde\Bsigma$ is the effective stress tensor.

\sectpb[Section22]{Energy quantities and variational principles}
\label{sec:energy_functions}

Let $\BfrakC$ denote the set of constitutive state variables. In the most general setting considered in this study, one has
% \mbox{Constitutive State Variables}\;
\begin{equation}
\BfrakC := \{ \Bve, \Bve^p, \alpha, d, \nabla \alpha, \nabla d \}
.
\label{state}
\end{equation}
%
A pseudo-energy density per unit volume is then defined as $W:=W(\BfrakC)$, which is additively decomposed into an elastic contribution $W_{elas}$,  a plastic contribution $W_{plas}$, and a (regularized) fracture contribution~$W_{frac}\;$:
%
\begin{equation}
\boxed{W(\BfrakC;\BM):= {W}_{elas}(\Bve,\Bve^p ,d ,\alpha;\BM) + {W}_{plas}(\alpha, d, \nabla \alpha) +
{W}_{frac}(d, \nabla d ; \BM) . } 
\label{psuedo-energy}
\end{equation}
%
%\ju[inline]{Should we split into energetic and dissipative contributions instead?}
%\ju{Maybe a remark/footnote is needed here.}
We note that $W$ is a state function that contains both energetic and dissipative contributions. With this function at hand, a pseudo potential energy functional can be written~as
% Then, the development of a Bayesian inversion framework for the phase-field modeling of elastic-plastic fracturing materials can the following pseudo potential density functional as a point of departure:
%\boxed{
\begin{equation}
	\calE(\Bu,\Bve^p,\alpha,d;\BM) := \int_{\calB} {W}(\BfrakC;\BM) \, dv 
	 \; - \; 
	\vphantom{\frac{d}{dt}}
	\mathcal{E}_{ext} (\Bu) , 
\label{potential-functional}
\end{equation}
% }
where $\mathcal{E}_{ext}$ denotes the work of external loads: %
%
\begin{equation}
	\mathcal{E}_{ext} (\Bu) := 
	\int_{\calB} \overline\Bf \cdot \Bu\, dv  +
	\int_{\partial_N\calB} \overline{\Btau} \cdot \Bu\, da.
\end{equation}

In \textit{variationally consistent models}, the governing equations of the fracturing elasto-plastic solid can be derived from knowledge of the energy functional~\eqref{potential-functional} by invoking rate-type variational principles~\citep{miehe2011,miehe2016aphase} in agreement with the principle of virtual power~\citep{maugin1990,fremond1996}. In such cases, a global rate potential of the form 
%
\begin{equation}
	\Pi(\dot\Bu,\dot\Bve^p,\dot\alpha,\dot{d};\BM) := \frac{d}{dt}\calE(\Bu,\Bve^p,\alpha,d;\BM) \; + \; \int_\calB \Phi_{vis} (\dot{d},\dot{\alpha}) \, dv   
\label{potential-functional-cont}
\end{equation}
%
is defined, where ${\Phi}_{vis}$ denotes the dissipative power density due to viscous resistance forces. In line with previous works~\citep{miehe+welschinger+hofacker10a,miehe2016aphase}, the function
%
\begin{equation}
{\Phi}_{vis} (\dot{d},\dot{\alpha}) := \frac{\eta_f}{2}\dot{d}^{\,2} + \frac{\eta_p}{2}\dot{\alpha}^2 ,
\label{Dvis}
\end{equation}
%
is considered, where $\eta_f$ and $\eta_p$ are material parameters that characterize the viscous response of the fracture and plasticity evolutions, respectively. Then, minimization of~\eqref{potential-functional-cont} with respect to $\dot\Bu$, the plasticity variables $(\dot\Bve^p,\dot\alpha)$ subject to the hardening law~\eqref{s2-evol-alpha}, and the crack phase-field $\dot d$ subject to the irreversibility condition $\dot d\geq0$ provide the governing equations for the elasticity problem, the plasticity problem, and the fracture problem, respectively. Such a variational structure results in a convenient numerical implementation based on incremental energy minimization, for which an algorithmic representation of the energy functional~\eqref{potential-functional} is defined as
%
\begin{equation}
	\Pi^\tau(\Bu,\Bve^p,\alpha,d;\BM) := \calE(\Bu,\Bve^p,\alpha,d;\BM) \; - \; \calE_n \; + \; \Delta  t\int_\calB  \Phi_{vis} \big([d-d_n]/\Delta t,[\alpha-\alpha_n)/\Delta t\big) \, dv  ,  
\label{potential-functional-disc}
\end{equation}
%
where $\Delta t:=t-t_n$ denotes the time step. The coupled evolution problem then follows as the incremental minimization principle
%
\begin{equation}
\boxed{ \{\Bu,d,\alpha,\Bve^p\} = \arg\big\{ \min_{\Bu\in\mathbf{V}(\overline{\Bu})} \ \min_{d\in\mathrm{W}_{d}(d_n)} \ \min_{\{\alpha,\Bve^p\}\in\mathrm{W}_{\alpha}(\Bve^p-\Bve^p_n,\alpha_n)\times\mathbf{Q}}  \, \Pi^\tau(\Bu,\Bve^p,\alpha,d;\BM)  \big\} . }
\label{inc_min}
\end{equation}
% This functional is minimized with respect to $\Bu\in\mathbf{V}$, the plasticity variables $(\Bve^p,\alpha)\in\mathrm{L}^2(\calB;\calR^{\delta\times\delta}_{dev})\times \mathrm{W}_\alpha$, and the crack phase-field $d\in \mathrm{W}_d$ to obtain the governing equations in incremental form. Note that the evolution constraints for the internal variables are embedded in their corresponding function spaces.
%

\begin{Remark} From equation~\eqref{Dvis}, it is clear that the rate-independent case is recovered by letting $\eta_f\to0$ and $\eta_p\to0$.  In this case, the coupled evolution problem can be equivalently derived in variational form using the energetic formulation for rate-independent systems~\citep{mielke2006,mielke2015}, based on notions of energy balance and stability. This path is followed, for instance, in references~\cite{pham2010,marigo2016,alessi2015,alessi2017,rodriguez2018,ulloa2021}. Moreover, the fact that \eqref{psuedo-energy} is a state function implies that the incremental rate-independent problem exactly recovers the continuous counterpart.
\end{Remark}


In summary, in fully variational models, it suffices to define the constitutive energy density functions $W_{elas}$, $W_{plas}$, and $W_{frac}$ to establish the multi-field evolution problem in terms of~\eqref{inc_min}. As we shall recall in the sequel, such a variational structure is not always present in phase-field models for ductile fracture, resulting in greater flexibility at the cost of  a convenient mathematical structure.

%=======================================================================
\sectpc{Elastic contribution}
%=======================================================================
The elastic energy density $W_{elas}$ is expressed in terms of the effective strain energy density $\psi_e$. For transversely isotropic materials, $\psi_e$ may be defined in terms of the elastic strain tensor $\Bve^e$ and the structural tensor $\BM$. In particular, $\psi_e$ admits the additive decomposition 
%
\begin{equation}
\psi_e(\Bve^e;\BM)=\psi_e^{iso}\big(I_1(\Bve^e),I_2(\Bve^e)\big) + \psi_e^{aniso}\big(I_4(\Bve^e;\BM)\big) .
\label{eq:strainenergy}
\end{equation}
%
The isotropic strain energy function reads
%
\begin{equation}
\psi_e^{iso}\big(I_1(\Bve^e),I_2(\Bve^e)\big):=\frac{\lambda}{2}I_1(\Bve^e)^2+\mu I_2(\Bve^e) ,
\label{eq:psi_iso}
\end{equation}
%
where $\lambda$ and $\mu$ are the elastic Lam\'e constants, and $I_1$ and $I_2$ denote the invariants
%
\begin{equation}
I_1(\Bve^e)=\tr[\Bve^e] \AND I_2(\Bve^e)=\tr[(\Bve^e)^2] .
\label{eq:prin_invar}
\end{equation}
%
On the other hand, the anisotropic strain energy function reads
%
\begin{equation}
\psi_e^{aniso}\big(I_4(\Bve^e;\BM)\big):=\chi_a I_4(\Bve^e;\BM)  ,
\label{eq:psi_aniso}
\end{equation}
%
where $\chi_a$ is a penalty-like parameter characterizing the anisotropic deformation response with preferred direction $\Ba$, and $I_4$ denotes the \emph{pseudo-invariant}
%
\begin{equation}
I_4(\Bve^e;\BM)=\tr[\Bve^e\cdot\BM]  .
\label{eq:pseudo_invar}
\end{equation}

In order to preclude fracture in compression, a decomposition of the effective strain energy density into \textit{damageable} and \textit{undamageable} parts is employed, such that the isotropic contribution admits the following form:
%
\begin{equation}
\psi_e^{iso}\big(I_1(\Bve^e),I_2(\Bve^e)\big)=\psi_e^{iso,+}(I_1^{+},I_2^+)+\psi_e^{iso,-}(I_1^{-},I_2^-)
\end{equation}
%
where
%
\begin{equation}
I_1^{\pm}:=\langle I_1(\Bve^e)\rangle_\pm \AND I_2^{\pm}:=I_2(\Bve^{e}_\pm) .
\label{split_inviso}
\end{equation}
%
Extending this notion to the anisotropic contribution (see also~\cite{noii2020bayesian}), we consider the split
%
\begin{equation}
\psi_e^{aniso}\big(I_4;\BM\big)=\psi_e^{aniso,+}(I_4^+)+\psi_e^{aniso,-}(I_4^-) ,
\end{equation}
%
where
%
\begin{equation}
I_4^{\pm}:=\langle I_4(\Bve^e;\BM)\rangle_\pm .
\label{split_invaniso}
\end{equation}
%
In equations~\eqref{split_inviso} and~\eqref{split_invaniso}, $\langle x \rangle_\pm := (x \pm \vert
x\vert)/2$ denote ramp functions of $\calR_\pm$, while the positive and negative elastic strain tensors are defined as $\Bve^e_+ := \hbox{$\sum_{a=1}^3$} \langle\varepsilon^e_a
\rangle_+\;\Bn_a \otimes \Bn_a$ and $\Bve^e_- := \Bve^e -
\Bve^e_+$. Here, $\{\varepsilon^e_a\}_{a=1,2,3}$ are the principal strains and $\{\Bn_a\}_{a=1,2,3}$ are the principal strain directions.

The elastic contribution to the pseudo-energy density~\eqref{psuedo-energy} finally reads
%
\begin{equation}
\begin{aligned}
{W}_{elas}(\Bve,\Bve^p,d,\alpha;\BM):= g_e(d,\alpha) \; \big[ \psi_e^{iso,+}(I_1^+,I_2^+)&+\psi_e^{aniso,+}(I_4^+) \big ] \\ &+ \psi_e^{iso,-}(I_1^-,I_2^-)+\psi_e^{aniso,-}(I_4^-) ,
\end{aligned}
\label{elas-part}
\end{equation}
%
where $g_e(d,\alpha)$ is the \textit{elastic degradation function}. Following the Coleman-Noll procedure, the stress tensor is obtained from the potential ${W}_{elas}$ in \req{elas-part} as
%
\begin{equation}
\begin{aligned}
&\Bsigma = \partial_{\Bve^e} {W}_{elas} = \Bsigma^{iso} + \Bsigma^{aniso} \WITH \\
&\Bsigma^{iso}=g_e(d,\alpha)\widetilde\Bsigma^{iso}_{+}+\widetilde\Bsigma^{iso}_{-} \AND  \Bsigma^{aniso}=g_e(d,\alpha)\widetilde\Bsigma^{aniso}_{+}+\widetilde\Bsigma^{aniso}_{-} ,
\end{aligned}
\label{stress}
\end{equation}
%
where $\widetilde\Bsigma^{iso}$ and $\widetilde\Bsigma^{aniso}$ are the effective stress tensors, given by
%
\begin{equation}
\begin{aligned}
&\widetilde\Bsigma^{iso}_{\pm} := \partial_{\Bve^e} \psi_e^{iso,\pm} = \kappa \langle\mbox{tr}[\Bve^e]\rangle_{\pm} \Bone 
+ 2 \mu \dev(\Bve^e_\pm) \AND \\ 
&\widetilde\Bsigma^{aniso}_{\pm} := \partial_{\Bve^e} \psi_e^{aniso,\pm} = \beta_a I_4^\pm\BM ,
\end{aligned}
\end{equation}
%
where $\kappa$ is the bulk modulus.
% From the above definitions, it remains to define the elastic degradation function $g_e(d,\alpha)$. The specific choice of degradation will depend on the specific model.

% To this end, we consider two alternative formulations that are widely used in the literature...  volumetric-deviatoric split~\citep{amor2009}... spectral decomposition~\citep{miehe+welschinger+hofacker10a}
 
%\ju[inline]{I neglected $I_6$, $I_5$ and $I_7$ for simplicity ($\Xi_a=\Xi_g=0$). Will they be considered? If not, should we add a remark?} 
%======================================================================= 
\sectpc{Fracture contribution} 
%=======================================================================
The phase-field contribution $W_{frac}$ is expressed in terms of the crack surface energy density $\gamma_l$ and the fracture length scale parameter $l_f$ that governs the regularization. In particular, the sharp-crack surface topology $\calC$ is regularized by a functional $\calC_l$, as outlined in~\cite{aldakheel16} and~\cite{miehe+hofacker+schaenzel+aldakheel15}. This geometrical perspective is in agreement with the framework of~\cite{bourdin2000numerical}, which was conceived as a $\Gamma$-convergence regularization of the variational approach to Griffith fracture~\cite{francfort1998revisiting}. For the case of isotropic materials, the regularized functional~reads
%
\begin{equation}
\calC_l(d) = \int_{\calB} \gamma_l(d, \nabla d) \, dv .
\label{s2-gamma_l}
\end{equation}
%%\WITH
%\gamma_l(d, \nabla d) =  
%\dfrac{1}{2l_d} d^2 + \dfrac{l_d}{2} \vert \nabla d %\vert^2. 
In this work, following~\cite{noii2020adaptive,noii2020bayesian}, anisotropic effects are introduced by means of the structural tensor $\BM$. In particular, we assume that $\gamma_l$ admits the additive decomposition 
%
\begin{equation}
\gamma_l(d, \nabla d;\BM) = \gamma_l^{iso}(d, \nabla d)+\gamma_l^{aniso}(d, \nabla d;\BM) .
\end{equation}
%
In line with standard phase-field models, a general surface density function for the isotropic part $\gamma_l^{iso}$ is defined as 
%
\begin{equation}
\gamma_l^{iso}(d, \nabla d):=\frac{1}{c_f}\, \bigg(\frac{\omega(d)}{l_f} + l_f \nabla d \cdot \nabla d \bigg) \WITH c_f:=4\int_0^1\sqrt{\omega(b)}\,db ,
\end{equation}
%
where $\omega(d)$ is a monotonic and continuous \emph{local fracture energy function} such that $\omega(0)=0$ and  $\omega(1)=1$. A variety of suitable choices for $\omega(d)$ are available in the literature~\citep{kuhn2015,wu2017,wu2018}. Here, the widely adopted linear and quadratic formulations are considered, which yield, respectively, models with and without an elastic stage. Specifically, we define 
%
\begin{equation}
\omega(d) : = \begin{cases}  d\phantom{^2} \implies c_f=8/3 \quad &\text{model with an elastic stage}, \\ d^2 \implies c_f=2 \quad &\text{model without an elastic stage}.  \end{cases}
\label{wd}
\end{equation}
%
On the other hand, the anisotropic part $\gamma_l^{aniso}$ reads
%
\begin{equation}
\gamma_l^{aniso}(d, \nabla d;\bm{M}):=\beta_a\dfrac{l_f}{c_f} \nabla d \cdot \bm{M} \cdot \nabla d  .
\end{equation}

Finally, the fracture contribution to the pseudo-energy density~\eqref{psuedo-energy} reads
%
\begin{equation}
\begin{aligned}
{W}_{frac}(d, \nabla d ; \BM):= g_f \gamma_l(d, \nabla d;\BM),
\end{aligned}
\label{frac-part}
\end{equation}
%
where $g_f$ is a parameter that allows to recover different models found in the literature, as will become apparent in the sequel.

% \ju[inline]{Maybe we should add more references for similar anisotropic fracture approaches.} 
%=======================================================================
\sectpc{Plastic contribution}
%=======================================================================
The plastic contribution $W_{plas}$ is expressed in terms of an effective plastic energy density $\psi_p$, whose form will depend on the adopted phenomenological model. In line with previous works~\citep{miehe2016aphase,miehe2017phase,rodriguez2018,ulloa2021} let us consider a function in the context of gradient-extended von Mises plasticity:   
%
\begin{equation}
{\psi}_{p}(\alpha,\nabla\alpha) := \sigma_Y\; \alpha + \frac{H}{2} \alpha^2 + \frac{\sigma_Y}{2}\,l_p^2\nabla\alpha\cdot\nabla\alpha ,
\label{psi_p}
\end{equation}
%
with the initial yield stress $\sigma_Y$, the isotropic hardening modulus $H\ge 0$ and the \emph{plastic length scale} $l_p$.
%
The plastic contribution to the pseudo-energy density~\eqref{psuedo-energy} then reads
%
\begin{equation}
\begin{aligned}
{W}_{plas}(\alpha,d ,\nabla \alpha):= g_p(d) {\psi}_{p}(\alpha,\nabla\alpha),
\end{aligned}
\label{plas-part}
\end{equation}
%
where $g_p(d)$ is the \textit{plastic degradation function}. The models presented in sections~\ref{sec:model1} and~\ref{sec:model2} are restricted to local plasticity, for which $l_p=0$, while the model presented in Sec.~\ref{sec:model3} will include non-local effects, with $l_p>0$. The plastic energy density can be further decomposed into energetic and dissipative parts:
%
\begin{equation}
\begin{aligned}
&{W}_{plas}(\alpha,d ,\nabla \alpha)={W}_{plas}^{ener}(\alpha ,d,\nabla \alpha) + {W}_{plas}^{diss}(\alpha,d)    \WITH \\
&{W}_{plas}^{ener}(\alpha,\nabla \alpha,d):=g_p(d) \frac{1}{2}\big(H\alpha^2 + \sigma_Y\,l_p^2\nabla\alpha\cdot\nabla\alpha\big) \AND {W}_{plas}^{diss}(\alpha,d):=g_p(d)\sigma_Y\alpha .
\end{aligned}
\label{plas-part_ener_diss}
\end{equation}
%


%\ju[inline]{Will we consider extending this to anisotropic gradient plasticity? As once discussed with Nima, perhaps it would be an idea to consider, in analogy with the phase-field treatment below, $\psi_p(\alpha,\nabla\alpha;\BM,\BG)$, maybe including terms like $\beta_{a}^{p}\frac{l_p^2}{2}\nabla\alpha\cdot\BM\cdot\nabla\alpha$ + $\beta_{g}^{p}\frac{l_p^2}{2}\nabla\alpha\cdot\BG\cdot\nabla\alpha$. On the other hand, it's more parameters...} 

% \ju[inline]{There's an issue here: $\psi_p$ is a pseudo-effective energy in models 1 and 2, containing both free energy and dissipation. In model 3, $\psi_p$ is free energy only. Maybe we can call the free energy $\Psi_p$, but then...}

\sectpb{Stationarity conditions and governing equations}
\label{sec:eq_general}

Let us now derive the \emph{variationally consistent} equations for the multi-field coupled problem. To this end, we seek to find the stationarity conditions for the minimization problem~\eqref{inc_min}. The models presented in sections~\ref{sec:model1}--\ref{sec:model3} shall take the developments below as a canonical forms, and will then deviate from the variationally consistent expressions in favor of greater flexibility.

%\subsubsection*{Elasticity}
\sectpc{Elasticity}

The minimization with respect to the displacement field in the variational principle~\eqref{inc_min} yields 
%
%
\begin{equation}
\calE_\Bu(\Bu,\Bve^p,\alpha,d;\delta\Bu)=\int_\calB\big[\Bsigma:\Bve(\delta\Bu)-\overline{\Bf}\cdot\delta\Bu\big]\,dv - \int_{\partial\calB_N}\overline{\Btau}\cdot\delta\Bu\,da =0 \quad \forall \,\delta\Bu\in\mathbf{V}(\bm{0}) , 
\label{equil_weak}
\end{equation}
which corresponds to the weak for of the mechanical balance equations~\eqref{s2-bcs} and $V(0)$ points out the function space for the virtual displacement fields, i.e., with homogeneous kinematic boundary conditions.
%=======================================================================
%\subsubsection*{Fracture}
\sectpc{Fracture}
%=======================================================================

The directional derivative of~\eqref{potential-functional} with respect to the crack phase-field can be written as
%
\begin{equation}
\begin{aligned}
\calE_d(\Bu,\Bve^p,\alpha,d;\delta d)=\int_\calB \bigg[ \bigg( & \partial_d \; g_e(d,\alpha)\big[\psi_e^{iso,+} + \psi_e^{aniso,+}\big]   \\ & + \frac{g_f}{c_f l_f} \omega'(d) + \partial I_+(d-d_n) + g_p'(d)\psi_p + \frac{\eta_f}{\Delta t} (d-d_n)  \bigg)\delta d  \\ & \hspace*{1cm} +  2\frac{g_f}{c_f} l_f \big( \nabla d \cdot \nabla (\delta d) + \beta_a\nabla d \cdot \BM \cdot \nabla (\delta d) \big) \bigg]\,dv \ni 0 \\ &  \hspace*{7.5cm} \forall \,\delta d\in W_d(0) ,
\end{aligned}
\label{phf_weak}
\end{equation}
%
where the indicator function $I_+\colon \calR \to \calR \cup \{+\infty\}$ has been introduced to impose the irreversibility condition embedded in $d\in\mathrm{W}_d(d_n)$. Let us now define the fracture yield function
%
\begin{equation}
f_d:=- \partial_d \; g_e(d,\alpha)\big[\psi_e^{iso,+} + \psi_e^{aniso,+}\big] - g_p'(d)\psi_p   - g_f\delta_d\gamma_l  . 
\label{phf_yield}
\end{equation}
%
The strong form of~\eqref{phf_weak} can then be written as
%
\begin{equation}
\begin{aligned}
-f_d + \frac{\eta_f}{\Delta t} (d-d_n)+ \partial I_+(d-d_n) \ni 0  \WITH  (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB . 
\end{aligned}
\label{phf_strong}
\end{equation}
Recalling that  
%
\begin{equation}
\partial I_+(d-d_n)=\begin{dcases}\{0\} & \text{if}  \quad d>d_n  , \\
\calR_-  & \text{if}  \quad d=d_n , \\
\varnothing &  \text{otherwise} , 
\end{dcases}
\label{subdiff_ind}
\end{equation}
%
the strong form yields, for the rate-dependent case, the evolution equation
%
\begin{equation}
\frac{\eta_f(d-d_n)}{\Delta t} = f_d \geq 0 \WITH  (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB .
\label{phf_strong_rdep}
\end{equation}
%
On the other hand, for the rate-independent case, we obtain the KKT conditions 
%
\begin{equation}
\begin{aligned}
f_d \leq 0 , \quad (d-d_n)f_d=0   \AND d-d_n\geq0 , \WITH
  (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB . 
\end{aligned}
\label{phf_strong_rindep}
\end{equation}


The main challenge in solving this evolution problem lies on imposing the irreversibility condition $d\geq d_n$, which allows to replace the set-valued expressions~\eqref{phf_weak} or~\eqref{phf_strong} by equalities. Several alternatives are available in the literature to tackle this problem, including simple penalization methods~\cite{gerasimov2019}, augmented Lagrangian penalization~\cite{wheeler2014}, the primal-dual active set method~\cite{heister2015}, interior point methods~\cite{wambacq2021}, and complementary system with Lagrange multipliers \cite{mang2020phase}. In this work, we employ the \textit{maximum crack-driving state function} method based on the \textit{history field}, as outlined in~\cite{MieWelHof10b,miehe+hofacker+schaenzel+aldakheel15,miehe2016aphase} and related works. % The point of departure is a modular structure generalized here as
%%
%\begin{equation}
%\begin{aligned}
%\frac{\eta_f}{\Delta t}(d-d_n)
%= 
%\widehat{g}_d (d,\alpha) \widetilde{D} - \big(d - l_f^2\div [ \nabla d ] - l_f^2 \beta_a \div [\nabla d \cdot\BM] \big) \geq 0
% \\ 
% \mbox{with} \qquad (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
%\quad \mbox{on} \quad \partial\calB , 
%\end{aligned}
%\label{euler-eq-d0}
%\end{equation}
%%
%where $\widetilde{D}$ is a \textit{crack driving state function} and $\widehat{g}_d$ is a function related to the derivative of the elastic/plastic degradation functions. To remove the inequality constraint from this expression and therefore account for the irreversibility condition, the maximum time history value of $\widetilde{D}$ is filtered out by means of the \textit{history field}
%%
%\begin{equation}
%\calH(\Bx,t):=\max_{s\in[0,t]}\widetilde{D}\big(\BfrakC(\Bx,s)\big) . 
%\end{equation}
%%
%Eq.~\eqref{euler-eq-d} is then rewritten as
%%
%\begin{equation}
%\begin{aligned}
%\frac{\eta_f}{\Delta t}(d-d_n)
%= 
%\widehat{g} (d,\alpha) \calH -  \big(d - l_f^2\div [ \nabla d ] - l_f^2 \beta_a \div [\nabla d \cdot\BM] \big)
% \\ 
% \mbox{with} \qquad (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
%\quad \mbox{on} \quad \partial\calB . 
%\end{aligned}
%\label{euler-eq-d}
%\end{equation}
%%
%We shall see that in the models considered in sections~\ref{sec:model1}--\ref{sec:model3}, it is possible to recover this formulation from the generic incremental evolution equation~\eqref{phf_strong}, where the functions $\widetilde{D}$ and $\widehat{g}$ will vary depending on the model.

%\subsubsection*{Plasticity}
%=======================================================================
\sectpc{Plasticity}
\label{plast_var}
%=======================================================================
The models considered in this study employ rate-independent von Mises plasticity. Consequently, only rate-independent plasticity will be considered hereinafter, such that $\eta_p=0$ in Eq.~\eqref{potential-functional-cont}. As will become clear, the plasticity problem does not follow from the incremental minimization problem~\eqref{inc_min} in all three models considered in this study. In particular, a variational formulation for the plasticity problem that is consistent with the governing equations is only possible if the elastic degradation function introduced in~\eqref{elas-part} does not depend on the hardening variable $\alpha$, that is, $g_{e}:=g_e(d)$, such that ${W}_{elas}:={W}_{elas}(\Bve,\Bve^p,d;\BM)$. Let us now summarize the variational formulation of such a model in the general gradient-extended case.

For a variational treatment, it is convenient to invoke the energetic-dissipative decomposition of the plastic energy~\eqref{plas-part_ener_diss}, such that a \textit{free energy density} can be defined~as 
%
\begin{equation}
{W}_{free}(\Bve,\Bve^p,d,\alpha;\BM):={W}_{elas}(\Bve,\Bve^p,d;\BM) + {W}_{plas}^{ener}(\alpha ,d,\nabla \alpha) .
\label{eq:Wfree} 
\end{equation}
%
The Coleman-Noll procedure yields the thermodynamic conjugate variables
%
\begin{equation}
\Bs^p := -\partial_{\Bve^p} {{W}_{free}}
= \Bsigma \AND h^p:=-\delta_\alpha{{W}_{free}}=-g_p(d)\,H\alpha + \sigma_Y \, l_p^2\div[g_p(d)\,\nabla\alpha] .
\label{dual}
\end{equation}
%
In agreement with the classical setting of elasto-plasticity, the yield function is defined as
%
\begin{equation}
\beta(\Bs^p,h^p;d):= \hbox{$\sqrt{3/2}$}\;\vert \BF^p \vert + h^p - g_p(d)\sigma_Y
\WITH
\BF^p:= \dev[\Bs^p] = \Bs^p - \frac{1}{3} \mbox{tr} [\Bs^p] \Bone .
\label{yield-fcn}
\end{equation}
%
With the yield function at hand, the strong form of the evolution problem follows from the principle of maximum plastic dissipation
%
\begin{equation}
\Phi^p(\dot\Bve^p,\dot\alpha;d) = \sup \{ \Bs^p:\dot{\Bve}^p + h^p\dot\alpha  \ \colon \ \beta(\Bs^p,h^p;d)\leq 0 \} ,
\label{pmd}
\end{equation}
%
where $\Phi^p$ is the \textit{plastic dissipation potential}. The Euler equations of the maximization principle~\eqref{pmd} follow as the flow rule and hardening law
%
\begin{equation}
\dot\Bve^p = \lambda^p \frac{\partial \beta}{\partial \Bs^p}  
\AND
\dot\alpha = \lambda^p\frac{\partial \beta}{\partial h^p} ,
\label{plast-evol-eqs}
\end{equation}
%
together with the KKT conditions conditions
%
\begin{equation}
\beta \le 0, \quad\quad  \quad\quad \lambda^p \ge 0 
\quad\quad \mbox{and} \quad\quad
\beta\; \lambda^p = 0 .
\label{palst-kkt}
\end{equation}
%
Equations~\eqref{plast-evol-eqs} and~\eqref{palst-kkt} constitute the so-called \textit{dual form} of the elasto-plastic problem in strong form. To arrive at a primal formulation~\citep{han1999,ulloa2020}, the dissipation potential is evaluated from~\eqref{pmd} as 
%
%\begin{equation}
%\Phi_p(\dot\Bve^p,\dot\alpha; d)=g(d)\widetilde{\Phi}(\dot\Bve^p,\dot\alpha) \WITH \widetilde{\Phi}(\dot\Bve^p,\dot\alpha):=\left\{
%\begin{array}{ll}
%\hbox{$\sqrt{2/3}$}\; \, \sigma_Y  \vert \dot\Bve^p \vert \quad &\text{if} \ \  \vert \dot\Bve^p \vert \leq \hbox{$\sqrt{3/2}$}\;\dot\alpha,  \\
%+\infty \quad &\text{otherwise}.
%\end{array}
%\right.
%\label{eq:pdiss}
%\end{equation}
\begin{equation}
\Phi_p(\dot\Bve^p; d)=g_p(d)\;\widetilde{\Phi}(\dot\Bve^p) \WITH \widetilde{\Phi}(\dot\Bve^p)=\sqrt{\frac{2}{3}}\, \sigma_Y  \vert \dot\Bve^p \vert  .
\label{eq:pdiss}
\end{equation}
%
The Legendre transformation of $\Phi_p$ then reads
%
\begin{equation}
\Phi_p^*(\Bs^p,h^p ; d )= \sup \{ \Bs^p:\dot{\Bve}^p + h^p\dot\alpha  - \Phi_p(\dot\Bve^p; d) \} ,
\label{eq:pdiss_trans}
\end{equation}
%
which yields, as a necessary condition, the primal representation of the plasticity evolution problem in the form of a Biot-type equation:
%
\begin{equation}
\{\Bs^p , h^p\}\in\partial_{\{\dot\Bve^p,\dot\alpha\}}\,\Phi_p(\dot\Bve^p;d) .
\label{eq:pbiot}
\end{equation}
%
From standard arguments of convex analysis~\cite{rockafellar1970,han1999}, this expression implies the associative flow relations~\eqref{plast-evol-eqs} as well as the loading/unloading conditions~\eqref{palst-kkt}.

To derive the governing equations above from the incremental minimization problem~\eqref{inc_min}, we make use of equations~\eqref{plas-part_ener_diss} and~\eqref{eq:pdiss}, such that the functional derivative of~\eqref{potential-functional-disc} with respect to $\{\Bve^p,\alpha\}$ can be written as 
%
\begin{equation}
\begin{aligned}
\calE_\alpha(\Bu,\Bve^p,\alpha,d;\delta \Bve^p, \delta \alpha)&=\int_\calB \bigg[\partial_{\Bve^p} W:\delta\Bve^p + \delta_\alpha W\delta\alpha \bigg]\,dv 
\\  &=   \int_\calB \bigg[\partial_{\Bve^p}\big(W_{elas} +  \Phi_p(\Bve^p-\Bve^p_n;d)\big):\delta\Bve^p   + \delta_\alpha{W}_{plas}^{ener}\delta\alpha\bigg]\,dv \ni 0  \\   & \hspace*{5.75cm} \forall \,\delta \Bve^p \in \mathbf{Q} ,  \ \delta \alpha \in \mathrm{W}_\alpha(\delta\Bve^p,0) .
\end{aligned}
\label{palst_weak}
\end{equation}
%
In view of equations~\eqref{eq:Wfree} and~\eqref{dual}, the strong form of~\eqref{palst_weak} can be written as
%
\begin{equation}
\{\Bs^p , h^p\}\in\partial_{\{\Bve^p,\alpha\}}\,\Phi_p(\Bve^p-\Bve^p_n;d) , \WITH
 \nabla \alpha \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB . 
\label{eq:pbiot_inc}
\end{equation}
%
Eq.~\eqref{eq:pbiot_inc} represents an incremental version of the compact evolution equation~\eqref{eq:pbiot} for the plasticity model, recovered in a variationally consistent manner from the incremental minimization principle~\eqref{inc_min}. Recall that in the present formulation, this was achieved by assuming an elastic degradation function that does not depend on the plastic variables.





\begin{table}[!]
	\caption{Functions and parameters for the three examined models.}
	\vspace{1mm}
	\centering
	\begin{tabular}{lccc}
		Model property                 & $(\calM_1)$ & $(\calM_2)$ & $(\calM_3)$ \\[2mm]\hline\\
		Elastic degradation  $g_e$          & $(1-d)^{2{\alpha}/{\alpha_c}}$   &  $(1-d)^2$  &  $(1-d)^2$  \\[4mm]
		Fracture constant $g_f$              & $G_c$   &    $2\,l_f c_f{\psi_c}$  & $l_f c_f{w_0}$   \\[4mm]
		Plastic degradation $g_p$           & $1$   &  $(1-d)^2$   &  $(1-d)^2$  \\[4mm]
		Local fracture energy $\omega$         & $d^2$   &  $d$  &  $d$  \\[4mm]
		Crack viscosity $\eta_f$               & $0$   &  $\geq0$  &  $0$  \\[4mm]
		Plastic length scale $\l_p$           & $0$   & $0$   & $\geq0$  \\[4mm]			Driving scaling factor $\zeta$           & $1$   & $\geq 0$   & $\geq 0$  	\\[4mm]    \hline
		\label{models}
	\end{tabular}
\end{table}

%=======================================================================
\sectpb{Specific models revisited}% : model based on~\citet{ambati2015}}
\label{sec:models}
%=======================================================================

In this section, three benchmark phase-field models  for ductile fracture, hereinafter labeled $(\calM_1)$, $(\calM_2)$ and $(\calM_3)$, are revisited within the framework elaborated in the previous subsections. The material parameters and constitutive functions that allow to recover each model from the general formulation are presented in Table~\ref{models}.

%=======================================================================
\sectpc{Local plasticity with $G_c$ based fracture criterion: Model 1 ($\mathcal{M}_1$)}% : model based on~\citet{ambati2015}}
\label{sec:model1}
%=======================================================================

The first model considered in this study takes~\cite{ambati2015} as a point of departure. Therein, an extension of the model proposed in~\cite{du2015} was considered, coupling the fracture process to plasticity by introducing dependence of the elastic degradation function on the hardening variable $\alpha$. The model was subsequently extended to finite strains and presented with experimental verification in~\cite{ambati2016}. As discussed in Sec.~\ref{plast_var}, dependence of the elastic degradation function on $\alpha$  results in lack of variational  consistency for the plasticity evolution problem, in favor of greater flexibility. Consider, in this case, the 
%
\begin{equation}
\mbox{Global Primary Fields}: \ 
\BfrakU := \{ \Bu, d \} , 
\label{primary_m1}
\end{equation}
%
and the
%
\begin{equation}
\mbox{Constitutive State Variables}: \ 
\BfrakC := \{ \Bve, \Bve^p, \alpha, d, \nabla d \}
.
\label{state_m1}
\end{equation}
%
With the constitutive choices shown in Table~\ref{models} for $(\calM_1)$, the following forms of the governing equations presented in Sec.~\ref{sec:eq_general} are obtained.


%The fracture yield function~\eqref{phf_weak} takes the form
%%
%\begin{equation}
%\begin{aligned}
%f_d=2\frac{\alpha}{\alpha_c}(1-d)^{2\frac{\alpha}{\alpha_c}-1}\big[\psi_e^{iso,+} + \psi_e^{aniso,+}\big] - \frac{G_c}{l_f} \big( {d} - l_f^2  \div [ \nabla d ] - l_f^2 \beta_a \div [\nabla d \cdot\BM] \big) ,
%\end{aligned}
%\label{phf_yield_m1}
%\end{equation}

The strong form of the crack phase-field evolution~\eqref{phf_strong} takes the form
%
\begin{equation}
\begin{aligned}
-2\frac{\alpha}{\alpha_c}(1-d)^{2\frac{\alpha}{\alpha_c}-1}\frac{l_f}{G_c}\big(\psi_e^{iso,+} + \psi_e^{aniso,+}\big) + \big( {d} - l_f^2  \div [ \nabla d ] - l_f^2 \beta_a \div [\nabla d \cdot\BM] \big) \\ + \frac{l_f}{G_c}\partial I_+(d-d_n) \ni 0  \\ 
 \mbox{with} \qquad (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB , 
\end{aligned}
\label{phf_strong_m1}
\end{equation}
%
where $\alpha_c$ is a threshold material parameter introduced in~\cite{ambati2015} to calibrate the softening branch. To enforce the irreversibility condition and, therefore, cast this expression as an equality, the history field 
%
\begin{equation}
\calH(\Bx,t):=\max_{s\in[0,t]}\widetilde{D}\big(\BfrakC(\Bx,s)\big) \WITH  \widetilde{D}:=\zeta\frac{2\,l_f}{G_c}\big(\psi_e^{iso,+} + \psi_e^{aniso,+}\big) 
\end{equation}
%
is introduced. Here, $\zeta\geq0$ is a scaling parameter that introduces further flexibility in the formulation, allowing to tune the post-critical range (cf.~\cite{aldakheel16}). Equation~\eqref{phf_strong_m1} is then restated as
%
\begin{equation}
\begin{aligned}
\frac{\alpha}{\alpha_c}(1-d)^{2\frac{\alpha}{\alpha_c}-1}\calH - \big( {d} - l_f^2  \div [ \nabla d ] - l_f^2 \beta_a \div [\nabla d \cdot\BM] \big) = 0  \\ 
 \mbox{with} \qquad (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB .
\end{aligned}
\label{phf_strong_m1_hist}
\end{equation}
% According to Table~\ref{models}, $\zeta=1$ is chosen for this model. 
With the last expression, and in view of Eq.~\eqref{equil_weak}, the global primary fields are found as the solution of the following coupled problem: find $\Bu\in\mathbf{V}(\overline{\Bu})$ and $d\in \mathrm{H}^1(\calB;[0,1])$ such that
%
\begin{align}
\tag{$\calM_1$}
\left\{
\begin{aligned}
&\int_\calB\big[\Bsigma(\Bve,\Bve^p,d,\alpha;\BM):\Bve(\delta\Bu)-\overline{\Bf}\cdot\delta\Bu\big]\,dv - \int_{\partial\calB_N}\overline{\Btau}\cdot\delta\Bu\,da =0 \quad  \forall \,\delta\Bu\in\mathbf{V}(\bm{0}) \  ,  \\
&\int_\calB \bigg[ \bigg(\frac{\alpha}{\alpha_c}(1-d)^{2\frac{\alpha}{\alpha_c}-1}\calH -  {d}\bigg)\delta d - l_f^2  \nabla d \cdot \nabla (\delta d) - l_f^2 \beta_a  \nabla d \cdot \BM \cdot \nabla (\delta d) \bigg]\,dv = 0    \\ 
&  && \hspace*{-2.75cm}\forall \,\delta d\in W_d(0)  . 
\end{aligned} 
\right.
\label{phf_weak_m1_hist}
\end{align}

\begin{Remark}
\label{variational_incons}
The introduction of the history field in the displacement Euler-Lagrange equation~\eqref{phf_strong_m1}, finally yielding~\eqref{phf_weak_m1_hist}$_1$, results in a loss of variational consistency with respect to the energy functional~\eqref{potential-functional-disc} due to (i) the filtering of the maximum history value of $\widetilde{D}$ and (ii) the scaling factor $\zeta$ for $\zeta\neq 1$. The upside of this choice is (i) a convenient numerical strategy for solving the original inequality-constrained PDE and (ii) greater flexibility in the model. 
\end{Remark}

\begin{Remark}
\label{zeta_M1}
The role of the parameter $\zeta$, i.e., tuning the post-critical range by scaling the driving force, is already achieved in the present model by means of $\alpha_c$ (see~\cite{miehe+hofacker+schaenzel+aldakheel15} for a similar approach). Consequently, $\zeta=1$ is assumed hereafter for $(\calM_1)$.
\end{Remark}

\begin{Remark}
	\label{Cdriv_m1}
	At this point, it is worth noting that the crack driving force in \eqref{phf_weak_m1_hist}$_2$, i.e., $\calH$, is scaled by the hardening variable $\alpha$, such that the crack driving force vanishes for $\alpha\rightarrow0$. As a consequence, fracture cannot occur outside the ductility zone, and a response corresponding to elastic damage followed by plastic damage is not possible in this model due to the strong coupling between damage and plasticity. For a detail discussion of different possible evolutions of elastic-plastic-damage, see \cite{alessi2017}.
\end{Remark}

%  $\texttt{E-D-PD}$ Instead, a response of the type $E-P-PD$ (one could compare this with $E-P-D$). 

Concerning the plasticity evolution problem, a variational derivation in the sense of Eq.~\eqref{palst_weak} is not possible in the present model due to the dependence of the elastic degradation function $g_p$ on $\alpha$. In this case, the \emph{local} evolution of the plasticity variables $\{\Bve^p,\alpha\}$ according to equations~\eqref{plast-evol-eqs} and~\eqref{palst-kkt} (alternatively, Eq.~\eqref{eq:pbiot} or Eq.~\eqref{eq:pbiot_inc}  in incremental form) is postulated in a non-variational context. For the present model, the yield function~\eqref{yield-fcn} takes the form
%
\begin{equation}
\beta= \hbox{$\sqrt{3/2}$}\;\vert \BF^p(\Bve,\Bve^p,d,\alpha;\BM) \vert - (\sigma_Y + H\alpha) .
\label{yield-fcn_m1}
\end{equation}

%=======================================================================
\sectpc{Local plasticity with $\psi_c$ based fracture criterion: Model 2 $(\calM_2)$} %: model based on~\citet{miehe+hofacker+schaenzel+aldakheel15}}
\label{sec:model2}
%=======================================================================

The second model is based on the geometrically conceived approach to the phase-field modeling of ductile fracture, outlined in~\cite{miehe+hofacker+schaenzel+aldakheel15} and widely considered in several works~\cite{aldakheel2019virtual,aldakheel16,aldakheel+wriggers+miehe18,miehe2016aphase,miehe2016bphase}. The original model is constructed within a variationally consistent framework, in agreement with the incremental energy minimization principle~\eqref{inc_min}. 

Consider, in this case, the 
%
\begin{equation}
\mbox{Global Primary Fields}: \ 
\BfrakU := \{ \Bu, d \}
\label{primary_m2}
\end{equation}
%
and the
%
\begin{equation}
\mbox{Constitutive State Variables}: \
\BfrakC := \{ \Bve, \Bve^p, \alpha, d, \nabla d \}
.
\label{state_m2}
\end{equation}
%
With the constitutive choices shown in Table~\ref{models} for $(\calM_2)$, the following forms of the governing equations described in Sec.~\ref{sec:eq_general} are obtained.


Letting $l_d:=\sqrt{2}\,l_f$ (cf.~\cite{marigo2016}), and after simple manipulations, the strong form of the crack phase-field evolution~\eqref{phf_strong} can be written as (cf.~\cite{miehe+hofacker+schaenzel+aldakheel15,aldakheel16}):
%
\begin{equation}
\begin{aligned}
-2(1-d)^2\psi_c\bigg(\frac{\psi_e^{iso,+} + \psi_e^{aniso,+}+ \psi_p}{\psi_c} - 1 \bigg) + 2\psi_c\big( d - l_d^2  \div [ \nabla d ] - l_d^2   \beta_a \div [\nabla d \cdot\BM] \big) \\ + \frac{\eta_f}{\Delta t} (d-d_n) + \partial I_+(d-d_n) \ni 0  \\ 
 \mbox{with} \qquad (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB , 
\end{aligned}
\label{phf_strong_m2}
\end{equation}
%
where the role of $\psi_c$ as a specific critical fracture energy density is clearly reflected. To enforce the irreversibility condition and, therefore, cast this expression as an equality, the history field 
%
\begin{equation}
\calH(\Bx,t):=\max_{s\in[0,t]}\widetilde{D}\big(\BfrakC(\Bx,s)\big) \WITH  \widetilde{D}:=\zeta\bigg(\frac{\psi_e^{iso,+} + \psi_e^{aniso,+}+ \psi_p}{\psi_c} - 1 \bigg)
\label{histfield_m2}
\end{equation}
%
is introduced. Letting $\eta_d:=\eta_f/(2\psi_c)$, Eq.~\eqref{phf_strong_m2} is restated as
%
\begin{equation}
\begin{aligned}
(1-d)\calH - \big( {d} - l_d^2  \div [ \nabla d ] - l_d^2 \beta_a \div [\nabla d \cdot\BM] \big) = \frac{\eta_d}{\Delta t}(d-d_n)  \\ 
 \mbox{with} \qquad (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB .
\end{aligned}
\label{phf_strong_m2_hist}
\end{equation}
% According to Table~\ref{models}, $\zeta=1$ is chosen for this model. 
%
With the last expression, and in view of Eq.~\eqref{equil_weak}, the global primary fields are found as the solution of the following coupled problem:  find $\Bu\in\Bu\in\mathbf{V}(\overline{\Bu})$ and $d\in \mathrm{H}^1(\calB;[0,1])$ such that
%
\begin{align}
\tag{$\calM_2$}
\left\{
\begin{aligned}
&\int_\calB\big[\Bsigma(\Bve,\Bve^p,d;\BM):\Bve(\delta\Bu)-\overline{\Bf}\cdot\delta\Bu\big]\,dv - \int_{\partial\calB_N}\overline{\Btau}\cdot\delta\Bu\,da =0 \quad  \forall \,\delta\Bu\in\mathbf{V}(\bm{0}) \  ,  \\
&\int_\calB \bigg[ \bigg((1-d)\calH -  {d} + \frac{\eta_d}{\Delta t}(d-d_n)\bigg)\delta d - l_d^2  \nabla d \cdot \nabla (\delta d) - l_d^2 \beta_a  \nabla d \cdot \BM \cdot \nabla (\delta d) \bigg]\,dv = 0    \\ 
&  && \hspace*{-2.75cm}\forall \,\delta d\in W_d(0)  . 
\end{aligned}
\right.
\label{phf_weak_m2_hist}
\end{align}
%
Note that, in light of Remark~\ref{variational_incons}, the introduction of the history field and the scaling parameter $\zeta$ in~\eqref{histfield_m2} results in a loss of variational consistency with respect to the energy functional~\eqref{potential-functional-disc} for the fracture problem.

As opposed to $(\calM_1)$, the local plasticity evolution problem in the present model is variationally consistent (see Sec.~\ref{plast_var}). The \emph{local} evolution of the plasticity variables $\{\Bve^p,\alpha\}$ according to the evolution equation~\eqref{eq:pbiot_inc}, which represents an incremental, \emph{primal} version of equations~\eqref{plast-evol-eqs} and~\eqref{palst-kkt}, is then a necessary condition of the minimization principle~\eqref{inc_min}. For the present model, the yield function~\eqref{yield-fcn} takes the form
%
\begin{equation}
\beta= \hbox{$\sqrt{3/2}$}\;\vert \BF^p(\Bve,\Bve^p,d;\BM) \vert - (1-d)^2(\sigma_Y + H\alpha) .
\label{yield-fcn_m2}
\end{equation}

%=======================================================================
\sectpc{Non-local plasticity with $w_0$ based fracture criterion: Model 3 ($\calM_3$)} %: model based on~\citet{rodriguez2018}}
\label{sec:model3}
%=======================================================================

The third model considered in this study takes~\cite{rodriguez2018} as a point of departure, where a variationally consistent phase-field model coupled to gradient plasticity was proposed. The modeling framework adopted therein is based on the energetic formulation advocated for ductile phase-field models in, e.g.,~\cite{alessi2015} and~\cite{ulloa2021}. This approach is consistent with the variational framework of~\cite{miehe2011} and the non-local treatment of plasticity adopted in other phase-field models~\citep{aldakheel16,miehe2016aphase,miehe2016bphase,miehe2017phase,dittmann2018}.  Consider, in this case, the 
%
\begin{equation}
\mbox{Global Primary Fields}: \  
\BfrakU := \{ \Bu, d ,\alpha \}
\label{primary_m3}
\end{equation}
%
and the
%
\begin{equation}
\mbox{Constitutive State Variables}: \  
\BfrakC := \{ \Bve, \Bve^p, \alpha, d ,\nabla\alpha, \nabla d \}
,
\label{state_m3}
\end{equation}
%
representing a combination of a  first-order gradient plasticity model and a first-order gradient damage model. With the constitutive choices shown in Table~\ref{models} for $(\calM_3)$, the following forms of the governing equations described in Sec.~\ref{sec:eq_general} are obtained.


With a slight change of parameters, the fracture problem in the present model admits the same formulation of $(\calM_2)$ in Sec.~\ref{sec:model2}. In this case, according to Table~\ref{models}, the strong form of the crack phase-field evolution~\eqref{phf_strong} can be written as:
%
\begin{equation}
\begin{aligned}
-(1-d)^2w_0\bigg(\frac{\psi_e^{iso,+} + \psi_e^{aniso,+}+ \psi_p}{w_0/2} - 1 \bigg) + w_0\big( d - l_d^2  \div [ \nabla d ] - l_d^2   \beta_a \div [\nabla d \cdot\BM] \big) \\  + \partial I_+(d-d_n) \ni 0  \\ 
 \mbox{with} \qquad (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB , 
\end{aligned}
\label{phf_strong_m3}
\end{equation}
%
where $w_0$ is a critical fracture energy density. The main difference of the present model with respect to $(\calM_1)$ and $(\calM_2)$ is that the plastic free energy $\psi_p$, defined in~\eqref{psi_p}, is considered here with $l_p>0$, and thus introduces non-local effects in the fracture driving force. To enforce the irreversibility condition, we define the history field 
%
\begin{equation}
\calH(\Bx,t):=\max_{s\in[0,t]}\widetilde{D}\big(\BfrakC(\Bx,s)\big) \WITH  \widetilde{D}:=\zeta\bigg(\frac{\psi_e^{iso,+} + \psi_e^{aniso,+}+ \psi_p}{w_0/2} - 1 \bigg) .
\label{histfield_m3}
\end{equation}
%
Eq.~\eqref{phf_strong_m3} is then restated as
%
\begin{equation}
\begin{aligned}
(1-d)\calH - \big( {d} - l_d^2  \div [ \nabla d ] - l_d^2 \beta_a \div [\nabla d \cdot\BM] \big) = 0  \\ 
 \mbox{with} \qquad (\BI+\beta_a\BM)\nabla d \cdot \Bn = 0
\quad \mbox{on} \quad \partial\calB .
\end{aligned}
\label{phf_strong_m3_hist}
\end{equation}
% 
As before, in light of Remark~\ref{variational_incons}, the introduction of the history field and the scaling parameter $\zeta$ in~\eqref{histfield_m2} results in a loss of variational consistency with respect to the energy functional~\eqref{potential-functional-disc} for the fracture problem.

As in $(\calM_2)$, the plasticity evolution problem for the present model is variationally consistent (see Sec.~\ref{plast_var}). Moreover, the problem now includes non-local effects modulated by the plastic length scale $l_p>0$, where the yield function~\eqref{yield-fcn} reads
%
\begin{equation}
\beta= \hbox{$\sqrt{3/2}$}\;\vert \BF^p(\Bve,\Bve^p,d;\BM) \vert - (1-d)^2(\sigma_Y + H\alpha) + \sigma_Y \,l_p^2 \div[ (1-d)^2\nabla\alpha  ] .
\label{yield-fcn_m3}
\end{equation}
%
To derive the global PDE governing the evolution of the non-local field $\alpha$, we  take the weak form~\eqref{palst_weak} as a point of departure, such that, for $\vert\Bve^p-\Bve^p_n\vert>0$:
%
\begin{equation}
\begin{aligned}
\int_\calB \bigg[\partial_{\Bve^p}\big(W_{elas} &+  \Phi_p(\Bve^p-\Bve^p_n;d)\big):\delta\Bve^p   + \delta_\alpha{W}_{plas}^{ener}\delta\alpha\bigg]\,dv \\ &=  \int_\calB \bigg[-\Bsigma(\Bve,\Bve^p,d;\BM):\delta\Bve^p  +  (1-d)^2\sigma_Y\hat\Bn:\delta\Bve^p   \\ & \hspace*{2cm}+(1-d^2)\,H\alpha\delta\alpha - \sigma_Y \, l_p^2\div[(1-d)^2\,\nabla\alpha]\delta\alpha\bigg]\,dv \\ &=  \int_\calB \bigg[-\sqrt\frac{3}{2}\vert\BF^p(\Bve,\Bve^p,d;\BM)\vert  +  (1-d)^2\sigma_Y   \\ & \hspace*{2cm}+(1-d^2)\,H\alpha - \sigma_Y \, l_p^2\div[(1-d)^2\,\nabla\alpha]\bigg]\delta\alpha\,dv = 0  ,
\end{aligned}
\label{palst_weak_m3_1}
\end{equation}
%
where $\hat\Bn:=(\Bve^p-\Bve^p_n)/\vert \Bve^p-\Bve^p_n \vert$ is the direction of the plastic flow. Note that in~\eqref{palst_weak_m3_1}, we have considered virtual fields 
%
\begin{equation}
\delta\Bve^p=\hat\Bn\vert\delta\Bve^p\vert=\sqrt{\frac{3}{2}}\hat\Bn\delta\alpha ,
\end{equation}
%
such that the direction of the plastic flow is fixed, while the virtual equivalent plastic strain $\delta\alpha\in\mathrm{W}_\alpha(\delta\Bve^p,0)$ is allowed to vary. To solve Eq.~\eqref{palst_weak_m3_1}, we must enforce the constraint embedded in $\alpha\in\mathrm{W}_\alpha(\Bve^p-\Bve^p_n,\alpha_n)$ (Eq.~\eqref{Walpha}), such that
%
\begin{equation}\label{plastic_law}
\alpha=\alpha_n+\sqrt{\frac{3}{2}}\vert\Bve^p-\Bve^p_n\vert .
\end{equation}
%
Recalling that~\eqref{palst_weak_m3_1} is a weak representation of~\eqref{eq:pbiot_inc} for $\vert\Bve^p-\Bve^p_n\vert>0$, and that~\eqref{eq:pbiot_inc}  implies the incremental version of the plastic flow rule~\eqref{plast-evol-eqs}, a possible way to proceed is to replace the local field $\Bve^p$ by setting, in agreement with~\eqref{plast-evol-eqs}, 
%
\begin{equation}
\Bve^p=\Bve^p_n+\sqrt{\frac{3}{2}}(\alpha-\alpha_n)\hat\Bn^{trial} \WITH \hat\Bn^{trial}=\frac{\BF^{p,trial}}{\vert \BF^{p,trial} \vert} 
\label{eq:ep_inc}
\end{equation}
%
where, from standard arguments of von Mises plasticity, $\BF^{p,trial}:=\BF^{p}(\Bve,\Bve^p_n,d;\BM)$. With this expression at hand, Eq.~\eqref{palst_weak_m3_1} may be left as a function of the non-local field $\alpha$, subject to the irreversibility condition $\alpha\geq\alpha_n$. 

Finally, the global primary fields are found as the solution of the following coupled problem:  find $\Bu\in\Bu\in\mathbf{V}(\overline{\Bu})$, $d\in \mathrm{H}^1(\calB;[0,1])$, and $\alpha\in \mathrm{H}^1(\calB;\calR_+)$ such that
%
\begin{align}
\tag{$\calM_3$}
\left\{
\begin{aligned}
&\int_\calB\big[\Bsigma(\Bve,\Bve^p,d;\BM):\Bve(\delta\Bu)-\overline{\Bf}\cdot\delta\Bu\big]\,dv - \int_{\partial\calB_N}\overline{\Btau}\cdot\delta\Bu\,da =0 \quad  \forall \,\delta\Bu\in\mathbf{V}(\bm{0}) \  ,  \\
&\int_\calB \bigg[ \big(\,(1-d)\calH -  {d}\, \big)\delta d - l_d^2  \nabla d \cdot \nabla (\delta d) - l_d^2 \beta_a  \nabla d \cdot \BM \cdot \nabla (\delta d) \bigg]\,dv = 0   \quad  \,\delta d\in W_d(0)
, \\
&\int_\calB \bigg[-\sqrt\frac{3}{2}\vert\BF^p(\Bve,\Bve^p,d;\BM)\vert  +  (1-d)^2\sigma_Y  + \partial I_+(\alpha-\alpha_n)   \\ & \hspace*{2cm}+(1-d^2)\,H\alpha + \sigma_Y \, l_p^2(1-d)^2\nabla\alpha\cdot\nabla(\delta\alpha)\bigg]\delta\alpha\,dv \ni 0  \quad \forall \,\delta \alpha\in \mathrm{H}^1(\calB;\calR_+).
\end{aligned}
\right.
\label{phf_weak_m3_hist}
\end{align}

Note that in~\eqref{phf_weak_m3_hist}$_3$, the indication function has been introduced to impose irreversibility of $\alpha$, resulting in a multivalued expression. To show the consistency of this equation with the governing equations derived in Sec.~\ref{plast_var}, we first recall that the incremental flow rule has been enforced by means of Eq.~\eqref{eq:ep_inc}. Then, we note that the strong form of Eq.~\eqref{phf_weak_m3_hist}$_3$ yields $\beta \in \partial I_+(\alpha-\alpha_n)$, with $\beta$ given in Eq.~\eqref{yield-fcn_m3}. In view of Eq.~\eqref{subdiff_ind}, it is easy to see that this expression represents the incremental version of the KKT conditions~\eqref{palst-kkt}. To handle the inequality constraint and eliminate the multivalued term $\partial I_+(\alpha-\alpha_n)$, a constrained optimization technique is required. For instance, an interior-point method has been recently proposed in~\cite{wambacq2021}.

In the sequel, the phase-field models for ductile fracture formulated in $(\calM_1)$, $(\calM_2)$, and $(\calM_3)$ will be taken as inputs for the Bayesian inversion framework described in a detail in Sec. 4.

\ju[inline]{I'm not sure that the labels  $(\calM_1)$, $(\calM_2)$, and $(\calM_3)$ are OK to refer to both the models and the global systems of PDEs. The models also include the local plasticity equations for  Mode 2 and Model 2. We should settle on the terminology.}

==> sec3.tex <==
%=======================================================================
\sectpa[Section3]{Parameter estimation based on Bayesian inference }
\label{Bayesian}
%=======================================================================

 
In this section, we review different parameter estimation techniques based on MCMC to identify the mechanical parameters involved in ductile fracture. First, some basic statistical principals are briefly recalled. 


In a Bayesian estimation, a parametric forward model (e.g., a PDE-based model) is used to update the available data (considered as random variables) based on the available information (denoting the prior knowledge). The posterior information is then provided as output \cite{rappel2020tutorial,smith2013uncertainty,wang2020uncertainty}. %, which leads to an accurate model response with respect to measurements.   

%{\color{red}Bayesian inference is based on the supposition that probabilities, and more generally our state of knowledge regarding an observed phenomenon, can be updated as additional information is obtained. In the context of parametric models, parameters are treated as random variables having associated densities.}

Bayes' formula prescribes the probability of an event according to related prior information and is given by
\begin{align}
P(A|B)=\frac{P(B|A)P(A)}{P(B)},
\label{Bay}
\end{align} 
where $P(A|B)$ denotes the conditional probability of event $A$ happening when $B$ has happened (similarly for $P(A|B)$), and $P(\cdot)$ is the probability of observations $A$ and $B$. Using a probability density function (pdf) $\pi$, we can rewrite \eqref{Bay} as
\begin{align}
\pi(\chi|v)=\frac{\pi(m|\chi) \pi_0(\chi)}{\pi(m)}.
\end{align}
Here, $\pi_0(\chi)$ is the prior distribution which indicates the available information regarding the parameter. Also, $\pi(\chi|m)$ denotes the posterior density, i.e., the probability density of the parameter $\chi$ considering the measurement $m$.  The probability of the parameter $\chi$ with respect to the observation/measurement is described by the likelihood $\pi(m|\chi)$. The denominator $\pi(m)$ is a constant normalization factor, such that
\begin{align}
\pi(\chi|m)\propto\pi(m|\chi)\pi_0(\chi).
\end{align}
In Bayesian inversion,  the solution of the inverse problem is the posterior density giving the distribution of the unknown parameter values based on the sampled observations.
MCMC is a popular method to calculate this distribution, where a Markov chain is constructed whose stationary distribution is the sought posterior distribution in Bayes' theorem.

In order to identify the unknown parameters, we introduce the following statistical model: 
\begin{align}
\label{81}
\mathbb{M}=f(\xx,\chi)+\varepsilon,
\end{align}
where $\mathbb{M}$ is a $n$-dimensional vector that indicates the measurement, $f$ denotes the PDE-based model, and $\chi=\{\chi_{_1},\chi_{_2}\ldots,\chi_{_k}\}$ is a $k$-dimensional vector denoting the model parameters. The model output $f(\chi)$ belongs to $\mathbb{R}^n$ in the ductile fracture model points out the load-displacement during $n$ time-steps (until the material fracture). For  the measurement error $\varepsilon$, we employ a Gaussian independent and identically distributed (iid) error $\varepsilon\sim\mathcal{N}(0,\sigma^2\,I)$ where $\sigma^2$ is a fidelity parameter.

%\ju[inline]{In the previous section, $\calR$ is the set of real numbers. We should settle on notation.}

Given a measurement or observation $m=\mathtt{obs}$, the conditional density reads
\begin{align}
\pi(\mathtt{obs})= \int_{\R^n}\pi(\mathtt{obs}|\chi)\pi_0(\chi)\,d\chi\neq 0.
\end{align}
The inverse problem in the Bayesian framework can thus be stated as follows:
given a measurement $m$, find the posterior density $\pi(\chi|m)$. To this end, one makes use of \textit{Bayes'~theorem~of~inverse~problems}, which can be stated as follows.
\begin{theorem}[\textit{Bayes'~theorem~for~parameter~estimation}]
	We consider random parameter variables $\chi$ and a specific prior distribution $\pi_0(\chi)$,  and we consider $m$ to be a realization of the random observation variable (denoting the measurement or virtual observation). The posterior distribution considering the measurement $m$ follows as
	\begin{align}\label{82}
	\pi(\chi|m)=\frac{\pi(m|\chi) \pi_0(m)}{\pi(m)}=\frac{\pi(m|\chi) \pi_0(\chi)}{\int_{\R^n}\pi(m|\chi)\pi_0(m)}.
	\end{align}
\end{theorem}
When using the above relation, one implicitly assumes that observed data is used to construct the posterior density. We should note that in our problem of interest, in case that an experimental measurement is not available, alternatively, a virtual observation $\mathtt{obs}$ using a significantly fine mesh can be used. Obviously, the observation will be more precise when a real experiment exists.

If we employ the statistical model \eqref{81} with the assumption that errors are Gaussian independent and identically distributed and $\varepsilon_i\sim N(0,\sigma^2)$, where $\sigma^2$ is fixed, then the likelihood function is
\begin{align}\label{83}
\pi(m|\chi)=L(\chi,\sigma^2|m)=\frac{1}{(2\pi\sigma^2)^{n/2}}\exp\left(-\sm/2\sigma^2\right)
\end{align} 
where
\begin{align}\label{84}
\sm=\sum_{j=1}^{n}[m_j-f_j(\xx,\chi)]^2
\end{align}
is the sum of square errors.

Considering the given likelihood function (\ref{83}), the posterior distribution has the following form
\begin{align}
\pi(\chi|m)=\frac{\exp\left(-\sm/2\sigma^2_0\right)}{\int_{0}^{\infty} \exp\left(-\sx/2\sigma^2_0\right)d\xi}\,=\frac{1}{\int_{0}^{\infty}\exp\left(-(\sx-\sm)\right)/2\sigma^2_0d\xi},
\end{align}
where $\sx$ is the sum of squares defined by the integration variable (see \eqref{83}). As a numerical point of view, we can approximate the integral as 
\begin{align}
\pi(\chi|m)\approx\frac{1}{\sum_{i=1}^{n} \exp\left(-(\sx-\sm)\right)/2\sigma^2_0w^i}
\end{align}
where the quadrature points and weights are denoted, respectively, by $\xi^i~\text{and}~w^i$.


In statistics, MCMC methods comprise a class of algorithms for sampling from a probability distribution. By constructing a Markov chain with the desired distribution as its equilibrium distribution, one can obtain a sample of the desired distribution by observing the chain after a number of steps. The more steps there are, the more closely the distribution of the sample matches the actual desired distribution. 

In Bayesian statistics, the recent development of MCMC methods has been a key step in making it possible to compute large hierarchical models that require integration over hundreds or even thousands of unknown parameters. 
In rare event sampling, they are also used for generating samples that gradually populate the rare failure region. 

Below, different popular MCMC methods are reviewed. These methods will be used to identify the parameters in ductile fracture in Sec. 4. A fair comparison between the performance of the methods will be given to clarify their efficiency.  
 

\sectpb[MH]{Metropolis and Metropolis-Hasting Algorithms}\label{MH1}
The Metropolis-Hastings (MH) algorithm   is one of the most common techniques among the MCMC methods due to its simplicity and its ability to handle many problems (specifically when the parameters are not strongly correlated). In order to estimate the posterior distribution, in each iteration, a new candidate  parameter value is proposed based on the current sample value according to a proposal distribution. Then, the acceptance ratio is calculated to decide whether the candidate value is accepted or rejected. The acceptance ratio points out how probable the new candidate value is with respect to the current sample. 

The method was first introduced by Metropolis \cite{metropolis1953equation} based on a random walk. The algorithm starts from the initial guess (the prior value) $\chi^0$. Afterwards, according to the chosen proposal distribution a new candidate $\cn$ is proposed, which possibly depends on the previous candidates. Having the new candidate $\cs$, the acceptance rate is calculated as 
\begin{align}
\lambda(\cn,\cs)=\min\left(1,\frac{\pi(\cs)}{\pi(\cn)}\right).
\end{align} 
As the next step, a random variable $\mathcal{R}\sim \text{Uniform}\,(0,1)$ is produced. If $\mathcal{R}<\lambda$ the candidate is accepted; otherwise, we reject the new proposal and keep the previous candidate in the chain. We follow this procedure for a sufficiently high number of replications. As seen, the algorithm is simple and efficient, specifically when a suitable proposal density is chosen and a large sampling is used. However, an inappropriate proposal results in a significant decrease in performance. If the proposal is very large, many of the candidates will be rejected; therefore, a good convergence to the target density (posterior distribution) will not be achieved. In contrast, if the proposal is too narrow, although many of the candidates are accepted, the chain movement is very slow, and many of the targets will not be captured.  

In the Metropolis algorithm, a symmetric proposal density (i.e., $\phi(\cs|\cn)=\phi(\cn|\cs)$) is assumed. According to this condition, a movement towards the proposed candidate from the current point is equal to a backward movement (from the current candidate to the proposed point). The use of a non-symmetric proposal distribution was proposed as an efficient improvement by Hastings \cite{hastings1970monte}. The algorithm is summarized in Algorithm 1.


\begin{algorithm}[ht!]
	\label{algorithm}
	\vspace{0.2cm}
	\textbf{Initialization ($j=0$)}: Generate the initial parameter $\chi^0\sim\pi(\chi^0|\,m)$.\\  

	\textbf{while}~{$j<N$}{\\
		
		
	
		
		\quad 1. Propose the new candidate $\chi^{*}\sim\phi(\chi^j|\,\chi^{j-1})$ ($\phi$ is the proposal distribution).    \\
		% (i.e., the proposal distribution)\\
		
		
		\quad 2. Compute the proposal correction parameter~$\beta(\chi^*|\,\chi^{j-1})=\cfrac{\phi(\chi^{j-1}|\,\chi^*)}{\phi(\chi^*|\,\chi^{\ell-1}))}$.
		%    =
		%   =
		%    \cfrac{\Pi(\beta|\,\alpha^*) \Pi_0(\alpha^*)}{\Pi(\beta|\alpha^{\ell-1})\Pi_0(\alpha^{\alpha-1})}$
		\\
		
		
		\quad  3. Calculate the acceptance/rejection probability $\lambda (\chi^*|\,\chi^{j-1})=\min\left(1, \cfrac{\pi(\chi^*|\,m)}{\pi(\chi^{j-1}|\,m)}\,\beta\right)$.\\
		
		\quad 4. Draw a random number $\mathcal{R}\sim \text{Uniform}\,(0,1)$.\\
		
		\quad 5.$~\textbf{if}~$ $\mathcal{R}<\lambda~$ \textbf{then}\\ 
		
		\qquad\quad accept the candidate $\chi^*$ and set $\chi^j=\chi^*$\\
		
		\qquad \textbf{else}\\
		
		\qquad\quad reject the candidate $\chi^*$ and set $\chi^{j}=\chi^{j-1}$\\
		
		\qquad \textbf{end if}\\
		
	\quad 6. Set $j=j+1$.\\		
		
	}
	\caption{The MH algorithm.}
\end{algorithm}

We can draw the following conclusions: 

\begin{itemize}
	\item A proposal $\cs$ that results in $\pi(m|\cs)>\pi(m|\cn)$ entails a small sum of squared error and thus leads to candidate acceptance.
	\item A proposal $\cs$ that leads to $\pi(m|\cs)<\pi(m|\cn)$  entails a higher 
	sum of squared error and the proposal may be rejected.
\end{itemize}

Regarding the proposal functions and how they affect the posterior distribution, if the variance is too large, a large percentage of the candidates will be rejected, since they will have smaller likelihoods, and hence the chain will stagnate for long periods. The acceptance ratio will be high if the variance is small, but the algorithm will be slow to explore the parameter space.   

There are different measures to determine if the Markov chain is efficiently sampling from the posteriori density. A good criterion is the acceptance rate (the percentage of accepted candidates). The ratio can be used to tune the proposal density, i.e., reduce its variance. Another efficiency test is the autocorrelation function.  The lag-$\tau$ autocorrelation function  $ACF\colon\mathbb{N}\rightarrow [-1,1]$ is estimated by
\begin{equation*}
ACF(\tau)=\frac{\sum_{j=1}^{N-\chi} (\chi_j -\bar{\chi})(\chi_{j+\tau} -\bar{\chi}) }{ \sum_{j=1}^{N}\left( \chi_j-\bar{\chi}\right)^2}=\frac{\text{cov}(\chi_j,\chi_{j+\tau})}{\text{var}(\chi_j)}.
\end{equation*}
Here, $\chi_j$ denotes the $j$-th element of the Markov chain and
$\bar{\chi}$ is the mean value. Note that $ACF(\tau)$ is positive and monotonically decreasing. The interested readers can refer to \cite{khodadadian2020bayesian}, where the authors studied the effect of $ACF$ on different parameters in phase-field modeling of brittle fracture. A more advanced convergence analysis such as $\hat{R}$-statistics can be implemented when multiple MCMCs with different initial values are used. In Sec. \ref{Section5}, we will use such a diagnostic tool to compare the performance of the Bayesian techniques. 


\sectpb[DRAM]{Delayed Rejection Adaptive Metropolis (DRAM)}\label{DRAM}


At this point, it is worth discussing some improvements in the MH algorithm based on the proposal distribution. The main disadvantage of the model is that the covariance of the proposal should be tuned manually. To improve the efficiency, an alternative to using a fixed proposal distribution in each iteration is to update the distribution according to the available samples (adaptive Metropolis). This approach is useful since the posterior distribution is not sensitive to the proposal distribution. 


To adapt the proposal function according to the obtained information, Haario \cite{haario2001adaptive} proposed a technique where the current point is chosen as the proposal center and the covariance function is updated using the estimated data. To this end, one can use the following proposal estimation
\begin{align}
V_j=S_p\text{Cov}\left(\chi^0,\chi^1\ldots,\chi^{j-1}\right)+\epsilon I_j,
\end{align}
where the parameter $\epsilon$ is chosen very small (close to zero) and $S_p=\frac{2.38^2}{j}$ (as the scaling parameter). The covariance function is calculated by
\begin{align}
\mathcal{COV}_j=\text{Cov}(\chi^0,\chi^1,\ldots,\chi^{j})=\frac{1}{j}\left(\sum_{i=0}^{j}
\chi^i\left(\chi^i\right)^T-(n+1)~\hat{\chi}^j\left(\hat{\chi}^j\right)^T\right),
\label{cov1}
\end{align}   
where $\hat{\chi}^j=\frac{1}{j+1}\sum_{i=0}^{j}\chi^j$ \cite{smith2013uncertainty}. The proposal adaptation can be done after a specific number of steps (e.g., 1000) instead of all steps.

The efficiency of the algorithm can be further enhanced by adding a delayed rejection step. Mira \cite{green2001delayed} proposed that instead of a rejected candidate, a second stage is used to propose it from another proposal density. As the first step we propose the new candidate using the Cholesky
decomposition of the covariance function \eqref{cov1}:
$$\chi^{*}=\chi^{j-1}+\mathcal{COV}_j\mathcal{U},$$ 
where
$\mathcal{U}\sim \text{Uniform}~(0,I_j)$ and $I_j$ is the $j$-dimensional identity matrix.
The alternative proposal $\chi^{**}$ is chosen using the proposal function
\begin{align}
\phi(\chi^{**}|\chi^{j-1},\chi^*)=\mathcal{N}(\chi^{j-1},\gamma_2^2 V_j),
\end{align}
where $V_j$ is the covariance matrix estimated by the adaptive algorithm \cite{green2001delayed}. The essential parameter is $\gamma_2$, which will be chosen less than one so that the next stage has a narrower proposal function (normally, $\gamma_2=1/5$ is chosen). We use the following acceptance ratio
\begin{align}\label{821}\nonumber
\lambda_2(\chi^{**}|\chi^{j-1},\chi^*)&:=\min\left(1,\frac{\pi(\chi^{**}|m) \phi(\chi^*|\chi^{**} ) \phi_2(\chi^{j-1}|\chi^{**},\chi^*) [1-\lambda(\chi^*|\chi^{**})]}{\pi(\chi^{j-1}|m) \phi(\chi^*|\chi^{j-1} ) \phi_2(\chi^{**}|\chi^{j-1},\chi^*) [1-\lambda(\chi^*|\chi^{j-1})]}\right)\\
&=\min\left(1,\frac{\pi(\chi^{**}|m) \phi(\chi^*|\chi^{**} )  [1-\lambda(\chi^*|\chi^{**})]}{\pi(\chi^{j-1}|m) \phi(\chi^*|\chi^{j-1} )  [1-\lambda(\chi^*|\chi^{j-1})]}\right).
\end{align}
Then, similar to the MH algorithm we follow the Markov chain to accept/reject the candidate. A summary of the process is given in Algorithm 2.



\begin{algorithm}[ht!]
	\vspace{0.2cm}
	\label{algorithm1}
	\textbf{Initialization ($j=0$)}: Generate the initial parameter $\chi^0\sim\pi(\chi^0|\,m)$.\\  
	
	
	
	
	\textbf{while~}{$j<N$}{
		\vspace{0.3cm}
		

		
		\quad 1. Propose a new candidate $\chi^{*}=\chi^{j-1}+\mathcal{R}_j\mathcal{Z}_j$  where $\mathcal{R}_j$ is the Cholesky decomposition \\
		
		\vspace{-0.3cm} ~~~~~~~of $\mathcal{V}_j$ and $\mathcal{Z}_j\sim$ Uniform (0, $I_j$) where $I_j$ denotes the identity matrix. \\
		% (i.e., the proposal distribution)\\
		
		
		
		
		
		\quad  2. Calculate the acceptance/rejection probability $$\lambda_1 (\chi^*|\,\chi^{j-1})=\min\left(1, \cfrac{\pi(\chi^*|\,m)~\phi(\chi^{j-1}|~\chi^*)}{\pi(\chi^{j-1}|\,m)~\phi(\chi^*|\,\chi^{j-1}))}\right)$$.
		
		\quad 3. Draw a random number $\mathcal{R}\sim \text{Uniform}\,(0,1)$.\\
		
		\quad 4.$~\textbf{if}~$ $\mathcal{R}<\lambda_1~$ \textbf{then}\\ 
		
		\qquad\quad accept the candidate $\chi^*$ and set $\chi^j=\chi^*$\\
		
		\qquad \textbf{else}\\
		
		\qquad\quad(i)  Calculate the alternative candidate
		\quad$\chi^{**}=\chi^{j-1}+\sigma^2\mathcal{R}_j\mathcal{Z}_j$.\\
		
		\qquad\quad (ii)   Calculate the acceptance/rejection probability\\ $$\qquad\qquad\lambda_2 (\chi^{**}|\,\chi^{j-1},\chi^*)=\min\left(1, \cfrac{\pi(\chi^{**}|\,m)~\phi(\chi^*|~\chi^{**})\left(1-\lambda_1(\chi^*|\chi^{**})\right)}{\pi(\chi^{j-1}|\,m)~\phi(\chi^*|~\chi^{j-1})\left(1-\lambda_1(\chi^*|\chi^{j-1})\right)}\right)$$.\\
		
		\vspace{-0.3cm}\qquad\quad (iii)  \textbf{if} ~$\mathcal{R}<\lambda_2$~~\textbf{then}\\
		
		\qquad\qquad\quad~~accept the candidate $\chi^{**}$ and set $\chi^{j}=\chi^{**}$\\
		
		\qquad\quad~~~   \textbf{else}\\
		
		\qquad\qquad\quad~~  reject the candidate $\chi^{**}$ and set $\chi^{j}=\chi^{j-1}$
		\qquad\quad\\
		
		\qquad \textbf{end if}\\
		
		\quad 5. Update the covariance matrix as $\mathcal{V}_j=\text{Cov}(\chi^0,\chi^1,\ldots,\chi^{j})$.\\
		
		\quad 6. Update $\mathcal{R}_j$.\\
		
		
				\quad 7. Set $j=j+1$.\\
	}
	\caption{The DRAM algorithm.}
\end{algorithm}


\sectpb[kalman]{MCMC with ensemble-Kalman filter}\label{kalman}
%Kalman-inspired proposal
As previously mentioned, a good detection of the proposal density will enhance the Markov chain movement to the target density. Here, we introduce another proposal distribution detection technique using  a {\color{black}ensemble-Kalman filter}. The idea is based on using the Kalman filter \cite{kalman1960new} and we obtain
\begin{align}
	\cs=\cn+\Delta \chi,
	\label{prop1}
\end{align}
where $\Delta \chi$ denotes the jump of Kalman-inspired proposal. In order to update the proposal, we can separate \eqref{prop1} into
\begin{align}
\Delta \chi=\mathcal{K}\left( y^{j-1}+s^{j-1}\right).
	\label{prop2}
\end{align} 
The first term indicates the so-called Kalman gain, i.e., 
\begin{align}
\mathcal{K}=\C_{\chi M}\left(\C_{MM}+\mathcal{R}\right)^{-1},
\end{align}
where $\C_{\chi M}$ is the covariance matrix between the inferred parameters and the PDE-based model, $\C_{MM}$ is the covariance matrix of the PDE response, and $\mathcal{R}$ denotes the measurement noise covariance matrix \cite{zhang2020improving}. In \eqref{prop2}, $y^{j-1}$ is the residual of candidates with respect to the model. In other words, considering $\bar{m}$ an observation/measurement, $y^{j-1}=\bar{m}-f(\chi^{j-1})$ and  $s^{j-1}\sim\N(0,\mathcal{R})$, related to the density of measurement. A summary of the procedure is given in Algorithm 3.

\begin{algorithm}[ht!]
	\vspace{0.2cm}
	\textbf{Initialization ($j=0$)}:  initiate the samples according to the prior density $\chi^0$\\[2mm]
	\textbf{while}~$j<N$ 	\\[3mm]
	\vspace{0.1cm}
	\quad 1. $\bullet$~set \var{FLAG}=true \qquad $\bullet$~set $ n=0$\\[3mm]
	\vspace{0.1cm}
	\textbf{While}~\var{FLAG}~\textbf{do}\\[3mm]
	\vspace{0.1cm}
	\qquad\quad(i) Solve the model equations $\mathcal{M}_1$, $\mathcal{M}_2$, and $\mathcal{M}_3$ considering   $\texttt{TOL}_\mathrm{Stag}$ and\\[3mm]
			\vspace{0.1cm}
	\hspace{1.7cm}  the proposed candidate $\cn$ an then obtain $f(\cn)$\\[3mm]
		\vspace{0.1cm}
		\qquad\quad(ii) update the Kalman gain			
	\begin{align}
\mathcal{K}=\C_{\chi M} \left(\C_{MM}+\mathcal{R}\right)^{-1}
	\end{align} 
	\vspace{0.1cm}
	\qquad \qquad \quad$\bullet$ $\mathcal{R}$ is the measurement noise covariance matrix\\[3mm]
		\vspace{0.1cm}
	\qquad \quad \hspace{-0.0cm}(iii) shift the ensemble 
\begin{align}
	\cs=\cn+\K\left( y^{j-1}+s^{j-1}\right) 
\end{align}
	\qquad \qquad ~$\bullet$ $y^{j-1}\sim\N(\varepsilon^{j-1},\mathcal{R})$ is the residual of the proposed parameters\\[3mm]
	\vspace{0.1cm}
	\qquad \qquad \,\,$\bullet$ $s^{j-1}\sim\N(0,\mathcal{R})$ relates to the measurment error\\[3mm]
		\vspace{0.1cm}
	\qquad \quad \hspace{0.0cm}(iv) \textbf{if} the full fracture is happened \textbf{then}\\[3mm]
		\vspace{0.1cm}
	\qquad \qquad \qquad ~~~~$\bullet$ set \var{FLAG}=false\\[3mm]
	\qquad \qquad~	
	\vspace{0.1cm}
	\qquad \quad \hspace{0.7cm} \textbf{else} \\[3mm]
	\vspace{0.1cm}
	\qquad \qquad \qquad ~~~ $\bullet$ set~ $n=n+1$\\[3mm]
	\qquad \qquad~	
			\vspace{0.1cm}
\qquad \quad \hspace{0.7cm} 	\textbf{end if}\\[3mm]			
	\quad 2. Accepted/rejected the material approximation.\\[3mm]
	\quad 3. Set $j=j+1$.\\
	\caption{Bayesian inversion with ensemble-Kalman filter.} 
	\label{algorithm3}	
\end{algorithm}


\sectpb[bayesian]{Bayesian inversion for ductile phase-field fracture}
\label{bayesian}
Knowledge about the mechanical parameters that influence the behavior of fracturing solids is crucial to develop models able to precisely predict crack initiation and propagation during different stages of the deformation process. Bayesian inversion techniques are convenient tools to monitor the crack behavior using observations (e.g., the measured data) and solving the inverse problem considering the PDE-based model. Below, we review different possibilities for the implementation of Bayesian inversion in the context of elastic-plastic fracturing solids governed by phase-field models.
\begin{itemize}
	\item \textbf{Based on the load-displacement curve}: this approach allows to observe the crack behavior from the stable position to the failure point (all time steps). At time-step $n$, the load-displacement curve can be computed using the stress tensor as
	\begin{align}
	F_n=\int_{\partial_D\mathcal{B}} \boldsymbol{n}\cdot\boldsymbol{\sigma}\cdot \boldsymbol{n}\,da.
	\end{align}
 The main advantage of working with this curve is its easiness, since we are working with a one-dimensional parameter. However, it is sensitive to the mesh size and the length scale; therefore, a sufficiently small (and thus more computationally expensive) mesh size is needed. 
	\item \textbf{Based on the point-wise displacement and point-wise phase-field}: this approach  monitors the crack behavior and the displacement in the whole geometry. Here, the Bayesian setting strives to find the inferred parameters $\chi^\star$ which minimize
	\begin{align}
	\|\bar{\boldsymbol{u}}(\boldsymbol{x})-\boldsymbol{u}(\boldsymbol{x},\chi^\star)-\varepsilon_1\mathcal{I}\|^2+\|\bar{d}(\boldsymbol{x})-d(\boldsymbol{x},\chi^\star)-\varepsilon_2\mathcal{I}\|^2,
	\end{align}
	where $\bar{\boldsymbol{u}}$ and $\bar{d}$ are the experimental data in the whole geometry with respective measurement errors $\varepsilon_1$ and $\varepsilon_2$. This method is informative and provides precise information since the displacement and phase-filed in the entire geometry are considered.  However, the measured data for the displacement can not be obtained easily. Furthermore, due to the mesh dependency of the problem, a  small mesh size must be chosen to guarantee that in the whole geometry, an accurate estimation of $\bar{\boldsymbol{u}}$ and $\bar{d}$ is obtained. Employing large meshes (larger length scale) leads to an overestimation of the fracture propagation, which also affects the neighboring elements. Therefore, the method is computationally prohibitive. 
	
	\item \textbf{Based on the point-wise phase-field propagation}: this approach is less complex than the previous method. Reliable experimental values of the crack path can be obtained using X-ray or $\mu$-CT scan in two- or three-dimensional problems. However, the computational problem regarding  mesh dependency still exists.
	
	\item \textbf{Based on snapshots of proper orthogonal decomposition (POD)}: this approach employs a reduced order method (ROM) to reduce the computational complexity. Here, the snapshots of the solution (using measurements of the crack phase-field) are used to construct the POD basis \cite{abbaszadeh2021reduced}. Since an efficient reduce-order method is used, the computational complexity can be reduced significantly.
		
	\item \textbf{Based on the effective stress-strain response}: this approach  explains the relation between $\boldsymbol{\varepsilon}$ and $\boldsymbol{\sigma}$. It shows useful information regarding different material properties such as bulk modulus, hardening, and yield strength. Therefore, considering the availability of the measurement, it entails an instructive procedure. Nevertheless, the computational costs, i.e., the effect of the mesh size and length scale, must be taken into account.
\end{itemize}   
In this work, we choose the load-displacement curve as the observation, and sufficiently small mesh sizes are used to model the crack propagation. Nevertheless, it is worth noting that POD-ROM approaches have significant simulation advantages (noticeable computational costs reduction), while methods based on the stress-strain response are significantly informative. These procedures will be addressed in future works.   

Now, we proceed to establish a Bayesian inversion ($\texttt{BI}$) setting to identify different parameters in ductile fracture. Let us assume the response of ductile phase-field fracture is either elastic, followed by elastic-plastic, followed by elastic-damage (hereafter $\texttt{E-P-D}$), or elastic, followed by elastic-plastic, followed elastic-plastic-damage (hereafter $\texttt{E-P-DP}$). Next, we aim to determine the candidate $\chi$ which belongs to $(\mu,K,H,\sigma_Y,\psi_c,G_c,w_0,l_p)$, as follows:

\begin{itemize}
	\item[(1)] To find $\tilde{\mu}$ and $\tilde{K}$, we set $H^0\rightarrow\infty$, $l^0_p\rightarrow0$ (in case of $\mathcal{M}_3$), $\chi^0_a\rightarrow0$ (in the anisotropic case) and $G^0_c\rightarrow\infty$ in $\mathcal{M}_1$, $\psi^0_c\rightarrow\infty$ in $\mathcal{M}_2$, and $w^0_0\rightarrow\infty$ in $\mathcal{M}_3$, thus reflecting an elastic response. We then have
	\begin{equation}
	(\tilde{\mu},\tilde{K})=\texttt{BI}\,(\mu^0,K^0,\sigma_Y^0,H^0,l^0_p,G^0_c,\psi^0_c,w^0_0,\chi^0_a).
	\end{equation}
	\item[(2)] To find $\tilde{\sigma_Y}$, we set $H^0\rightarrow 0$, $l^0_p\rightarrow0$ (in case of $\mathcal{M}_3$), $\chi^0_a\rightarrow0$ (in the anisotropic case),  and $G^0_c\rightarrow\infty$ in $\mathcal{M}_1$, $\psi^0_c\rightarrow\infty$ in $\mathcal{M}_2$, and $w^0_0\rightarrow\infty$ in $\mathcal{M}_3$, thus reflecting an ideal plastic response. We then have
	\begin{equation}
	\tilde{\sigma_Y}=\texttt{BI}\,(\tilde{\mu},\tilde{K},Y^0_0,H^0,l^0_p,G^0_c,\psi^0_c,w^0_0,\chi^0_a).
	\end{equation}
	\item[(3)] To find $\tilde{H}$, and $\tilde{l_p}$ (in case of $(\mathcal{M}_3)$), we set $\chi^0_a\rightarrow0$ (in the anisotropic case), $G^0_c\rightarrow\infty$ in $\mathcal{M}_1$, $\psi^0_c\rightarrow\infty$ in $\mathcal{M}_2$, and $w^0_0\rightarrow\infty$ in $\mathcal{M}_3$, thus reflecting an elastic-plastic response prior to fracture. We then have
	\begin{equation}
	(\tilde{H},\tilde{l_p})=\texttt{BI}\,(\tilde{\mu},\tilde{K},\tilde{\sigma_Y},H^0,l^0_p,G^0_c,\psi^0_c,w^0_0,\chi^0_a).
	\end{equation}
	\item[(4)] Depending on the model, to find $\tilde{\chi_a}$ (in the anisotropic case), $\tilde{G_c}$ in $\mathcal{M}_1$, $\tilde{\psi_c}$ in $\mathcal{M}_2$, and $\tilde{w_0}$ in $\mathcal{M}_3$, which reflect ductile anisotropic fracture response, thus we have,
	\begin{equation}
	(\tilde{G_c},\tilde{\psi_c},\tilde{w_0},\tilde{\chi_a})=\texttt{BI}\, \left(\tilde{\mu},\tilde{K},\tilde{\sigma_Y},\tilde{H},\tilde{l_p},G^0_c,\psi^0_c,w^0_0,\chi^0_a\right).
	\end{equation}
	\item[(5)] Finally, we will have the following parameter estimation
	\begin{equation}
	(\mu,K,\sigma_Y,H,l_p,G_c,\psi_c,w_0,\chi_a)=\texttt{BI}\, \left(\tilde{\mu},\tilde{K},\tilde{\sigma_Y},\tilde{H},\tilde{l_p},\tilde{G_c},\tilde{\psi_c},\tilde{w_0},\tilde{\chi_a}\right).
	\end{equation}
\end{itemize}
Figure \ref{FigureBA_ductile} shows the overall procedure, indicating all stages of the deformation process. Note that, from the implementation point of view, we set the limit $\infty$ as $10^8\times E$, where $E$ refers to Young's modulus and set the limit $0$ as 0. From the statistical point of view, we employ the MCMC techniques (Algorithms 1--\ref{algorithm3}) to identify the parameters in Step (1), then, we follow Step (2) to estimate $\sigma_Y$ and pursue the parameter identification procedure until we determine the whole material parameters (Step (4)). 

In a similar manner, if the response of ductile phase-field fracture is elastic, followed by elastic-damage, followed by elastic-plastic-damage, i.e., $\texttt{E-D-PD}$ (see \cite{alessi2017} for a detailed discussion on different possible evolutions), we first determine the elastic moduli, followed by the the anisotropic fracture properties by assuming that the response is brittle, and finally, we determine the plastic proprieties in the final dissipative stage.

\begin{figure}[!]
	\centering
	{\includegraphics[clip,trim=0cm 21cm 0cm 8cm, width=16cm]{Figures/Final/BA_ductile.pdf}}  %left, bottom, right and top 
	\caption{Step-wise Bayesian inversion method to determine the posterior density of the material unknowns for ductile phase-field fracture models.}
	\label{FigureBA_ductile}
\end{figure}


%
%%=======================================================================
%\sectpb[Section31]{Bayesian inversion for thermo-elastic-plastic solids }
%%=======================================================================
%
%%=======================================================================
%\sectpb[Section32]{Extension to the anisotropic setting}
%%=======================================================================
%
%%=======================================================================
%\sectpb[Section3]{The DRAM algorithm for phase-field trhomo-elastic-plastic fracturing materials}
%%=======================================================================
%
%\sectpb[Section3]{Ensemble Kalman filter and Markov chain Monte Carlo}
%%================================================================

==> sec4.tex <==
%=======================================================================
\sectpa[Section4]{Bayesian inversion for phase-field fracture \textcolor{red}{(NN+AK)}}
%=======================================================================


==> sec5.tex <==
%=======================================================================
\sectpa[Section5]{Numerical examples}
\label{Section5}
%=======================================================================
This section demonstrates the performance of the proposed Bayesian inversion approaches for parameter estimation within ductile phase-field fracture models presented earlier. We investigate four numerical examples. To validate the numerical method, the last two examples are concerned with experimental observations, in which the posterior responses compared with experimental load-displacement curves. The material parameters listed in Table~\ref{material-parameters} are considered, which are initialized based on \cite{ambati2016,ambati2015}.  

In the numerical simulations, the global primary variables are discretized using finite element basis functions, with bilinear quadrilateral $Q_1$ elements for the two-dimensional problems and 8-node hexahedral elements for the three-dimensional problems. An alternate minimization scheme is used for solving the variational equations resulting from ductile phase-field fracture (Sec. \ref{sec:models}). 
Thus, for model 1 $(\calM_1)$, and model 2 $(\calM_2)$, we alternately {solve} for $d$ by fixing ${\bm u}$, and then solving for ${\bm u}$ by fixing $d$ until convergence is reached. Accordingly, for model 3 $(\calM_3)$, we alternately {solve} for ${\bm u}$ by fixing $(\alpha,d)$, and the solve for $\alpha$ by fixing $(\bm u,d)$. Next, we obtain plastic strain $\Bve^p$ though the equivalent plastic evolution equation \req{plastic_law}, and lastly, we find $d$ by fixing $(\bm u,\alpha)$, until convergence is reached. Finally, in the MCMC  and the observational noise, $\sigma^2=10^{-3}$ is employed.

\TODO{Nima: Please mention the computational parameters, including number of iterations in different models (for $(\calM_3)$ was 10), NR-tolerance, stopping criterion for the iterations, etc. Please see page 36 and 37 of Thomas comments.}

\setcounter{table}{0}
\begin{table}[!ht]
	\caption{Material parameters used in the numerical experiments. The fixed values in all examples are mentioned. Other parameters are inferred with Bayesian inversion.}	\vspace{1mm}
	\centering
	\begin{tabular}{cllcccccc}
	  parameter & name                  & unit       & value     \\[2mm]\hline 
	   $\mu$        & shear modulus    &     $\mathrm{MPa}$ &$\mathrm{BI}$ \\[2mm]
	  $K$      & bulk modulus    &   $\mathrm{MPa}$     &$\mathrm{BI}$            \\[2mm]
	 $H$        & hardening modulus         & $\mathrm{MPa}$ &$\mathrm{BI}$\\[2mm]
	  $\sigma_Y$        & yield stress      & $\mathrm{MPa}$&$\mathrm{BI}$ \\[2mm]
	 	 	 	 $\alpha_{\text{crit}}$        & hardening critical value      & --&$\mathrm{BI}$ \\[2mm]
		 $\psi_c$     & specific fracture energy    & $\mathrm{MPa}$ &$\mathrm{BI}$\\[2mm]
	 $G_c$     & Griffith's energy release rate     & $\mathrm{MPa}$ &$\mathrm{BI}$\\[2mm]
	 $w_0$     & specific fracture toughness    & $\mathrm{MPa}$ &$\mathrm{BI}$\\[2mm]
	 		 		 $\zeta$    &driving scaling factor&--&$\mathrm{BI}$\\[2mm]
	 		 		 		 $\chi_a$ & penalty parameter &--&$\mathrm{BI}$\\[2mm]
		 $\eta_f$    & crack viscosity       & $\mathrm{N/m^{2}s}$&$10^{-9}$\\[2mm] 
		 $\eta_p$    & plasticity viscosity       & $\mathrm{N/m^{2}s}$&$10^{-9}$\\[2mm] 
	 $\kappa$    & stabilization parameter   & -- & $10^{-8}$& & \\[2mm]
		 $l_d$    & fracture length-scale  &  $\mathrm{mm}$  & $10^{-8}$ & \\[2mm]
		 $l_p$    & plastic length-scale     &$\mathrm{mm}$& $10^{-8}$ \\[2mm]
		 $\phi$       & fiber rotation & degree & $[30^{\circ}, 45^{\circ}, 60^{\circ}]$\\[2mm]
		\hline
		\label{material-parameters}
	\end{tabular}
\end{table}

\begin{table}[!]
	\caption{The uniform prior distribution of the inferred parameters in Example 1.}
	\vspace{1mm}
	\centering
	\begin{tabular}{llcccccccccccccc}
		&parameters  &$H$        & $\mu$    &   $K$   &   $\sigma_Y$   &$G_c$&$\alpha_{\text{crit}}$     &$\psi_c$   &$w_0$ &$l_p$ &$\zeta$ \\[2mm]\hline\\
		&   min   &150   & 20\,000  & 40\,000 &275 & 5 & 0.05 &20&20&0.5& 0.25& \\[4mm]
		& max &   375  &  40\,000  &  100\,000 & 400 &15 &0.2 & 60 &60&2.5& 10&\\[4mm]
		&   initial  &220  & 25\,000   & 80\,000 &350 & 12 & 0.12 &30& 25 & 1.2&2  \\[4mm]
		\hline
		\label{range1}
	\end{tabular}
\end{table}
%=======================================================================
\sectpb[Section51]{Example 1: Asymmetrically I-shaped specimen under tensile loading}
%=======================================================================
To gain a first insight into the performance of the Bayesian inversion approach, the following numerical example is concerned with the asymmetrically notched I-shaped specimen under tension.  The configuration is shown in Figure \ref{Figure1bvp}a. The geometrical dimensions are set as $H_1=110$ mm, $H_2=25$ mm, $r_1=3.625$ mm, $w_1=22$ mm, and $w_2=14.8$ mm, with half-circular notches of radius $r_2=2.5$ mm. The two notches placed at a vertical distance from the center of $10$ mm.

A monotonic displacement increment  ${\Delta \bar{u}}_y=2\times10^{-3}$ mm is applied in a vertical direction at the top boundary of the specimen. The minimum finite element size in the domain is $0.3$ mm, for which the heuristic requirement $h<l/2$ inside the localization zone is fulfilled. Consequently, the I-shaped domain partition contains 21598 elements. The material and numerical parameters are given in Table \ref{material-parameters} and Table \ref{range1}, respectively. 

\begin{figure}[!]
	\centering
	{\includegraphics[clip,trim=5cm 15cm 18cm 7.5cm, width=10cm]{Figures/Final/exm12.pdf}}  %left, bottom, right and top 
	\caption{ Geometry and boundary conditions of the I-shaped tensile specimen: (a) Example 1, and (b) Example 2.}
	\label{Figure1bvp}
\end{figure}


\begin{figure}[t!]
	\vspace{0.1cm}
	\hspace{-1cm}
	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/Model1/Ex1_mu.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/Model1/Ex1_K.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/Model1/Ex1_H.png}}
	\hfill 
	\vspace{0.1cm}
	\hspace{-1.1cm}
	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/Model1/Ex1_SY.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/Model1/Ex1_Ep.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/Model1/Ex1_Gf.png}}
	\hfill 
	\vspace{0.1cm}
	\hspace{-1.1cm}
	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/Ex2_Ps.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/zeta_M3.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/Example1/Model3/Ex1_w.png}}
	\caption{Example 1: the effect of the all studied parameters on  the load-displacement curve. Here, we illustrate the obtained curve by $(\mathcal{M}_1)$  for $\mu$, $K$, $H$, $\sigma_Y$, $\alpha_{\text{crit}}$, $G_c$ (the first and the second row). In the third row, we depict the effect of $\psi_c$ ($(\mathcal{M}_2)$) as well as $\zeta$ and $w_0$ ($(\mathcal{M}_3)$).}
	\label{Example1}
\end{figure}
%
\begin{table}[!]
	\caption{Example 1: the mean value of posterior density of  the model parameters for the three models.}
	\vspace{1mm}
	\centering
	\begin{tabular}{ccccccccccccccc}
		&model  &$H$        & $\mu$    &   $K$   &   $\sigma_Y$   &$G_c$&$\alpha_{\text{crit}}$     &$\psi_c$   &$w_0$ &$l_p$&$\zeta$  \\[2mm]\hline\\
		&    $(\mathcal{M}_1)$   &240   & 27\,212 & 71\,527 &335 & 10.5 & 0.11 &--&--&--&-- \\[4mm]
		& $(\mathcal{M}_2)$ &   241  & 27\,120  &  71\,245 & 330 &-- &-- & 41& &--&0.98&\\[4mm]
		&   $(\mathcal{M}_3)$  &248  & 26\,699   & 74\,500 &328 & -- & -- &--& 38 & 1.25&1.02  \\[4mm]
		\hline
		\label{Example1_posterior}
	\end{tabular}
\end{table}
%
\begin{table}[!]
	\caption{Example 1: using Bayesian inversion to estimate the equivalence of $\psi_c$  $(\mathcal{M}_2)$ with $\alpha_{\text{crit}}$ and $G_c$ $(\mathcal{M}_1)$ in addition to $w_0$ and $l_p$  $(\mathcal{M}_3)$.}
	\vspace{1mm}
	\centering
	\begin{tabular}{cccccccccccc}
		&$\psi_c$  &25        & 35   &   45   &   55   &65&      \\\hline 
		&    $\alpha_{\text{crit}}$   &0.065  & 0.092 & 0.12&0.136& 0.15 &   \\[2mm]
		& $G_c$&   8.25  & 10.1  &  12 & 15 &18   \\[2mm]
		& $w_0$&  20.8  & 29.1   &  38 & 48  &55 &   \\[2mm]
		& $l_p$& 1.05   &  1.11  & 1.25  & 1.4  &1.6 &   \\[2mm]
		\hline
		\label{Example1_equivalence}
	\end{tabular}
\end{table}

For all three models, the shear modulus $\mu$, the bulk modulus $K$, the hardening modulus $H$, and the yield stress $\sigma_Y$ are common. First, we study the effect of the common parameters on the load-displacement curve.  Figure \ref{Example1} shows the diagrams where $(\mathcal{M}_1)$ is used to obtain the solutions. To monitor different critical values $\alpha_{\text{crit}}$ and energy release rates $G_c$, as well as fracture energies $\psi_c$, $(\mathcal{M}_1)$ and $(\mathcal{M}_2)$ are respectively  employed. Moreover, we used $(\mathcal{M}_3)$ to observe how the curve is affected by specific values of $w_0$ and the parameter $\zeta$, as shown in Figure \ref{Example1}.
%

Next, we proceed to identify the effective parameters in the ductile fracture process using the Metropolis-Hastings algorithm introduced in Subsection \ref{MH1}. The Bayesian framework for ductile fracture is presented in Subsection \ref{bayesian}.
We employ a uniform distribution to estimate the parameters more accurately, as listed in Table \ref{range1} (the prior densities and the initial values) and use $N=10\,000$ number of candidates.  Regarding the reference values, a synthetic measurement is used, using a total number of degrees of freedom $\mathcal{N}_{\text{dof}}=28\,380$; the rest of the initial values are summarized in Table \ref{range1}.
%
The posterior density of the parameters using the three models is shown in Figure \ref{Example1_models}. The mean values of the posterior distributions are used to verify the parameter estimation. The inferred information is listed in Table \ref{Example1_posterior}. To verify the accuracy of the data, we employ the parameters in all three models and compute  the load-displacement until the fracture point. Figure \ref{example12} shows the curves resulting from the different models and the reference observation. An excellent agreement indicates that the Bayesian inversion framework identified the parameters correctly, showing a consistent behavior for all three models in all stages.

The efficiency of the Bayesian inversion for all models enables us to provide equivalence for the model parameters. As previously mentioned, all models have four common parameters, but each model is also characterized by its features. Here, we strive to find an equivalent value for different fracture energies. This allows us to use $(\mathcal{M}_1)$ and $(\mathcal{M}_3)$ and derive similar quantities in $(\mathcal{M}_2)$, and vice versa. To that end, we select the diagram estimated by $(\mathcal{M}_2)$ as the reference observation, where all parameters are chosen according to the estimated values (see Table \ref{Example1_posterior}). However, $\psi_c$ varies between 25 and 65. We again use the MH algorithm to identify the equivalence of $\psi_c$ in $(\mathcal{M}_1)$ (i.e, $G_c$ and $\alpha_{\text{crit}}$) and $(\mathcal{M}_3)$ (i.e., $l_p$ and $w_0$). The estimated quantities are summarized in Table \ref{Example1_equivalence}. Figure \ref{example1_psi} presents the results obtained by the inferred values, where, again, Bayesian inversion provides a very good agreement.
%%
%\begin{figure}[!t]
%	\centering
%	{\includegraphics[width=0.85\textwidth]{Figures/Example1/zeta_M3.png}}  %left, bottom, right and top 
%	\caption{Example 1. The effect of different values of $\zeta$ on the load-displacement curve. \TODO{(AK)-add this one in Figure 7 instead of $l_p$.} 
%	}
%	\label{example1_zata}
%\end{figure}

%width=6cm,height=3.75cm

 \begin{figure}[t!]
 \vspace{0.1cm}
  \hspace{-1cm}
 	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_mu.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_K.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_sigma.png}}
 	 \hfill 
 	   \vspace{0.1cm}
  \hspace{-1.1cm}
 	 		 \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_H.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_lp.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_Gc.png}}
 	 		  	 \hfill 
 	 		  	 \vspace{0.1cm}
 	 		  	 \hspace{-1.1cm}
 	 		  	  \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_psi.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_alpha.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example1/Ex1_zeta.png}}
 	\caption{Example 1: the posterior distribution of the effective parameters using $(\mathcal{M}_1)$, $(\mathcal{M}_2)$, and $(\mathcal{M}_3)$.}
 	\label{Example1_models}
 \end{figure}
 
 \begin{figure}[t!]
 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/Example1/Model2/Compare_model1_model2.png}} 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/Example2/compare_all.png}}  
 	\caption{Load-displacement curve computed using the inferred values, employing $(\mathcal{M}_1)$, $(\mathcal{M}_2)$, and $(\mathcal{M}_3)$. The reference values are depicted as well. Here, Table \ref{Example1_posterior} and Table \ref{Example2_posterior} are used for Example 1 (left) and Example 2 (right).}
 	\label{example12}
 \end{figure}

The resulting equivalent plastic strain ($\alpha$) and crack phase-field ($d$) at complete failure are shown in Figure \ref{Figure13}. The solutions are  based on the posterior density of the material parameters for different models, which are given in Table \ref{Example1_posterior}. Accordingly, the fracture path initiates within the maximum equivalent plastic regions, which appear near the notches. Next, the crack propagates in the plastic localization band, in which two cracks merge at the specimen center.  It can be observed that even though the load-displacement curves shown are practically identical in all models, the corresponding phase-field profiles, and thus, hardening profiles, are not. This can be explained, first of all, by the solution non-uniqueness of the phase-field fracture problem, and, secondly, by the fact that the different phase-field models in fact provide only the approximation of the fracture problem. Thus, the necessity of comparing the results with an experimental observation is crucial. Hereby, based on the experimental test provided in \cite{ambati2016} (second experiment), a sharp crack transition between two notches is expected. Thus $(\calM_2)$ and $(\calM_3)$ seem to yield a more accurate fracture pattern.
%
\begin{figure}[!]
	\centering
	\subfloat{{\includegraphics[clip,trim=0cm 21cm 16cm 4.5cm, width=12cm]{Figures/Final/A1.pdf}}}\\  %left, bottom, right and top 
	\subfloat{{\includegraphics[clip,trim=0cm 21cm 16cm 4.5cm, width=12cm]{Figures/Final/A2.pdf}}}\\  %left, bottom, right and top 
	\subfloat{{\includegraphics[clip,trim=0cm 20cm 16cm 4.5cm, width=12cm]{Figures/Final/A3.pdf}}}  %left, bottom, right and top 
	\caption{ Example 1: approximated solution obtained through the posterior density of the material parameters at complete failure. The hardening value $\alpha$ and the crack phase-field $d$ are shown for different models.}
	\label{Figure13}
\end{figure}
%

%
\begin{figure}[!t]
	\centering
   	{\includegraphics[width=0.85\textwidth]{Figures/Example1/PS_all.png}}  %left, bottom, right and top 
	\caption{Example 1: the load-displacement curve for the inferred equivalent values $\psi_c$, with  $\psi_c$ varying between 25 and 65.  
	}
	\label{example1_psi}
\end{figure}
%
\begin{figure}[!]
	\centering
	{\includegraphics[clip,trim=0cm 1cm 12cm 6cm, width=13cm]{Figures/Final/F2.pdf}}  %left, bottom, right and top 
	\caption{ Example 2: material parameters distribution (prior density) on each element of the domain $\calB$.}
	\label{Figure21}
\end{figure}
%

%
%=======================================================================
\sectpb[Section52]{Example 2: I-shaped tensile specimen for anisotropic ductile fracture}
%=======================================================================

The main objective of this example is the adoption of the Bayesian inversion for an  anisotropic ductile phase-field fracture process. The boundary value problem depicted in Figure \ref{Figure1bvp}b consists of an I-shaped specimen with a circular void in the center of the domain. The geometrical dimensions in Figure \ref{Figure1bvp}b are set as $H_1=110$ mm, $H_2=28.6$ mm, $w_1=22$ mm, and $w_2=14.8$ mm, with central void that is located in $(x,y)=(H_1/2,w_1/2)$ with a radius of $r=2.5$ mm.

Herein, we assume that the material constituents are not distributed uniformly through the continuum domain, and thus, the material is divided into several phases. Hence, heterogeneity in strength from one area of the domain to another one is expected. As a result, the pseudo-energy density per unit volume $W$ given in \req{psuedo-energy} is related to the position of point $\Bx$ within the domain. Here, we consider the parameters as a random field (with given mean and variation).
Figure \ref{Figure21} illustrates the fluctuation of different material parameters (on the element-wise basis) where a  10\% variation is included. For instance, for the parameter $K$, the expectation is assumed as $K$=75\,000\,MPa,  with  a variation between 71\,700\,MPa and 78\,800\,MPa. This fluctuation will be used to provide the reference observation. In other words, we will replicate 500 simulations (with a specific mesh size) to estimate the reference observation considering the mentioned variation. The distribution of the parameters on the geometry is shown in Figure \ref{Figure21}.

The numerical example is performed by applying a monotonic displacement increment  ${{\Delta \bar{u}}_y}=2\times10^{-3}$ mm in the vertical direction at the top boundary of the specimen (Figure \ref{Figure1bvp}). To remove the rigid body motion, the bottom edge is fixed in the $x-y$ directions. The minimum finite element size is $0.45$ mm. The I-shaped domain partition contains 17038 elements. 

 \begin{figure}[t!]
	\vspace{0.1cm}
	\hspace{-1cm}
	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_mu.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_K.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_sigma.png}}
	\hfill 
	\vspace{0.1cm}
	\hspace{-1.1cm}
	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_H.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_lp.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_gc.png}}
	\hfill 
	\vspace{0.5cm}
	\hspace{-1.1cm}
	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_psi.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_alpha.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_zeta.png}}
	\hfill 
	\vspace{0.1cm}
	\hspace{4.75cm}
	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example2/Ex2_chi.png}}  
	\caption{Example 2: the posterior distribution of the effective parameters using $(\mathcal{M}_1)$, $(\mathcal{M}_2)$, and $(\mathcal{M}_3)$.}
	\label{Example2_models}
\end{figure}

\begin{figure}[!]
	\centering
	{\includegraphics[width=0.85\textwidth]{Figures/Example2/Aniso_all_30_60.png}}  %left, bottom, right and top 
	\caption{Example 2: the load-displacement curve obtained by the estimated values for $\phi=30^o$ and $\phi=60^o$ and all three models.
	}
	\label{example2-phi}
\end{figure}

In this example, to determine the mechanical parameters, the DRAM algorithm is used. Due to the anisotropic structure of the solid, in addition to the identified parameters in Example 1, the penalty parameter $\chi_a$ must be estimated. Here, we select $\phi=45^o$ for the parameter identification and propose $N=10\,000$ candidates. A synthetic reference value using $\mathcal{N}_{\text{dof}}=26\,870$ is employed as the reference observation considering the already mentioned parameter variation. 
The prior (uniform) densities of the parameters are listed in Table \ref{range2}.  For each parameter, the inferred values by different models are relatively similar, which highlights the efficiency of the Bayesian setting. The posterior distributions are depicted in Figure \ref{Example2_models}. The mean values of the posterior distributions are given in Table \ref{Example2_posterior} using $(\mathcal{M}_1)$, $(\mathcal{M}_2)$, and $(\mathcal{M}_3)$. Again, we solve the model equations employing the identified parameters to verify the effectiveness of the Bayesian framework, as shown in Figure \ref{example12}. All diagrams show that implementing the DRAM algorithm gives rise to a reasonable agreement between the models and also the reference observation.

For further investigation, the inferred parameters are used for two additional preferential fiber directions, namely $\phi=30^o$ and $\phi=60^o$. Again, Figure \ref{example2-phi} illustrates the robustness of the Bayesian setting, showing for all models and different orientations a consistent behavior in the in elastic, plastic, and fracture stages.  Figures \ref{Figure22} and \ref{Figure23} illustrate the crack phase-field  and equivalent plastic strain solutions, respectively, at complete failure for $\phi=30^o$, $\phi=45^o$, and $\phi=60^o$. Note that the solutions are based on the posterior density of the material parameters, which are given in Table \ref{Example3_posterior}. An important observation is that both the equivalent plastic strain and the crack phase-field evolve in the direction of the preferred fiber orientation. 
%
\begin{table}[!]
	\caption{The uniform prior distribution of the inferred parameters in Example 2.}
	\vspace{1mm}
	\centering
	\begin{tabular}{llcccccccccccccc}
		&parameters  &$H$        & $\mu$    &   $K$   &   $\sigma_Y$   &$G_c$&$\alpha_{\text{crit}}$     &$\psi_c$   &$w_0$ &$l_p$ &$\zeta$ &$\chi_a$  \\[2mm]\hline\\
		&   min   &150   & 20\,000  & 40\,000 &275 & 5 & 0.01 &10&10&0.5& 0.25& 10\\[4mm]
		& max &   375  &  40\,000  &  100\,000 & 400 &15 &0.2 & 60 &60&10& 10&100\\[4mm]
		\hline
		\label{range2}
	\end{tabular}
\end{table}
%
\begin{table}[!]
	\caption{Example 2: the mean value of posterior density of  the model parameters for the three models.}
	\vspace{1mm}
	\centering
	\begin{tabular}{ccccccccccccccc}
		&model  &$H$        & $\mu$    &   $K$   &   $\sigma_Y$   &$G_c$&$\alpha_{\text{crit}}$     &$\psi_c$   &$w_0$ &$l_p$&$\zeta$ &$\chi_a$  \\[2mm]\hline\\
		&    $(\mathcal{M}_1)$   &265   & 26\,050 & 94\,010 &355 & 11.6 & 0.038  &--&--&--&-- &50 \\[4mm]
		& $(\mathcal{M}_2)$ &   245  & 26\,100  &  92\,100 & 354 &-- &-- & 25.25& &--&1.01&52\\[4mm]
		&   $(\mathcal{M}_3)$  &220  & 26\,300   & 88\,950 &340 & -- & -- &--& 22 & 8.29&1.6 &55 \\[4mm]
		\hline
		\label{Example2_posterior}
	\end{tabular}
\end{table}
%
\begin{table}[!]
	\caption{The uniform prior distribution of the inferred parameters in Example 3.}
	\vspace{1mm}
	\centering
	\begin{tabular}{llcccccccccccccc}
		&parameters  &$H$        & $\mu$    &   $K$   &   $\sigma_Y$   &$G_c$&$\alpha_{\text{crit}}$     &$\psi_c$   &$w_0$ &$l_p$ &$\zeta$ & \\[2mm]\hline\\
		&   min   &10   & 20\,000  & 40\,000 &50 & 100 & 0.001 &5&5&0.001& 1\\[4mm]
		& max &   50  &  40\,000  &  100\,000 & 200 &300 &0.1 & 25 &25&10& 20\\[4mm]
		\hline
		\label{range33}
	\end{tabular}
\end{table}
%
\begin{table}[!]
	\caption{Example 3: the mean value of posterior density of  the model parameters for the three models.}
	\vspace{1mm}
	\centering
	\begin{tabular}{ccccccccccccccc}
		&model  &$H$        & $\mu$    &   $K$   &   $\sigma_Y$   &$G_c$&$\alpha_{\text{crit}}$     &$\psi_c$   &$w_0$ &$l_p$&$\zeta$ & \\[2mm]\hline\\
		&    $(\mathcal{M}_1)$   &30   & 26\,500 & 73\,500 &115 & 248 & 0.0142  &--&--&--&--  \\[4mm]
		& $(\mathcal{M}_2)$ &   15  & 26\,200  &  73\,700 & 116 &-- &-- & 13.4& &--&2\\[4mm]
		&   $(\mathcal{M}_3)$  &15  & 30\,100   & 75\,050 &112 & -- & -- &--& 10.3 & 0.0018&15  \\[4mm]
		\hline
		\label{Example3_posterior}
	\end{tabular}
\end{table}
%
 \begin{figure}[!]
	\centering
	{\includegraphics[clip,trim=0cm 6cm 16cm 4.5cm, width=12cm]{Figures/Final/B1.pdf}}  %left, bottom, right and top 
	\caption{ Example 2: the crack phase-field at complete failure for all three models. Different referential fiber direction within transversly isotropic setting with (a) $\phi=30^o$, (b) $\phi=45^o$, and (c) $\phi=60^o$.}
	\label{Figure22}
\end{figure}

\begin{figure}[!]
	\centering
	{\includegraphics[clip,trim=0cm 6cm 16cm 4.5cm, width=12cm]{Figures/Final/B2.pdf}}  %left, bottom, right and top 
	\caption{ Example 2: the equivalent plastic strain at complete failure for all three models. Different referential fiber direction within transversly isotropic setting with (a) $\phi=30^o$, (b) $\phi=45^o$, and (c) $\phi=60^o$.}
	\label{Figure23}
\end{figure}

%=======================================================================
 \sectpb[Section53]{ Example 3: Flat I-shaped Al-5005 test under tensile loading}
%=======================================================================

While so far, synthetic observations have been used, the last two examples are concerned with experimental observations to estimate the posterior density of the material unknowns. The following example considers an I-shaped specimen for Al-5005 material under tensile loading. We aim at reproducing the experimentally observed ductile fracture process of the tensile test through the proposed Bayesian inversion framework. The boundary value problem is shown in Figure \ref{exm3bvp}a. The experimental observations of necking and fracture are shown in Figure \ref{exm3bvp}c.  The geometrical dimensions are set as $H_1=144$ mm, $H_2=27$ mm, $H_3=22$ mm, $w_1=20$ mm, $w_2=12$ mm, and $r_1=14$ mm. The specimen domain has a $3$ mm thickness, as shown in Figure \ref{exm3bvp}b.

The numerical example is performed by applying a monotonic displacement increment  ${\Delta \bar{u}}_y=0.02$ mm in the vertical direction at the top boundary of the specimen for 300 time steps. The minimum finite element size is $1.5$ mm. The flat I-shaped domain partition contains 3230 hexahedron linear elements.

\begin{figure}[!ht]
	\centering
	{\includegraphics[clip,trim=4cm 17cm 7cm 5cm, width=16cm]{Figures/Final/exm3.pdf}}  %left, bottom, right and top 
	\caption{Example 3: flat I-shaped Al-5005 test under tensile loading. (a) Geometry of specimen with boundary conditions, (b) three-dimensional prospective, and (c) experimental observation reprinted from \cite{ambati2016}.}
	\label{exm3bvp}
\end{figure}
 
Both DRAM and ensemble-Kalman filter (EKF) are efficient MCMC techniques and have shown their computational performance reasonably. However, a fair comparison can determine which method will be more advantageous in ductile fracture.  
 
%=======================================================================


In Subsection \ref{MH}, we studied the performance of the MH algorithm and used it in Example 1. As the first comparison, we employ the DRAM and EKF algorithms to estimate Young's modulus in the one-dimensional problem. Figure \ref{convergence1} shows the $\hat{R}$-convergence for both methods, where using the Kalman filter enhances the method efficiency and increases its convergence rate. Here, 4 parallel MCMCs are used ($m=4$) and in each chain, 2\,500 samples are employed. The Kalman filter is used for whole the chain, and the prior density is a uniform distribution between 0.5 and 20.  Here, we used a threshold of 1.2 (shown with a dashed red line), and as shown in most of the samples, PSRF is below the threshold.

In the I-shaped example, another comparison is used, taking all inferred parameters into account. We use $n=1\,000$ and five parallel MCMCs ($m=5$) with a uniform distribution indicated in Table \ref{range33}. Figure \ref{convergence2} shows that by employing EKF in all parameters, fewer candidates are necessary to converge to the posterior density. Indeed, for all parameters excluding $K$, after $1\,500$ samples, $\hat{R}$-statistics converges to 1, showing a high level of accuracy. The performance of the DRAM is acceptable, since most of the variables after $2\,500$ samples are below the threshold, although again, the bulk modulus shows more variation (probably due to the large chosen prior density).
%
 \begin{figure}[t!]
 	\vspace{0.1cm}
 	\hspace{-1cm}
 	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_mu.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_K.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_sigma.png}}
 	\hfill 
 	\vspace{0.1cm}
 	\hspace{-1.1cm}
 	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_H.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_lp.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_gc.png}}
 	\hfill 
 	\vspace{0.5cm}
 	\hspace{-1.1cm}
 	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_psi.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_alpha.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example3/Ex3_zeta.png}}
 	\caption{Example 3: the posterior distribution of the effective parameter using $(\mathcal{M}_1)$, $(\mathcal{M}_2)$, and $(\mathcal{M}_3)$.}
 	\label{Example3_models}
 \end{figure}
%
 \begin{figure}[t!]
 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/Ishape/Ishape_all}} 	\subfloat{\includegraphics[width=0.5\textwidth]{Figures/sandia/Sandia_all}}  
 	\caption{Load-displacement curve computed using the inferred values, employing $(\mathcal{M}_1)$, $(\mathcal{M}_2)$, and $(\mathcal{M}_3)$. The reference values are depicted as well. The experimental data are depicted with red. Here, Table \ref{Example3_posterior} and Table \ref{Example4_posterior} are used for Example 3 (left) and Example 4 (right). The results of Example 4 are also compared with the results of \cite{ambati2016}.}
 	\label{example34}
 \end{figure}
 
According to the above-mentioned discussion, we choose the EKF technique for the rest of the examples. We use five parallel MCMCs with $2\,000$ samples. For the observation, we use experimental data taken from \cite{ambati2016}. Figure \ref{Example3_models} shows the posterior density of estimated parameters, and the mean values are summarized in Table \ref{Example3_posterior}. We then employ the identified quantities in all three models. Figure \ref{Figure31} shows a comparison between the load-displacement curve obtained by the models and the experiments. Interestingly, by employing the Bayesian framework, all crack propagation stages (until fracture reaches the boundary) are modeled accurately.

%\ju[inline]{Should this study be shown before examples 1 and 2? We can then say that from the conclusion, we use the simple MH algorithm for the synthetic study (1 and 2) and the EKF for the experimental ones (3 and 4).}
%
%\ju[inline]{There is a missing reference in the legend of Figure 21.}


Next, we investigate the ductile failure response employing the posterior density of the material parameters given in Table \ref{Example3_posterior}. The evolution of the crack phase-field $d$ is provided in Figure \ref{Figure31} at three deformation stages up to complete failure. Additionally, the equivalent plastic strain $\alpha$ at final failure is shown. It can be grasped that, regardless of the formulations, fracture initiation appears at the center of the specimen, and then evolves towards the two edges of the specimen until complete failure. The first important observation is that the simulation results are in well-agreement with the experimental failure pattern shown in Figure \ref{exm3bvp}c. Another important observation is that the crack phase-field in $(\calM_2)$ and $(\calM_3)$ is more diffuse than $(\calM_1)$. The main reason for this is that the crack driving force of $(\calM_1)$ is scaled by $\alpha$; thus, the phase-field diffusivity is strongly coupled to the ductile response; see Remark \ref{Cdriv_m1}. 

%
 \begin{figure}[!]
	\centering
	\subfloat{{\includegraphics[clip,trim=2cm 21cm 8cm 4.5cm, width=15cm]{Figures/Final/C1.pdf}}}\\  %left, bottom, right and top 
	\subfloat{{\includegraphics[clip,trim=2cm 21cm 8cm 4.5cm, width=15cm]{Figures/Final/C2.pdf}}}\\  %left, bottom, right and top 
	\subfloat{{\includegraphics[clip,trim=2cm 19cm 8cm 4.5cm, width=15cm]{Figures/Final/C3.pdf}}}  %left, bottom, right and top 
	\caption{ Example 3: (a) the equivalent plastic strain at complete failure, and (b) the evolution of the crack phase-field  for different deformation stages up to final failure at $\bar{u}_y=6$ mm}. 
	\label{Figure31}
\end{figure}
%
%=======================================================================
\sectpb[Section54]{Example 4:  Sandia fracture challenge}
%==========================================================
%
The last example aims at estimating the posterior density of the material unknowns for a specimen frequently used in the literature, namely, a Sandia fracture challenge \cite{boyce2014sandia}. The 2014 fracture challenge problem launched by the Sandia National Lab \cite{boyce2014sandia} has provided an ideal platform to assess the computational predictions capability and limitations of each participating team \cite{zhang2014modeling}. Specifically, this challenge aims to evaluate the computational ability to predict crack initiation and propagation of ductile fracture with respect to the experimental observation. As reported in \cite{ambati2016}, standard phase-field formulations without estimating accurate ductile material properties quantitatively overestimates the post-yielding load-displacement response, which can be improved by performing an accurate calibration of the plasticity and phase-field parameters. Hence, we aim at reproducing the experimentally observed Sandia fracture challenge through proposed Bayesian inversion framework.


%Accordingly, the prior density function of material parameters are used in this numerical examples is based on \cite{guo2013experimental, ambati2016}, and given in Table \ref{range3}. 

The experiments are based on the material Al-5052 H34, which experimentally induces a complex failure mode; see \cite{guo2013experimental, ambati2016}. The configuration is shown in Figure \ref{exm4bvp}a, while the experimental observations are shown in Figure \ref{exm3bvp}c.  The geometrical configuration includes two pins. The top pin is displaced vertically, while the lower pin is fixed in all directions. The geometrical dimensions are set as $H_1=80$ mm, $H_2=35$ mm, $H_3=15$ mm, $H_4=6.5$ mm, $w_1=22$ mm, $w_2=36$ mm, and $w_3=12.5$ mm. The pins have an identical radius of $r_1=6$ mm, while the horizontal notch is rounded with a radius of $r_5=3.25$ mm. The specimen includes three voids with centers and radii $c_2=(x_2,y_2)=(27,32)$ mm and $r_2=3$ mm, $c_3=(x_3,y_3)=(24,45)$ mm and $r_3=1.75$ mm, and $c_4=(x_4,y_4)=(22,38)$ mm and $r_4=1.75$ mm. The specimen domain has a $2$ mm thickness, as shown in Figure \ref{exm4bvp}b.

The numerical example is performed by applying a monotonic displacement increment  ${\Delta \bar{u}}_y=0.02$ mm in the vertical direction at the top pin for 400 time steps. The minimum finite element size is $0.32$ mm. Consequently, the Sandia specimen domain partition contains 17980 hexahedron linear elements.

Due to its efficiency, the EKF technique is again considered for this example to identify the parameters. We use four parallel MCMCs with $2\,500$ samples. The experimental data (reference observation) is taken from \cite{ambati2016} and the prior densities are indicated in Table \ref{range3}. The posterior distributions are shown in Figure \ref{Example4_models}, while the mean values summarized in Table \ref{Example4_posterior}. Finally, once again we solve $(\mathcal{M}_1)$, $(\mathcal{M}_2)$, and $(\mathcal{M}_3)$ using the inferred values, and compare the results with those obtained in \cite{ambati2016}. As shown in Figure \ref{example34}, by employing the proposed Bayesian inversion framework, the parameters are estimated accurately, showing a very good agreement between the simulated data in all models and the experiments. This implementation also enhanced the computational capabilities of $(\mathcal{M}_1)$, showing an improved model accuracy compared to the results obtained in \cite{ambati2016}.
%
\begin{figure}[!ht]
	\centering
	{\includegraphics[clip,trim=0cm 20cm 0cm 5cm, width=16cm]{Figures/Final/exm4.pdf}}  %left, bottom, right and top 
	\caption{Example 4: Sandia fracture challenge. (a) Geometry of specimen with their boundary condition, (b) three-dimensional prospective, and (c) experimental observation reprinted from \cite{ambati2016}.}
	\label{exm4bvp}
\end{figure}
%
\begin{table}[!]
	\caption{Example 4: the uniform distribution of the inferred parameters in the Sandia example.}
	\vspace{1mm}
	\centering
	\begin{tabular}{llcccccccccccccc}
		&parameters  &$H$        & $\mu$    &   $K$   &   $\sigma_Y$   &$G_c$&$\alpha_{\text{crit}}$     &$\psi_c$   &$w_0$ &$l_p$ &$\zeta$ & \\[2mm]\hline\\
		&   min   &5   & 20\,000  & 40\,000 &150 & 100 & 0.001 &10&10&5& 1\\[4mm]
		& max &   20  &  40\,000  &  100\,000 & 300 &400 &0.3 & 50 &50&30& 20\\[4mm]
		\hline
		\label{range3}
	\end{tabular}
\end{table}
%
\begin{table}[!]
	\caption{Example 4: the mean value of posterior density of  the model parameters for the three models.}
	\vspace{1mm}
	\centering
	\begin{tabular}{ccccccccccccccc}
		&model  &$H$        & $\mu$    &   $K$   &   $\sigma_Y$   &$G_c$&$\alpha_{\text{crit}}$     &$\psi_c$   &$w_0$ &$l_p$&$\zeta$ & \\[2mm]\hline\\
		&    $(\mathcal{M}_1)$   &9.8   & 25\,500 & 67\,500 &195 & 360 & 0.2  &--&--&--&--  \\[4mm]
		& $(\mathcal{M}_2)$ &   10  & 26\,200  &  67\,200 & 194 &-- &-- & 35& &--&8\\[4mm]
		&   $(\mathcal{M}_3)$  &10.1  & 25\,900   & 67\,800 &195 & -- & -- &--& 28 & 9.64&15  \\[4mm]
		\hline
		\label{Example4_posterior}
	\end{tabular}
\end{table}
 %
 \begin{figure}[b!]
 	\vspace{0.1cm}
 	\hspace{-1cm}
 	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_mu.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_K.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_sigma.png}}
 	\hfill 
 	\vspace{0.1cm}
 	\hspace{-1.1cm}
 	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_H.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_lp.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_gc.png}}
 	\hfill 
 	\vspace{0.5cm}
 	\hspace{-1.1cm}
 	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_psi.png}}   \subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_alpha.png}}  	\subfloat{\includegraphics[width=0.37\textwidth]{Figures/RESULT/Example4/Ex4_zeta.png}}
 	\caption{Example 4: the posterior distribution of the effective parameters using $(\mathcal{M}_1)$, $(\mathcal{M}_2)$, and $(\mathcal{M}_3)$.}
 	\label{Example4_models}
 \end{figure}

For a better insight into the fracture process in all models, the evolution of the crack phase-field $d$ is provided in Figure \ref{Figure41} at three deformation stages up to complete failure. Additionally, the equivalent plastic strain $\alpha$ at final failure is shown. Note that the solutions are based on the posterior density of the material parameters, which are given in Table \ref{Example4_posterior}.

It can be grasped that, for all three models, the fracture path first initiates at the void located in the middle of the specimen, and afterwards, evolves outwards the right edge of the domain. In addition, a secondary crack initiates from the central void, but this time from its left side, and then propagates towards the left edge of the specimen until complete failure. Based on our numerical result, it is worth noting that this step of crack evolution can be no longer predictable through Model 2. Note further that the simulation results are in well-agreement with the experimental failure pattern shown in Figure \ref{exm4bvp}c. 
%
 \begin{figure}[!t]
	\centering
	\subfloat{{\includegraphics[clip,trim=0cm 23cm 0cm 4.5cm, width=16cm]{Figures/Final/D1.pdf}}}\\  %left, bottom, right and top 
	\subfloat{{\includegraphics[clip,trim=0cm 23cm 0cm 4.5cm, width=16cm]{Figures/Final/D2.pdf}}}\\  %left, bottom, right and top 
	\subfloat{{\includegraphics[clip,trim=0cm 21cm 0cm 4.5cm, width=16cm]{Figures/Final/D3.pdf}}}  %left, bottom, right and top 
	\caption{ Example 4: (a) The equivalent plastic strain at complete failure, and (b) the evolution of the crack phase-field for different deformation stages up to final failure at $\bar{u}_x=8$ mm. The final fracture stage was not captured with Model 2 due to lack of convergence.}
	\label{Figure41}
\end{figure}

\ju[inline]{We should change the text in Fig. 25 from 'it is not converged' to 'not converged'. Or even better, remove it, since it's now mentioned in the caption.}
 


